Policy Optimization for Markov Games: Unified Framework and Faster Convergence

This paper studies policy optimization algorithms for multi-agent reinforcement learning. We begin by proposing an algorithm framework for two-player zero-sum Markov Games in the full-information setting, where each iteration consists of a policy update step at each state using a certain matrix game algorithm, and a value update step with a certain learning rate. This framework unifies many existing and new policy optimization algorithms. We show that the state-wise average policy of this algorithm converges to an approximate Nash equilibrium (NE) of the game, as long as the matrix game algorithms achieve low weighted regret at each state, with respect to weights determined by the speed of the value updates. Next, we show that this framework instantiated with the Optimistic Follow-The-Regularized-Leader (OFTRL) algorithm at each state (and smooth value updates) can find an $\mathcal{\widetilde{O}}(T^{-5/6})$ approximate NE in $T$ iterations, and a similar algorithm with slightly modified value update rule achieves a faster $\mathcal{\widetilde{O}}(T^{-1})$ convergence rate. These improve over the current best $\mathcal{\widetilde{O}}(T^{-1/2})$ rate of symmetric policy optimization type algorithms. We also extend this algorithm to multi-player general-sum Markov Games and show an $\mathcal{\widetilde{O}}(T^{-3/4})$ convergence rate to Coarse Correlated Equilibria (CCE). Finally, we provide a numerical example to verify our theory and investigate the importance of smooth value updates, and find that using "eager" value updates instead (equivalent to the independent natural policy gradient algorithm) may significantly slow down the convergence, even on a simple game with $H=2$ layers.

==> Notes/Sections/new_alg.tex <==
\section{New 2p0s algorithm with $1/T$ rate}

\begin{algorithm}[h]
\caption{Modified OFTRL (max-player; Q form)}
\label{algorithm:modified-oftrl-q}
\begin{algorithmic}[1]
\STATE \textbf{Initialize:} $\up{Q}_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$t=1,\dots,T$}
\FOR{$h=H,\dots,1$}
\STATE Update policies for all $s\in\cS$ by OFTRL:
\vspace{-5pt}
\begin{align*}
    & \textstyle \mu^{t}_h(a | s) \propto_a \exp\paren{ (\eta/w_t) \cdot \brac{ \sum_{i=1}^{t-1} w_i(\up{Q}_h^i\nu_h^i)(s, a) + w_t(\up{Q}_h^{t-1}\nu_h^{t-1})(s, a) } }.
    % & \textstyle \nu^{t}_h(b | s) \propto_b \exp\paren{ -(\eta/w_t) \cdot \brac{ \sum_{i=1}^{t-1} w_i((Q_h^i)^\top\mu_h^i)(s, b) + w_{t-1}((Q_h^{t-1})^\top\mu_h^{t-1})(s, b) } }. 
\end{align*}
\vspace{-10pt}
\STATE Update Q-value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\vspace{-5pt}
\begin{align}\label{eq:up-Q}
    \textstyle \up{Q}_h^{t}(s,a,b) \setto r_h(s,a,b) + \P_h\brac{\max_{\mu^\dagger\in\Delta_\cA} \<\mu^\dagger, \sum_{i=1}^t \alpha_t^i \up{Q}_{h+1}^i\nu_{h+1}^i \>} (s,a,b).
    % (1-\alpha_t) Q_h^{t-1}(s,a,b) + \alpha_t \paren{r_h + \P_h[ (\mu_{h+1}^t)^\top Q_{h+1}^t\nu_{h+1}^t ]} (s,a,b).
\end{align}
\vspace{-5pt}
\ENDFOR
\ENDFOR
\STATE Output state-wise average policy for all $(h,s)$:
\vspace{-5pt}
\begin{equation*}
    \textstyle \widehat{\mu}_h^T(\cdot|s) \setto \sum_{t=1}^T\alpha_T^t\mu_{h}^{t}(\cdot|s).
\end{equation*}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Modified OFTRL (max-player; V form)}
\label{algorithm:modified-oftrl-v}
\begin{algorithmic}[1]
\STATE \textbf{Initialize:} $\up{V}_h^1(s)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$t=1,\dots,T$}
\FOR{$h=H,\dots,1$}
\STATE Update policies for all $s\in\cS$ by OFTRL:
\vspace{-5pt}
\begin{align*}
    & \textstyle \mu^{t}_h(a | s) \propto_a \exp\paren{ (\eta/w_t) \cdot \brac{ \sum_{i=1}^{t-1} w_i\up{L}_h^i(s, a) + w_{t-1}\up{L}_h^{t-1}(s, a) } }.
    % & \textstyle \nu^{t}_h(b | s) \propto_b \exp\paren{ -(\eta/w_t) \cdot \brac{ \sum_{i=1}^{t-1} w_i((Q_h^i)^\top\mu_h^i)(s, b) + w_{t-1}((Q_h^{t-1})^\top\mu_h^{t-1})(s, b) } }. 
\end{align*}
\vspace{-10pt}
\STATE Update losses for all $(s,a)\in\cS\times\cA$:
\vspace{-5pt}
\begin{align}
    \textstyle \up{L}_h^t(s,a) \setto \< r_h(s,a,\cdot) + \brac{\P_h\up{V}_{h+1}^t}(s,a,\cdot), \nu_h^t(\cdot|s) \>.
\end{align}
\vspace{-10pt}
\STATE Update V-value for all $s\in\cS$:
\vspace{-5pt}
\begin{align}
    \textstyle \up{V}_h^t(s) \setto \max_{\mu^\dagger\in\Delta_\cA} \< \mu^\dagger, \sum_{i=1}^t \alpha_t^i \up{L}_h^i(s,\cdot) \>.
    % \up{Q}_h^{t}(s,a,b) \setto r_h(s,a,b) + \P_h\brac{\max_{\mu^\dagger\in\Delta_\cA} \<\mu^\dagger, \sum_{i=1}^t \alpha_t^i \up{Q}_{h+1}^i\nu_{h+1}^i \>} (s,a,b).
    % (1-\alpha_t) Q_h^{t-1}(s,a,b) + \alpha_t \paren{r_h + \P_h[ (\mu_{h+1}^t)^\top Q_{h+1}^t\nu_{h+1}^t ]} (s,a,b).
\end{align}
\vspace{-5pt}
\ENDFOR
\ENDFOR
\STATE Output state-wise average policy for all $(h,s)$:
\vspace{-5pt}
\begin{equation*}
    \textstyle 
    \widehat{\mu}_h^T(\cdot|s) \setto \sum_{t=1}^T\alpha_T^t\mu_{h}^{t}(\cdot|s).
\end{equation*}
\end{algorithmic}
\end{algorithm}

==> Notes/Sections/proof.tex <==

\section{Proofs}
In this section, we consider the following definitions of regret, which is slightly different from the definition in (cite??):
\begin{talign*}
    & \reg_{h,\mu}^t(s) \defeq \max_{\mu^\dagger\in\Delta_\cA} \sum_{i=1}^t \alpha_t^i \<\mu^\dagger - \mu_h^i(\cdot|s), \brac{\up Q_h^i\nu_h^i}(s, \cdot)\>, \\
    & \reg_{h,\nu}^t(s) \defeq \max_{\nu^\dagger\in\Delta_\cB} \sum_{i=1}^t \alpha_t^i \< \nu_h^i(\cdot|s) - \nu^\dagger, \brac{(\low Q_h^i)^\top\mu_h^i}(s, \cdot) \>,  \\
    & \reg_{h,\mu+\nu}^t \defeq \max_{s\in\cS} \up\reg_{h,\mu}^t(s) + \low\reg_{h,\nu}^t(s).
\end{talign*}
\begin{lemma}\label{lemma:up-low-sandwich}
\begin{equation*}
    \low{Q}_h^t(s,a,b)\le Q^\star_h(s,a,b) \le \up Q_h^t(s,a,b).
\end{equation*}
\begin{proof}


\end{proof}
\end{lemma}

% \begin{lemma}[Performance difference for Markov policies]\label{lem:duality-2}
% In two-player zero-sum Markov games, suppose a Markov policy $(\mu,\nu)$ satisfies the following for all $h\in[H+1]$:
% \begin{align*}
%     &\max_{s} \max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB} \left(\brac{(\mu^\dagger)^\top \up Q_h^\star \nu_h}(s)- \brac{\mu_h^\top \low Q_h^\star \nu^\dagger}(s)\right)\le \epsilon_h
% \end{align*}
% Then we have for all $h\in[H]$ that
% \begin{align*}
%     \max\set{ \|V_h^{\dagger,\nu} - V_h^\star\|_\infty, \|V_h^{\mu,\dagger} - V_h^\star\|_\infty } \le \sum_{h'=h}^H\epsilon_{h'}.
% \end{align*}
% \begin{proof}
% The proof is a direct corollary from Lemma \ref{lemma:up-low-sandwich} and Lemma \ref{lem:duality}.

% From \ref{lem:duality} we know that
% \begin{align*}
%     \max\set{ \|V_h^{\dagger,\nu} - V_h^\star\|_\infty, \|V_h^{\mu,\dagger} - V_h^\star\|_\infty } \le \sum_{h'=h}^H \max_{s} \max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB} \left(\brac{(\mu^\dagger)^\top \up Q_h^\star \nu_h}(s)- \brac{\mu_h^\top \low Q_h^\star \nu^\dagger}(s)\right)
% \end{align*}
% \end{proof}
% \end{lemma}

Throughout the rest of this section, we define the following shorthand for the gap between $\up Q_h^t, \low Q_h^t$ defined in \eqref{eq:up-Q}:
\begin{equation*}
    \delta_h^t := \|\up Q_h^t - \low Q_h^t\|_\infty = \max_{s,a,b}\up Q_h^t(s,a,b) - \low Q_h^t(s,a,b),
\end{equation*}
\begin{lemma}[Recursion of $\delta_h^t$]
Algorithm \ref{algorithm:modified-oftrl-q} guarantees that for all $(t,h)\in[T]\times[H]$,
\begin{align*}
    \delta_h^t \le \sum_{i=1}^t \alpha_t^i \delta_{h+1}^i + \reg_{h+1,\mu+\nu}^t.
\end{align*}
Further, suppose that $\reg_{h,\mu+\nu}^t\le \barreg_{h,\mu+\nu}^t$ for all $(h,t)\in[H]\times[T]$, where $\barreg_{h,\mu+\nu}^t$ is non-increasing in $t$: $\barreg_{h,\mu+\nu}^t\ge \barreg_{h,\mu+\nu}^{t+1}$ for all $t\ge 1$. Then we have
\begin{align*}
    \delta_h^t \le 2H\cdot\frac{1}{t}\sum_{i=1}^t\max_{h'}\barreg_{h',\mu+\nu}^i.
\end{align*}
\begin{proof}The proof structure resembles Lemma \ref{lemma:recursion-of-value-estimation}. From the definition of $\up Q_h^t, \low Q_h^t$, we have that
\begin{align*}
    \up Q_h^t(s,a,b) - \low Q_h^t(s,a,b) &\le \P_h\max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB}\<\mu^\dagger, \sum_{i=1}^t\alpha_t^i \up Q_{h+1}^i\nu_{h+1}^i\> - \<\nu^\dagger, \sum_{i=1}^t\alpha_t^i(\low Q_{h+1}^i)^\top\mu_{h+1}^i\>\\
    &= \P_h\left[\max_{\mu^\dagger\in\Delta_\cA}\<\mu^\dagger, \sum_{i=1}^t\alpha_t^i \up Q_{h+1}^i\nu_{h+1}^i\> - \sum_{i=1}^t\alpha_t^i (\mu_{h+1}^i)^\top\up Q_{h+1}^i \nu_{h+1}^i\right.\\
    &+ \max_{\nu^\dagger\in\Delta_\cB} \sum_{i=1}^t\alpha_t^i (\mu_{h+1}^i)^\top\up Q_{h+1}^i \nu_{h+1}^i - \<\nu^\dagger, \sum_{i=1}^t\alpha_t^i(\low Q_{h+1}^i)^\top\mu_{h+1}^i\>\\
    &+ \sum_{i=1}^t\alpha_t^i (\mu_{h+1}^i)^\top\up Q_{h+1}^i \nu_{h+1}^i - \sum_{i=1}^t\alpha_t^i (\mu_{h+1}^i)^\top\up Q_{h+1}^i \nu_{h+1}^i \\
    &\le \reg_{h+1,\mu+\nu}^t + \sum_{i=1}^t\alpha_t^i \|\up Q_{h+1}^i-\low Q_{h+1}^i\|_\infty= \sum_{i=1}^t\alpha_t^i\delta_{h+1}^i + \reg_{h+1,\mu+\nu}^t.
\end{align*}
Then using the same argument as in (cite Lemma C.2), we can consider an auxiliary sequence
\begin{equation}
    \begin{cases}
    \Delta_h^t =  \sum_{i=1}^{t} \alpha_{t}^i \Delta_{h+1}^{i} + \barreg_{h+1,\mu+\nu}^t,\\
    \Delta_{H+1}^t= 0,~ \text{ for all } t.
    \end{cases}
\end{equation}
 Observe that $\{\Delta_h^t \}_{h,t}$ satisfies the following properties 
\begin{equation}
    \begin{cases}
    \Delta_h^t \ge \delta_h^t\qquad &\text{ (by definition)},\\
    \Delta_h^t \le \Delta_h^{t-1} \quad &\text{ (by Lemma \ref{lem:delta.monotonic})}.
    \end{cases}
\end{equation}
Therefore, to control $\delta_h^t$, it suffices to bound $\Delta_h^t\le \frac{1}{t}\sum_{i=1}^t \Delta_h^i$, which follows from the standard argument in \cite{jin2018q}:
\begin{align*}
     \frac{1}{t}\sum_{i=1}^t \Delta_h^i 
     &=  \frac{1}{t}\sum_{i=1}^t  \sum_{j=1}^{i} \alpha_{i}^j \Delta_{h+1}^{j} + \frac{1}{t}\sum_{i=1}^t \barreg_{h+1,\mu+\nu}^i\\
     & \le\frac{1}{t}\sum_{j=1}^{t}\paren{\sum_{i=j}^t\alpha_{i}^j} \Delta_{h+1}^{j} + \frac{1}{t}\sum_{i=1}^t \barreg_{h+1,\mu+\nu}^i\\
     &\le \paren{1+\frac{1}{H}} \cdot \frac{1}{t}\sum_{i=1}^{t}\Delta_{h+1}^{i} + \frac{1}{t}\sum_{i=1}^t \barreg_{h+1,\mu+\nu}^i\\
     &\le \paren{1+\frac{1}{H}}^2 \cdot \frac{1}{t}\sum_{i=1}^{t}\Delta_{h+2}^{i} + \paren{1+\frac{1}{H}}\cdot \frac{1}{t}\sum_{i=1}^t \barreg_{h+2,\mu+\nu}^i +
     \frac{1}{t}\sum_{i=1}^t \barreg_{h+1,\mu+\nu}^i\\
     &\le \cdots\\
     &\le \paren{\sum_{h'=h+1}^{H}\paren{1+\frac{1}{H}}^{h'-h}}\cdot\frac{1}{t}\sum_{i=1}^t \max_{1\le h'\le H}\barreg_{h',\mu+\nu}^i\\
     &\le 2H\cdot \frac{1}{t}\sum_{i=1}^t \max_{1\le h'\le H}\barreg_{h',\mu+\nu}^i,
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

\begin{lemma}[Bound the $\negap$ by $\reg_{h,\mu+\nu}$]\label{lemma:bound-NE-gap-by-regret}
Suppose that the per-state regrets can be upper-bounded as $\reg_{h,\mu+\nu}^t\le \barreg_{h,\mu+\nu}^t$ for all $(h,t)\in [H]\times[T]$ where $\barreg_{h,\mu+\nu}^t$ is non-increasing in $t$: $\barreg_{h,\mu+\nu}^t\ge\barreg_{h,\mu+\nu}^{t+1}$ for all $t\ge 1$. Then, the output policy $(\hat{\mu}^T,\hat{\nu}^T)$ of Algorithm \ref{algorithm:modified-oftrl-q} satisfies
\begin{equation*}
    \negap(\hat{\mu}^T,\hat{\nu}^T)\le 2H\max_h\barreg_{h,\mu+\nu}^T + 24H^2\log T\cdot \frac{1}{T}\sum_{t=1}^T\max_h\barreg_{h,\mu+\nu}^t
\end{equation*}
\begin{proof}
From (Cite Lemma C.1) we have that
\begin{align*}
    & \quad \negap(\hat{\mu}^T,\hat{\nu}^T)=\paren{V_1^{\dagger,\hat{\nu}^T}(s_1) - V_1^\star(s_1)} + \paren{V_1^\star(s_1)- V_1^{\hat{\mu}^T,\dagger}(s_1)}\\
    &\le 2\sum_{h=1}^H \max_s\max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB}\brac{(\mu^\dagger)^\top Q_h^\star \hat\nu_h^T \!-\!\paren{\hat\mu_h^T}^\top Q_h^\star \nu^\dagger }(s)\\
    &= 2\sum_{h=1}^H \max_s\max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB}\sum_{t=1}^T\alpha_T^t\brac{(\mu^\dagger)^\top Q_h^\star \nu_h^t \!-\!\paren{\mu_h^t}^\top Q_h^\star \nu^\dagger }(s)\\
    &\le 2\sum_{h=1}^H \max_s\max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB}\sum_{t=1}^T\alpha_T^t\brac{(\mu^\dagger)^\top \up Q_h^t \nu_h^t \!-\!\paren{\mu_h^t}^\top \low Q_h^t \nu^\dagger}(s)\\
    &\le 2\sum_{h=1}^H \max_s\left(\max_{\mu^\dagger\in\Delta_\cA}\sum_{t=1}^T\alpha_T^t\brac{(\mu^\dagger)^\top \up Q_h^t \nu_h^t \!-\!\paren{\mu_h^t}^\top \up Q_h^t \nu_h^t}(s)\right.\\
    &\qquad \qquad+\left.\max_{\nu^\dagger\in\Delta_\cB}\sum_{t=1}^T\alpha_T^t\brac{(\mu_h^t)^\top \low Q_h^t \nu_h^t \!-\!\paren{\mu_h^t}^\top \low Q_h^t \nu^\dagger}(s)\right)\\
    &+2\sum_{h=1}^H \max_s\max_{\mu^\dagger\in\Delta_\cA,\nu^\dagger\in\Delta_\cB}\sum_{t=1}^T\alpha_T^t\brac{(\mu_h^t)^\top \up Q_h^t \nu_h^t \!-\!\paren{\mu_h^t}^\top \low Q_h^t \nu_h^t}(s)\\
    &\le 2\sum_{h=1}^H\barreg_{h,\mu+\nu}^T + 2\sum_{h=1}^H\sum_{t=1}^T \alpha_T^t\delta_h^t\\
    &\le 2H\max_h\barreg_{h,\mu+\nu}^T + 4H^2\sum_{t=1}^T \alpha_T^t \frac{1}{t}\sum_{i=1}^t \max_h \reg_{h,\mu+\nu}^i \quad \textup{(Lemma \ref{lemma:up-low-sandwich})}\\
    &\le 2H\max_h\barreg_{h,\mu+\nu}^T + 4H^2\paren{\sum_{t=1}^T\frac{1}{t}\alpha_T^t}\paren{\sum_{i=1}^T\max_h\reg_{h,\mu+\nu}^i}\\
    &\le 2H\max_h\barreg_{h,\mu+\nu}^T + 24H^2\log T\cdot \frac{1}{T}\sum_{t=1}^T\max_h\reg_{h,\mu+\nu}^t~~ \textup{(cite Lemma A.3)},
\end{align*}
\end{proof}
\end{lemma}

\begin{lemma}[Bound $\reg_{h,\mu+\nu}^t$]\label{lemma:bound-regret-sum}
Running Algorithm \ref{algorithm:modified-oftrl-q} with $\eta = \frac{1}{16H}$ can guarantee that 
\begin{equation*}
    \reg_{h,\mu+\nu}^T(s) \le \frac{18H^2\log AB}{T}
\end{equation*}
\begin{proof}
From (cite Lemma B.3 in our paper), substituting $g_t = w_t\up Q_h^t\nu_h^t(s), M_t = w_t\up Q_h^{t-1}\nu_h^{t-1}(s), \eta_t = \frac{\eta}{w_t}$, we can get that
\begin{align*}
    &\sum_{t=1}^T w_t\<\mu^\dagger, \up Q_h^t\nu_h^t\> - \<\mu_h^t, \up Q_h^t\nu_h^t\>\le \frac{w_T\log A }{\eta} + \eta\sum_{t=1}^Tw_t\|\up Q_h^t\nu_h^t(s)-\up Q_h^{t-1}\nu_h^{t-1}(s)\|_\infty^2 - \sum_{t=2}^T \frac{w_t}{8\eta}\|\mu_h^t(\cdot|s) - \mu_h^{t-1}(\cdot|s)\|_1^2\\
    &\Longrightarrow ~~\reg_{h,\mu}^T \le \alpha_T^1\sum_{t=1}^T w_{t-1}\<\mu^\dagger, \up Q_h^t\nu_h^t\> - \<\mu_h^t, \up Q_h^t\nu_h^t\>\\
    &\qquad\qquad\quad~ \le \frac{\alpha_T\log A }{\eta} + \eta\sum_{t=1}^T\alpha_T^t\|\up Q_h^t\nu_h^t(s)-\up Q_h^{t-1}\nu_h^{t-1}(s)\|_\infty^2 - \sum_{t=2}^T \frac{\alpha_T^{t-1}}{8\eta}\|\mu_h^t(\cdot|s) - \mu_h^{t-1}(\cdot|s)\|_1^2.
\end{align*}
Further we have that
\begin{align*}
    \|\up Q_h^t\nu_h^t(s)-\up Q_h^{t-1}\nu_h^{t-1}(s)\|_\infty^2 \le 2\|\up Q_h^t-\up Q_h^{t-1}\|_\infty^2 + 2\|\nu_h^t(s)-\nu_h^{t-1}(s)\|_1^2.
\end{align*}
From the definition of $\up Q_h^t$ we have that
\begin{align*}
    \|\up Q_h^t - \up Q_h^{t-1}\| &\le \left\|\sum_{i=1}^t \alpha_t^i \up Q_{h+1}^i \nu_{h+1}^i - \sum_{i=1}^{t-1}\alpha_{t-1}^i \up Q_{h+1}^i \nu_{h+1}^i\right\|_\infty\\
    &= \left\|\alpha_t \up Q_{h+1}^t\nu_{h+1}^t + (1-\alpha_t)\sum_{i=1}^{t-1} \alpha_{t-1}^i \up Q_{h+1}^i \nu_{h+1}^i - \sum_{i=1}^{t-1}\alpha_{t-1}^i \up Q_{h+1}^i \nu_{h+1}^i\right\|_\infty\\
    & = \left\|\alpha_t \up Q_{h+1}^t\nu_{h+1}^t  -\alpha_t\sum_{i=1}^{t-1} \alpha_{t-1}^i \up Q_{h+1}^i \nu_{h+1}^i\right\|_\infty\le \alpha_t H.
\end{align*}
Substitute this inequality to the regret bound we have
\begin{align*}
    \reg_{h,\mu}^T(s) &\le \frac{\alpha_T\log A }{\eta} + 2\eta\sum_{t=1}^T\alpha_T^t \alpha_t^2 H^2 + 2\eta\sum_{t=1}^T\alpha_T^t\|\nu_h^t(s)-\nu_h^{t-1}(s)\|_1^2  - \sum_{t=2}^T \frac{\alpha_T^{t-1}}{8\eta}\|\mu_h^t(\cdot|s) - \mu_h^{t-1}(\cdot|s)\|_1^2\\
    &\le \frac{\alpha_T\log A }{\eta} + \frac{8\eta H^3}{T} + 2\eta\sum_{t=1}^T\alpha_T^t\|\nu_h^t(s)-\nu_h^{t-1}(s)\|_1^2 + - \sum_{t=2}^T \frac{\alpha_T^{t-1}}{8\eta}\|\mu_h^t(\cdot|s) - \mu_h^{t-1}(\cdot|s)\|_1^2. ~~\textup{(cite Lemma A.3)}
\end{align*}
Similar bound holds for $\reg_{h,\nu}^T$:
\begin{equation*}
    \reg_{h,\nu}^T(s)\le \frac{\alpha_T\log B }{\eta} + \frac{8\eta H^3}{T} + 2\eta\sum_{t=1}^T\alpha_T^t\|\mu_h^t(s)-\mu_h^{t-1}(s)\|_1^2 + - \sum_{t=2}^T \frac{\alpha_T^{t-1}}{8\eta}\|\nu_h^t(\cdot|s) - \nu_h^{t-1}(\cdot|s)\|_1^2.
\end{equation*}
Summing $\reg_{h,\mu}^T(s),\reg_{h,\nu}^T(s)$ together we get
\begin{align*}
    \reg_{h,\mu+\nu}^T(s) \le \frac{\alpha_T\log AB}{\eta} + \frac{16\eta H^3}{T} + 16\eta \alpha_T^1 +\sum_{t=2}^T \paren{2\eta\alpha_T^t - \frac{\alpha_T^{t-1}}{8\eta}} \paren{\|\mu_h^t(\cdot|s) - \mu_h^{t-1}(\cdot|s)\|_1^2 + \nu_h^t(\cdot|s) - \nu_h^{t-1}(\cdot|s)\|_1^2}.
\end{align*}
Since $\frac{\alpha_T^{t-1}}{\alpha_T^t} \ge \frac{1}{H}$, by setting $\eta = \frac{1}{16 H}$ we can guarantee that $2\eta\alpha_T^t - \frac{\alpha_T^{t-1}}{8\eta} \le 0$, thus
\begin{align*}
    \reg_{h,\mu+\nu}^T(s) \le \frac{\alpha_T\log AB}{\eta} + \frac{16\eta H^3}{T} + 16\eta \alpha_T^1\le \frac{16H^2 \log AB}{T} + \frac{H^2}{T} + \frac{1}{T}\le \frac{18H^2\log AB}{T}
\end{align*}
\end{proof}
\end{lemma}

Given Lemma \ref{lemma:bound-NE-gap-by-regret} and \ref{lemma:bound-regret-sum}, we can have the following theorem 
\begin{theorem}[Convergence rate for Algorithm \ref{algorithm:modified-oftrl-q}]
Running Algorithm \ref{algorithm:modified-oftrl-q} with $\eta = \frac{1}{16H}$ can guarantee that
\begin{equation*}
    \negap(\hat{\mu}^T,\hat{\nu}^T)\le C\brac{\frac{H^4 \log AB \paren{\log T}^2}{T}},
\end{equation*}
where $C$ is some absolute constant.
\begin{proof}
From Lemma \ref{lemma:bound-NE-gap-by-regret} and \ref{lemma:bound-regret-sum} we have that:
\begin{align*}
        \negap(\hat{\mu}^T,\hat{\nu}^T)&\le 2H\max_h\barreg_{h,\mu+\nu}^T + 24H^2\log T\cdot \frac{1}{T}\sum_{t=1}^T\max_h\barreg_{h,\mu+\nu}^t\\
        &\le 2H\frac{18H^2\log AB}{T} + 24H^2\log T\cdot \frac{1}{T}\sum_{t=1}^T\frac{18H^2\log AB}{t}\\
        &\le \frac{468H^4 \log AB \paren{\log T+1}^2}{T},
\end{align*}
which completes the proof.
\end{proof}
\end{theorem}

==> Sections/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{As this work is primarily theoretical and about understandings, we do not foresee any negative societal impacts of this work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{Our simulations are deterministic.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerYes{}
    %\answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> Sections/framework.tex <==
\section{Algorithm framework for two-player zero-sum Markov Games}


\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^k(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k-1}(s',\cdot,\cdot), \mu_{h+1}^{k-1}(\cdot|s')\times\nu_{h+1}^{k-1}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le k-1}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games \textcolor{red}{(Ver 2)}}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^k(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k-1}(s',\cdot,\cdot), \mu_{h+1}^{k-1}(\cdot|s')\times\nu_{h+1}^{k-1}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games \textcolor{red}{(Ver 3)}}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^k(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{{\color{red} k}}(s',\cdot,\cdot), \mu_{h+1}^{k-1}(\cdot|s')\times\nu_{h+1}^{k-1}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games \textcolor{red}{(Ver 4 $\equiv$ Ver 3, with shifted index)}}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^{k-1}(s,a,b) \setto (1-\alpha_k) Q_h^{k-2}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{{\color{red} k-1}}(s',\cdot,\cdot), \mu_{h+1}^{k-1}(\cdot|s')\times\nu_{h+1}^{k-1}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k-1}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
\textcolor{red}{Runyu: I think Ver 5 is equivalent to Ver 4?}
\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games \textcolor{red}{(Ver 5)}}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k-1}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align}\label{eq:Q-update}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{{\color{red} k}}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


We define the following auxiliary variables:
\begin{align*}
    \alpha_k^t = (1-\alpha_k)(1-\alpha_{k-1})\cdots(1-\alpha_{t+1})\alpha_t
\end{align*}
It is not hard to verify that
\begin{equation*}
    \sum_{t=1}^k \alpha_k^t = 1,
\end{equation*}
and we have that
\begin{align}\label{eq:Q-relationship}
    Q_h^{{\color{red} k-1}}(s,a,b) = \sum_{t=1}^k\alpha_k^t \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t-1}(s',\cdot,\cdot), \mu_{h+1}^{t-1}(\cdot|s')\times\nu_{h+1}^{t-1}(\cdot|s')\>] }(s,a,b) }
\end{align}


Define weighted regret as
\begin{align*}
    & \reg_{h,\mu}^k(s) \defeq \max_{z\in\Delta_\cA} \sum_{t=1}^k \alpha_k^t \< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t-1}(\cdot|s)\> - \sum_{t=1}^k \alpha_k^t \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times \nu_h^{t-1}(\cdot|s)\>, \\
    & \reg_{h,\nu}^k(s) \defeq \sum_{t=1}^k \alpha_k^t \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times \nu_h^{t-1}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \alpha_k^t \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times z\>  \\
    & \reg_h^k \defeq \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\}.
\end{align*}
Consider the value estimation error
\begin{align*}
    \delta_h^k \defeq \linf{ Q_h^k - Q_h^\star } = \max_{s,a,b} \abs{Q_h^k(s,a,b) - Q_h^\star(s,a,b)}.
\end{align*}


\begin{lemma}[Recursion of value estimation, {\color{red} Ver 4}]
We have for all $(k,h)\in[K]\times[H]$ that
\begin{align*}
    \delta_h^{k-1} \le \sum_{t=1}^k \alpha_k^t \delta_{h+1}^{t-1} + \reg_{h+1}^k.
\end{align*}
\end{lemma}
\begin{proof}
From the definition of $Q_h^*$ we have that
\begin{align*}
    Q^*_h(s,a,b) &= r_h(s,a,b) + \max_{\mu_{h+1}}\min_{ \nu_{h+1}} \P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\nu_{h+1}(\cdot|s')\>}(s,a,b)\\
    &\le r_h(s,a,b) + \max_{\mu_{h+1}}\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\paren{\sum_{t=1}^k \alpha_k^t \nu_{h+1}^{t-1}}(\cdot|s')\>}(s,a,b)\\
    &= r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t-1}(\cdot|s')\>}(s,a,b)}\\
    &\le  r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t-1}(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t-1}(\cdot|s')\>}(s,a,b) + \delta_{h+1}^{t-1}}\\
    &\le r_h(s,a,b)+\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t-1}(s',\cdot,\cdot), \mu_{h+1}^{t-1}(\cdot|s')\times \nu_{h+1}^{t-1}(\cdot|s')\>}(s,a,b)} + \reg_{h+1}^k + \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t-1}\\
    &= Q_h^{{\color{red}k-1}}(s,a,b) +\sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t-1}+\reg_{h+1}^k ~~\textup{(From \eqref{eq:Q-relationship})}
\end{align*}
Thus we have that
\begin{equation*}
    Q^*_h(s,a,b) - Q_h^{k-1}(s,a,b) \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t-1}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Apply similar analysis to the minimizing player, we get
\begin{equation*}
      Q_h^{k-1}(s,a,b) -  Q^*_h(s,a,b)  \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t-1}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Thus we get
\begin{equation*}
    \delta_h^{k-1} \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t-1}+\reg_{h+1}^k,
\end{equation*}
which completes the proof.
\end{proof}


Define the state-wise average policy as
\begin{equation*}
    \hat{\mu}_h^k(\cdot|s) := \frac{1}{k}\sum_{t=1}^k\mu_{h}^{t-1}(\cdot|s),\quad 
    \hat{\nu}_h^k(\cdot|s) := \frac{1}{k}\sum_{t=1}^k \nu_h^{t-1}(\cdot|s).
\end{equation*}

\begin{lemma}{\color{red} (This lemma doesn't need to be changed when switching to Alg ver.4)}
Define the unweighted regret as:
\begin{align*}
    & \avgreg_{h,\mu}^k(s) \defeq \frac{1}{k}\max_{z\in\Delta_\cA} \sum_{t=1}^k \< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t-1}(\cdot|s)\> - \sum_{t=1}^k \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times \nu_h^{t-1}(\cdot|s)\>, \\
    & \avgreg_{h,\nu}^k(s) \defeq \frac{1}{k}\sum_{t=1}^k \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times \nu_h^{t-1}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t-1}(\cdot|s)\times z\>  \\
    & \avgreg_h^k \defeq \max_{s\in\cS}( \avgreg_{h,\mu}^k(s)+ \avgreg_{h,\nu}^k(s)).
\end{align*}
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le 2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t-1}
\end{align*}
\begin{proof}
We first give a bound for $\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB} Q_h^*(s,\mu_h^k\times z)$, then we will  apply Lemma \ref{lem.duality} to complete the proof.
\begin{align*}
    &\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB}    Q_h^*(s,\mu_h^k\times z) \\
    &= \max_{z\in\Delta_\cA}\frac{1}{k}\sum_{t=1}^kQ_h^*(s,z\times \nu_h^{t-1}) - \min_{z\in\Delta_\cB} \frac{1}{k}\sum_{t=1}^{k}Q_h^*(s,\mu_h^{t-1}\times z) \\
    &\le \max_{z\in\Delta_\cA}\frac{1}{k}\sum_{t=1}^kQ_h^t(s,z\times \nu_h^{t-1}) - \min_{z\in\Delta_\cB} \frac{1}{k}\sum_{t=1}^{k}Q_h^t(s,\mu_h^{t-1}\times z) + \frac{2}{k}\sum_{t=1}^k\delta_h^{t-1}\\
    &= \avgreg_h^k + \frac{2}{k}\sum_{t=1}^k\delta_h^{t-1}
\end{align*}
Then by applying Lemma \ref{lem.duality}, we have
\begin{align*}
    &\|V_h^{\dagger,\hat{\nu}^k} - V_h^{\hat{\mu}^k,\dagger}\|\le \|V_h^{\dagger,\hat{\nu}^k} - V_h^*\| + \|V_h^*- V_h^{\hat{\mu}^k,\dagger}\|\\
    &\le \sum_{h'=h}^{H}\max_s\max_{z\in\Delta_\cA} \paren{Q_{h'}^*(s,z\times\hat\nu_{h'}^k)- V_{h'}^*(s)} + \sum_{h'=h}^H\max_s\min_{z\in\Delta_\cB}\paren{V_{h'}^*(s) - Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H \max_s\paren{\max_{z\in\Delta_\cA} Q_{h'}^*(s,z\times\hat\nu_{h'}^k) - \min_{z\in\Delta_\cB}Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t-1},
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

\section{Examples}
\subsection{GDA-critic}
\begin{algorithm}[h]
\caption{GDA-critic}
\label{alg:gda.critic-ver2}
\begin{algorithmic}
\STATE \textbf{Initialize:} learning rate $\eta$ and $\{\alpha_k\}_{k=1}^K$, set $V_{i,h}^0(s)=H-h+1$ and $\pi_{i,h}^0(s)$ to be uniform for all $i,h,s$.
\FOR{$k=1,\ldots,K$}
\FOR{$h = H, \ldots, 1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\paren{\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,\cdot,b)}}}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) + \eta\paren{\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,a, \cdot)}}}
\end{align*}
\STATE Update V value for all $s\in\cS$:
\begin{align}\label{eq:V-update}
    V_h^{k}(s) \setto (1-\alpha_k) V_h^{k-1}(s) + \alpha_k \mathbb{E}_{a\sim \mu_h^{k}(\cdot|s), b\sim \nu_h^{k}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k}(s') }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{lemma}
Algorithm \ref{alg:gda.critic-ver2} is equivalent to using the unified framework (Algorithm \ref{alg:framework}) with the $\matrixgamealg$ as
\begin{align*}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}Q_h^{k-1}(s,\cdot,b)}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) + \eta\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)} Q_h^{k-1}(s,a, \cdot)}
\end{align*}
\begin{proof}
We first show that
\begin{equation}\label{eq:relation-Q-V}
    Q_h^{k}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^k(s')}(s,a,b)
\end{equation}
\textcolor{red}{This might not be exactly true... The iteration rule is the same, but initial value might differ. BUt for now let's first assume that}
\begin{equation*}
    Q_h^{0}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^0(s')}(s,a,b),
\end{equation*}
We now prove by induction on both $k$ and $h$. Given that $ Q_h^{0}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^0(s')}(s,a,b)$, it is not hard to verify that $Q_H^{k}(s,a,b) = r_H(s,a,b),~\forall~k\ge 0$. We assume that \eqref{eq:relation-Q-V} holds for $(k-1,h)$ and $(k, h+1)$, then for $(k,h)$, from \eqref{eq:Q-relationship}
\begin{align*}
     Q_h^{k}(s,a,b) &= (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }\\
     &= (1-\alpha_k)\brac{r_h+ \mathbb{P}_hV_{h+1}^{k-1}(s')}(s,a,b)\\
     &+\alpha_k \paren{ \brac{r_h + \P_h[\<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s')}(s,\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) } ~~\textup{(induction assumptions)}\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>\right) }(s,a,b)\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \mathbb{E}_{a\sim\mu_{h+1}^{k}(\cdot|s'), b\sim \nu_{h+1}^{k}(\cdot|s')}\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',a,b)\right) }(s,a,b)\\
     &= \brac{r_h + \mathbb{P}_h V_{h+1}^k(s')}(s,a,b)~~\textup{(from \eqref{eq:V-update})},
\end{align*}
which completes the proof by induction
\end{proof}
\end{lemma}

\begin{lemma}
Set $\alpha_k$ in Algorithm \ref{alg:gda.critic-ver2} as
\begin{equation*}
    \alpha_k = \frac{H+1}{H+k}.
\end{equation*},
then we have that .... \textcolor{blue}{TODO: re-organize Qinghua's proof here}
\end{lemma}

\subsection{Nash V-learning}
\textcolor{blue}{TODO}
\subsection{Nash Q-learning}
\begin{algorithm}[h]
\caption{Nash Q-learning}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \NE(Q_h^{k-1}(s,\cdot,\cdot)).
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{$\alpha_k = 1$}
In this case, we have that $Q_h^k$ equals to $Q_h^{\mu^k\times\nu^k}$.
\begin{lemma}
When $\alpha_k$'s are all set to $\alpha_k = 1$, then we have that for $k \ge H-h+1$,
\begin{equation*}
    Q_h^k(s,a,b) = Q_h^*(s,a,b),~~\forall ~h, ~\forall~s,a,b
\end{equation*}
\begin{proof}
We prove this by induction. For h = H, we have that
\begin{equation*}
    Q_H^{k}(s,a,b) = r_H(s,a,b),~~\forall k \ge 1.
\end{equation*}
Assume that for $h+1$, the condition holds, then for time horizon $h$ and iteration step $k\ge H-h+1$, we have that
\begin{align*}
    Q_h^k(s,a,b) &= \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)
\end{align*}
Additionally, from the induction assumption,
\begin{align*}
    (\mu_{h+1}^k(\cdot|s), \nu_{h+1}^k(\cdot|s)) =  \NE(Q_{h+1}^{k-1}(s,\cdot,\cdot)) = \NE(Q_{h+1}^*(s,\cdot,\cdot)),
\end{align*}
we have that
\begin{align*}
    \<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\> = V_{h+1}^*(s').
\end{align*}
Thus
\begin{align*}
    Q_h^k(s,a,b)
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[V(s')]}(s,a,b) = Q_h^*(s,a,b),
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}
\begin{lemma}
\textcolor{blue}{TODO: bound $\reg_h^k$}
\end{lemma}
\subsection{$\alpha_k = \frac{H+1}{H+k}$}

\subsection{A Counterexample - 'Eager value function'}
In this section, we consider the GDA-critic algorithm (Algorithm \ref{alg:gda.critic-ver2}) with 
\begin{equation*}
    \alpha_k = 1.
\end{equation*}
In this case, $V_h^k$ is the true value function of policy $\mu^k\times \nu^k$. However, although the value function estimation is more accurate in this setting, this actually introduces larger weighted regret $\reg_h^k$ and thus this algorithm no-longer works. \textcolor{blue}{TODO: put our numerical simulation suggesting the problem of this algorithm} Notice that in this setting we can no longer guarantee that the weighted regret $\reg_h^k$'s are small, i.e.,
\begin{align*}
    & \reg_{h,\mu}^k(s) = \max_{z\in\Delta_\cA} \< Q_h^{k-1}(s,\cdot,\cdot), z\times \nu_h^{k-1}(\cdot|s)\> - \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> \sim O(1)\\
    & \reg_{h,\nu}^k(s) = \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> - \min_{z\in\Delta_\cB} \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times z\> \sim O(1) \\
    &\Longrightarrow~~ \reg_h^k = \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\} \sim O(1)
\end{align*}


==> Sections/framework_clean_up.tex <==
\section{Algorithm framework for two-player zero-sum Markov Games}
\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k-1}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align}\label{eq:Q-update}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{{\color{red} k}}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


We define the following auxiliary variables:
\begin{align*}
    \alpha_k^t = (1-\alpha_k)(1-\alpha_{k-1})\cdots(1-\alpha_{t+1})\alpha_t
\end{align*}
It is not hard to verify that
\begin{equation*}
    \sum_{t=1}^k \alpha_k^t = 1,
\end{equation*}
and we have that
\begin{align}\label{eq:Q-relationship}
    Q_h^{k}(s,a,b) = \sum_{t=1}^k\alpha_k^t \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }
\end{align}

From now on, we consider the state-wise average policy (with weight $\beta_k^t$)
\begin{equation*}
    \hat{\mu}_h^k(\cdot|s) :=\sum_{t=1}^k\beta_k^t\mu_{h}^{t}(\cdot|s),\quad 
    \hat{\nu}_h^k(\cdot|s) :=\sum_{t=1}^k\beta_k^t \nu_h^{t}(\cdot|s).
\end{equation*}
Here $\beta_k^t$ needs to satisfy that
\begin{equation*}
    \sum_{t=1}^k \beta_k^t = 1.
\end{equation*}

Define weighted regret with weight $\alpha_k^t$ as
%\textcolor{blue}{[Runyu: I did some index change to match with the algorithm]}
\begin{align*}
    & \reg_{h,\mu}^k(s) \defeq \max_{z\in\Delta_\cA} \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\>, \\
    & \reg_{h,\nu}^k(s) \defeq \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>  \\
    & \reg_h^k \defeq \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\}.
\end{align*}
Define the weighted regret with weight $\beta_k^t$ as:
\begin{align*}
    & \avgreg_{h,\mu}^k(s) \defeq \max_{z\in\Delta_\cA} \sum_{t=1}^k \beta_k^t\< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k\beta_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\>, \\
    & \avgreg_{h,\nu}^k(s) \defeq \sum_{t=1}^k\beta_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k\beta_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>  \\
    & \avgreg_h^k \defeq \max_{s\in\cS}( \avgreg_{h,\mu}^k(s)+ \avgreg_{h,\nu}^k(s)).
\end{align*}

From now on, we assume that exist sequences $\reg^k, \avgreg^k$'s such that
\begin{align*}
    \reg^k \ge \reg_h^k, ~~\forall~ h,k,\\
    \avgreg^k \ge \avgreg_h^k, ~~\forall~ h,k,
\end{align*}
and that $\reg^k, \avgreg^k$'s are non-increasing with respect to $k$.

Consider the value estimation error
\begin{align*}
    \delta_h^k \defeq \linf{ Q_h^k - Q_h^\star } = \max_{s,a,b} \abs{Q_h^k(s,a,b) - Q_h^\star(s,a,b)}.
\end{align*}


\begin{lemma}[Recursion of value estimation]\label{lemma:recursion-of-value-estimation}
We have for all $(k,h)\in[K]\times[H]$ that
\begin{align*}
    \delta_h^{k} \le \sum_{t=1}^k \alpha_k^t \delta_{h+1}^{t} + \reg_{h+1}^k.
\end{align*}
Further, we have that
\begin{equation*}
    \delta_h^k\le \frac{2H}{k}\sum_{t=1}^k\reg^t
\end{equation*}
\end{lemma}
\begin{proof}
From the definition of $Q_h^*$ we have that
\begin{align*}
    Q^*_h(s,a,b) &= r_h(s,a,b) + \max_{\mu_{h+1}}\min_{ \nu_{h+1}} \P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\nu_{h+1}(\cdot|s')\>}(s,a,b)\\
    &\le r_h(s,a,b) + \max_{\mu_{h+1}}\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\paren{\sum_{t=1}^k \alpha_k^t \nu_{h+1}^{t}}(\cdot|s')\>}(s,a,b)\\
    &= r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b)}\\
    &\le  r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b) + \delta_{h+1}^{t}}\\
    &\le r_h(s,a,b)+\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b)} + \reg_{h+1}^k + \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}\\
    &= Q_h^{k}(s,a,b) +\sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k ~~\textup{(From \eqref{eq:Q-relationship})}
\end{align*}
Thus we have that
\begin{equation*}
    Q^*_h(s,a,b) - Q_h^{k}(s,a,b) \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Apply similar analysis to the minimizing player, we get
\begin{equation*}
      Q_h^{k}(s,a,b) -  Q^*_h(s,a,b)  \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Thus we get
\begin{equation*}
    \delta_h^{k} \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,
\end{equation*}
which completes the proof of the first inequality in the Lemma. Now consider an auxiliary sequence 
$\{\Delta_h^k \}_{h,k}$ defined by 
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \reg^k,\\
    \Delta_{H+1}^k= 0 \text{ for all } k.
    \end{cases}
\end{equation}
Observe that $\{\Delta_h^k \}_{h,k}$ satisfies the following properties 
\begin{equation}
    \begin{cases}
    \Delta_h^k \ge \delta_h^k\qquad &\text{ (by definition)},\\
    \Delta_h^k \le \Delta_h^{k-1} \quad &\text{ (by Lemma \ref{lem:delta.monotonic})}.
    \end{cases}
\end{equation}
Therefore, to control $\delta_h^k$, it suffices to bound $\frac{1}{k}\sum_{t=1}^k \Delta_h^t$, which follows from the standard argument in \cite{jin2018q}:
\begin{align*}
     \frac{1}{k}\sum_{t=1}^k \Delta_h^t 
     = & \frac{1}{k}\sum_{t=1}^k  \sum_{j=1}^{t} \alpha_{t}^j \Delta_{h+1}^{j} + \frac{1}{k}\sum_{t=1}^k \reg^t\\
      \le  & \frac{1}{k}  \sum_{j=1}^{k} \left(\sum_{t=j}^k \alpha_{t}^{j}\right) \Delta_{h+1}^{j} + \frac{1}{k}\sum_{t=1}^k \reg^t\\
     \le & \left(1+\frac{1}{H}\right)\frac{1}{k}\sum_{t=1}^k \Delta_{h+1}^t + \frac{1}{k}\sum_{t=1}^k \reg^t\\
     \le & \left(1+\frac{1}{H}\right)^2\frac{1}{k}\sum_{t=1}^k \Delta_{h+2}^t + \left(1+\left(1+\frac{1}{H}\right)\right)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le &\cdots\\
     \le &  \left(\sum_{h=1}^H\left(1+\frac{1}{H}\right)^h\right)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le & H(e-1)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le& \frac{2H}{k}\sum_{t=1}^k \reg^t,
\end{align*}
which completes the proof of the second inequality in the Lemma.
\end{proof}




\begin{lemma}[Policy guarantee]
\label{lemma:NE-gap}
We have
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t. %2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t}
\end{align*}
\begin{proof}
We first give a bound for $\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB} Q_h^*(s,\hat\mu_h^k\times z)$, then we will  apply Lemma \ref{lem.duality} to complete the proof.
\begin{align*}
    &\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB}    Q_h^*(s,\hat\mu_h^k\times z) \\
    &= \max_{z\in\Delta_\cA}\sum_{t=1}^k\beta_k^tQ_h^*(s,z\times \nu_h^{t}) - \min_{z\in\Delta_\cB}\sum_{t=1}^{k}\beta_k^tQ_h^*(s,\mu_h^{t}\times z) \\
    &\le \max_{z\in\Delta_\cA}\sum_{t=1}^k\beta_k^tQ_h^t(s,z\times \nu_h^{t}) - \min_{z\in\Delta_\cB}\sum_{t=1}^{k}\beta_k^tQ_h^t(s,\mu_h^{t}\times z) + \frac{2}{k}\sum_{t=1}^k\delta_h^{t}\\
    &= \avgreg_h^k + \frac{2}{k}\sum_{t=1}^k\delta_h^{t}\\
    &\le \avgreg^k + \frac{2}{k}\sum_{t=1}^k\frac{2H}{t}\sum_{t=1}^j\reg^j~~~\textup{(Lemma \ref{lemma:recursion-of-value-estimation})}\\
    &\le \avgreg^k + \frac{2}{k}\sum_{j=1}^k\paren{\sum_{t=1}^k\frac{2H}{t}}\reg^j\\
    &\le \avgreg^k+\frac{4H\ln(k+1)}{k}\sum_{j=1}^k\reg^j
\end{align*}
Then by applying Lemma \ref{lem.duality}, we have
\begin{align*}
    &\|V_h^{\dagger,\hat{\nu}^k} - V_h^{\hat{\mu}^k,\dagger}\|\le \|V_h^{\dagger,\hat{\nu}^k} - V_h^*\| + \|V_h^*- V_h^{\hat{\mu}^k,\dagger}\|\\
    &\le \sum_{h'=h}^{H}\max_s\max_{z\in\Delta_\cA} \paren{Q_{h'}^*(s,z\times\hat\nu_{h'}^k)- V_{h'}^*(s)} + \sum_{h'=h}^H\max_s\min_{z\in\Delta_\cB}\paren{V_{h'}^*(s) - Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H \max_s\paren{\max_{z\in\Delta_\cA} Q_{h'}^*(s,z\times\hat\nu_{h'}^k) - \min_{z\in\Delta_\cB}Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H\paren{\avgreg^k+\frac{4H\ln(k+1)}{k}\sum_{j=1}^k\reg^j}\\
    &\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{j=1}^k\reg^j,
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

\section{Examples}
\subsection{GDA-critic}
\begin{algorithm}[h]
\caption{GDA-critic}
\label{alg:gda.critic-ver2}
\begin{algorithmic}
\STATE \textbf{Initialize:} learning rate $\eta$ and $\{\alpha_k\}_{k=1}^K$, set $V_{i,h}^0(s)=H-h+1$ and $\pi_{i,h}^0(s)$ to be uniform for all $i,h,s$.
\FOR{$k=1,\ldots,K$}
\FOR{$h = H, \ldots, 1$}
\STATE Update policy for all $s\in\cS$:
\begin{equation}\label{eq:mu-nu-update}
\begin{split}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\paren{\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,\cdot,b)}}}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) - \eta\paren{\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,a, \cdot)}}}
\end{split}
\end{equation}
\STATE Update V value for all $s\in\cS$:
\begin{align}\label{eq:V-update}
    V_h^{k}(s) \setto (1-\alpha_k) V_h^{k-1}(s) + \alpha_k \mathbb{E}_{a\sim \mu_h^{k}(\cdot|s), b\sim \nu_h^{k}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k}(s') }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{lemma}
Algorithm \ref{alg:gda.critic-ver2} is equivalent to using the unified framework (Algorithm \ref{alg:framework}) with the $\matrixgamealg$ as
\begin{align*}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}Q_h^{k-1}(s,\cdot,b)}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) - \eta\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)} Q_h^{k-1}(s,a, \cdot)}
\end{align*}
\begin{proof}
It suffices to show that
\begin{equation}\label{eq:relation-Q-V}
    Q_h^{k}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^k(s')}(s,a,b)
\end{equation}
It is not hard to verify that
\begin{equation*}
    Q_h^{1}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^1(s')}(s,a,b),
\end{equation*}
We now prove by induction on both $k$ and $h$. Given that $ Q_h^{0}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^0(s')}(s,a,b)$, it is not hard to verify that $Q_H^{k}(s,a,b) = r_H(s,a,b),~\forall~k\ge 0$. We assume that \eqref{eq:relation-Q-V} holds for $(k-1,h)$ and $(k, h+1)$, then for $(k,h)$, from \eqref{eq:Q-relationship}
\begin{align*}
     Q_h^{k}(s,a,b) &= (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }\\
     &= (1-\alpha_k)\brac{r_h+ \mathbb{P}_hV_{h+1}^{k-1}(s')}(s,a,b)\\
     &+\alpha_k \paren{ \brac{r_h + \P_h[\<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s')}(s,\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) } ~~\textup{(induction assumptions)}\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>\right) }(s,a,b)\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \mathbb{E}_{a\sim\mu_{h+1}^{k}(\cdot|s'), b\sim \nu_{h+1}^{k}(\cdot|s')}\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',a,b)\right) }(s,a,b)\\
     &= \brac{r_h + \mathbb{P}_h V_{h+1}^k(s')}(s,a,b)~~\textup{(from \eqref{eq:V-update})},
\end{align*}
which completes the proof by induction
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:reg-h-k-GDA-critic}
Set $\alpha_k$ in Algorithm \ref{alg:gda.critic-ver2} as
\begin{equation*}
    \alpha_k = \frac{H+1}{H+k}.
\end{equation*},
then we have that
\begin{equation*}
    \reg^k = \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta \max\{A,B\}H^2}{2}, \avgreg = \frac{4}{\eta k}+\frac{\eta(A+B)H^2}{2}
\end{equation*}
\begin{proof}
We apply Lemma \ref{lem:gd.regret} to \eqref{eq:mu-nu-update} and we can get an upperbound for both $\reg_{h,\mu}^k, \reg_{h,\nu}^k$:
\begin{align*}
    \reg_{h,\mu^k}&\le \frac{1}{2\eta}\alpha_k^k\max_{z,z'\in\Delta_\cA}\|z-z'\|^2 + \frac{\eta AH^2}{2}\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta AH^2}{2}\\
    \reg_{h,\nu^k}&\le \frac{1}{2\eta}\alpha_k^k\max_{z,z'\in\Delta_\cB}\|z-z'\|^2 + \frac{\eta BH^2}{2}\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta BH^2}{2},\\
    \Longrightarrow\quad \reg_h^k &\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta \max\{A,B\}H^2}{2}.
\end{align*}
Similarly,
\begin{align*}
    \avgreg_{h,\mu^k}&\le \frac{1}{2\eta k}\max_{z,z'\in\Delta_\cA}\|z-z'\|^2 + \frac{\eta AH^2}{2}\le \frac{2}{\eta k} + \frac{\eta AH^2}{2}\\
    \avgreg_{h,\nu^k}&\le \frac{1}{2\eta k}\max_{z,z'\in\Delta_\cB}\|z-z'\|^2 + \frac{\eta BH^2}{2}\le \frac{2}{\eta k} + \frac{\eta BH^2}{2},\\
    \Longrightarrow\quad \avgreg_h^k &\le \frac{4}{\eta k} + \frac{\eta (A+B)H^2}{2} .
\end{align*}
\end{proof}
\end{lemma}

\begin{theorem}\label{thm:2p0s}
For all $(i,h)\in[2]\times[H]$, 
$$
\|V_{i,h}^{\dagger,\hat\pi_{-i}^k} - V_{i,h}^\star \|_\infty\le 
6\eta\max\{A,B\}H^4 + \frac{32H^3\left(\ln(H+k)^2 + 1\right)}{\eta k}.
$$
\begin{proof}
From Lemma \ref{lemma:NE-gap} and Lemma \ref{lemma:reg-h-k-GDA-critic} we have that
\begin{align*}
     \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
     &\le 2H\paren{ \frac{4}{\eta k} + \frac{\eta (A+B)H^2}{2}} + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{2}{\eta}\frac{H+1}{H+t} + \frac{\eta \max\{A,B\}H^2}{2}}\\
     &\le \frac{8H}{\eta k}+{\eta (A+B)H^3} +\frac{32H^3\ln(H+k)\ln(k+1)}{\eta k} + {4\eta\max\{A,B\}H^4}\\
     &\le 6\eta\max\{A,B\}H^4 + \frac{32H^3\left(\ln(H+k)^2 + 1\right)}{\eta k}
\end{align*}
\end{proof}
\end{theorem}

\subsection{Nash V-learning (full feedback)}
\begin{prop}
V-learning (with full feedback) is equivalent to using the unified framework (Algorithm \ref{alg:framework}) with the $\matrixgamealg$ as
\begin{align*}
    \mu_h^k(a|s)& \propto \exp\paren{\frac{\eta}{w_{k-1}}\sum_{t=1}^{k-1}\mathbb{E}_{b\sim \nu_h^{t}(\cdot|s)}w_tQ_h^{t}(s,a,b)}\\
    \nu_h^k(b|s)&\propto\exp\paren{ - \frac{\eta}{w_{k-1}}\sum_{t=1}^k\mathbb{E}_{a\sim \mu_h^{t}(\cdot|s)} w_t Q_h^{t}(s,a, b)}
\end{align*}
where $w_k = \frac{\alpha_k}{\alpha_k^1}$, and $\alpha_k$ set as $\alpha_k = \frac{H+1}{H+k}$.
\end{prop}

\begin{lemma}\label{lemma:reg-V-learning}
Set $\beta_k^t = \alpha_k^t$, we have that
\begin{equation*}
    \reg^k = \frac{(H+1)\log A}{\eta k} + \frac{\eta H^2}{2}, ~~\avgreg^k = 2\reg^k
\end{equation*}
\begin{proof}
From Lemma \ref{lemma:FTRL} we have that
\begin{align*}
    \max_{z\in\Delta_\cA} \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\>\le \frac{w_{k+1}}{\eta}\log A + \frac{\eta H^2}{2}\sum_{t=1}^k w_t
\end{align*}
Further, it is not hard to verify that $\alpha_k^t = w_t \cdot \alpha_k^1$ for $1\le t\le k$,  thus we have
\begin{align*}
    \reg^k &= \alpha_k^1\paren{\frac{w_{k+1}}{\eta}\log A + \frac{\eta H^2}{2}\sum_{t=1}^k w_t}\\
    &=\frac{\alpha_k^1w_{k+1}}{\eta}\log A + \frac{\eta H^2}{2}\sum_{t=1}^k \alpha_k^t\\
    &= \frac{\alpha_{k+1}}{1-\alpha_{k+1}}\frac{1}{\eta}\log A + \frac{\eta H^2}{2}\\
    &= \frac{(H+1)\log A}{\eta k} + \frac{\eta H^2}{2}
\end{align*}
\end{proof}
\end{lemma}
\begin{theorem}
For Nash V-learning (with full feedback), 
\begin{equation*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le 6\eta H^4\ln(k+1) + \frac{16 H^3\paren{\ln(k+1)^2 + 1}\log A}{k\eta}
\end{equation*}
\begin{proof}
From Lemma \ref{lemma:NE-gap} and Lemma \ref{lemma:reg-V-learning}, we have
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty &\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
    &= 4H\paren{\frac{(H+1)\log A}{\eta k} + \frac{\eta H^2}{2}} + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \paren{\frac{(H+1)\log A}{\eta t} + \frac{\eta H^2}{2}}\\
    &\le 6\eta H^4\ln(k+1) + \frac{16 H^3\paren{\ln(k+1)^2 + 1}\log A}{k\eta}
\end{align*}
\end{proof}
\end{theorem}
\yub{State-wise averaging guarantee}

\subsection{OFTRL $T^{-3/4}$ analysis}
In this section we consider Algorithm \ref{alg:framework} with $\alpha_k = \frac{H+1}{H+k}$ and \matrixgamealg as 
\begin{align*}
    \mu_h^k(\cdot|s)& = \argmax_{\mu}\<\mu, \sum_{t=1}^{k-1}w_t\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) + w_k\E_{b\sim\nu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,\cdot,b)\> - \frac{w_k}{\eta}H(\mu)\\
    \nu_h^k(\cdot|s) &= \argmin_{\nu}\<\nu, \sum_{t=1}^{k-1}w_t\E_{a\sim\mu_h^t(\cdot|s)}Q_h^t(s,a,\cdot) + w_k\E_{a\sim\mu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,\cdot)\> + \frac{w_k}{\eta}H(\nu)\\
    \Longleftrightarrow~~ \mu_h^k(a|s)&\propto \exp\paren{\frac{\eta}{w_k}\sum_{t=1}^{k-1}w_t\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,a,b) + w_k\E_{b\sim\nu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,b)}\\
    \nu_h^k(b|s)&\propto\exp\paren{-\frac{\eta}{w_k}\sum_{t=1}^{k-1}w_t\E_{a\sim\mu_h^t(\cdot|s)}Q_h^t(s,a,b) + w_k\E_{a\sim\mu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,b)}
\end{align*}

\begin{lemma}\label{lemma:OFTRL-reg}
Set $\beta_k^t = \alpha^t$, the for OFTRL algorithm we have
\begin{equation*}
    \reg^k = \frac{H+1}{k\eta} + \frac{2\eta(H+1)^3}{k} + 32\eta^3 H^4,\quad \avgreg^k = 2\reg^k
\end{equation*}
\begin{proof}
From Lemma \ref{lemma:OFTRL-auxillary}, we have that
\begin{align*}
     \max_{z\in\Delta_\cA} \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> \\
     \le \frac{w_{k+1}}{\eta} + \sum_{t=1}^k \frac{\eta}{w_t} w_t^2\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty^2. 
\end{align*}
\begin{align*}
    \reg_{h,\mu}^k(s) &= \alpha_k^1 \max_{z\in\Delta_\cA} \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> \\
    &\le \frac{\alpha_{k+1}}{(1-\alpha_{k+1})\eta} + \eta \sum_{t=1}^k \alpha_k^t\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty^2\\
    &\le \frac{H+1}{k\eta} + \eta \sum_{t=1}^k \alpha_k^t\left(\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty \right.\\
    &\qquad\qquad \qquad + \left. \left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^{t-1}(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty\right)^2\\
    &\le \frac{H+1}{k\eta} + \eta \sum_{t=1}^k \alpha_k^t\paren{\|Q_h^t - Q_h^{t-1}\|_\infty + H\|\nu_h^{t}(\cdot|s) -\nu_h^{t-1}(\cdot|s)\|_1}^2\\
    &\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty^2 + 2\eta H^2\sum_{t=1}^k\alpha_k^t\|\nu_h^t(\cdot|s)-\nu_h^{t-1}(\cdot|s)\|_1^2\\
    &\textup{\textcolor{blue}{TODO: check whether the bound can be better if we reweight the $H$-factor of the two terms.}}\\
    &\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2+ 32\eta^3 H^4 \quad \textup{(Lemma \ref{lemma:mu-nu-total-variation-bound})}
\end{align*}
Based on the update of $Q_h^t$, we have
\begin{align*}
    |Q_h^t(s,a,b) - Q_h^{t-1}(s,a,b)| = \left|\alpha_t\paren{[r_h + \P_h[\<Q_{h+1}^t(s',\cdot,\cdot),\mu_{h+1}^t(\cdot|s')\times\nu_{h+1}^t(\cdot|s)\>]](s,a,b)} - \alpha_t Q_h(s,a,b)\right| \le \alpha_t H, 
\end{align*}
thus we get that
\begin{align*}
    \sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2 &\le  \sum_{t=1}^k\alpha_k^t\alpha_t^2 H^2 \le \frac{(H+1)^3}{k}\quad \textup{(Lemma \ref{lemma:bound-A-k})}
\end{align*}
Substituting this bound to the above inequality we get that
\begin{align*}
    \reg_{h,\mu}^k(s)\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2+ 32\eta^3 H^4\le \frac{H+1}{k\eta} + \frac{2\eta(H+1)^3}{k} + 32\eta^3 H^4.
\end{align*}
The same bound also holds for $\reg_{h,\nu}^k(s)$, which completes the proof.
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:NE-gap-OFTRL}
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le \frac{12(H+1)^3\ln(k+1)^2}{k\eta} + \frac{24(H+1)^5\ln(k+1)^2}{k}\eta + 384\eta^3H^6\ln(k+1)
\end{align*}
\begin{proof}
From Lemma \ref{lemma:NE-gap} we have
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t \le \frac{12H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
    &=\frac{12H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{H+1}{t\eta} + \frac{2\eta(H+1)^3}{t} + 32\eta^3 H^4}\\
    &\le \frac{12(H+1)^3\ln(k+1)^2}{k\eta} + \frac{24(H+1)^5\ln(k+1)^2}{k}\eta + 384\eta^3H^6\ln(k+1)
    %2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t}
\end{align*}
\end{proof}
\end{lemma}









\subsection{OFTRL $T^{-5/6}$ analysis}
In this section we consider Algorithm \ref{alg:framework} with $\alpha_k = \frac{H+1}{H+k}$ and \matrixgamealg as 
\begin{align*}
    \mu_h^k(\cdot|s)& = \argmax_{\mu}\<\mu, \sum_{t=1}^{k-1}w_t\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) + w_k\E_{b\sim\nu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,\cdot,b)\> - \frac{w_k}{\eta}H(\mu)\\
    \nu_h^k(\cdot|s) &= \argmin_{\nu}\<\nu, \sum_{t=1}^{k-1}w_t\E_{a\sim\mu_h^t(\cdot|s)}Q_h^t(s,a,\cdot) + w_k\E_{a\sim\mu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,\cdot)\> + \frac{w_k}{\eta}H(\nu)\\
    \Longleftrightarrow~~ \mu_h^k(a|s)&\propto_a \exp\paren{\frac{\eta}{w_k}\sum_{t=1}^{k-1}w_t\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,a,b) + w_k\E_{b\sim\nu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,b)}\\
    \nu_h^k(b|s)&\propto_b\exp\paren{-\frac{\eta}{w_k}\sum_{t=1}^{k-1}w_t\E_{a\sim\mu_h^t(\cdot|s)}Q_h^t(s,a,b) + w_k\E_{a\sim\mu_h^{k-1}}(\cdot|s)Q_h^{k-1}(s,a,b)}
\end{align*}

\begin{lemma}\label{lemma:OFTRL-reg}
Set $\beta_k^t = \alpha^t$, the for OFTRL algorithm we have
\begin{equation*}
    \reg^k = \frac{H+1}{k\eta} + \frac{2\eta(H+1)^3}{k} + 32\eta^3 H^4,\quad \avgreg^k = 2\reg^k
\end{equation*}
\begin{proof}

\yub{to be updated.}
Our matrix game algorithm is equivalent to the OFTRL algorithm 

Lemma \ref{lemma:OFTRL-auxillary}, 


we have that
\begin{align*}
     & \quad \max_{z\in\Delta_\cA} \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> \\
     & \le \frac{\log A\cdot w_{k+1}}{\eta} + \sum_{t=1}^k \frac{\eta}{w_t} w_t^2\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty^2. 
\end{align*}
\begin{align*}
    \reg_{h,\mu}^k(s) &= \alpha_k^1 \max_{z\in\Delta_\cA} \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k w_t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> \\
    &\le \frac{\alpha_{k+1}}{(1-\alpha_{k+1})\eta} + \eta \sum_{t=1}^k \alpha_k^t\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty^2\\
    &\le \frac{H+1}{k\eta} + \eta \sum_{t=1}^k \alpha_k^t\left(\left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^t(s,\cdot,b) - \E_{b\sim\nu_h^{t}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty \right.\\
    &\qquad\qquad \qquad + \left. \left\|\E_{b\sim\nu_h^t(\cdot|s)}Q_h^{t-1}(s,\cdot,b) - \E_{b\sim\nu_h^{t-1}(\cdot|s)}Q_h^{t-1}(s,\cdot,b)\right\|_\infty\right)^2\\
    &\le \frac{H+1}{k\eta} + \eta \sum_{t=1}^k \alpha_k^t\paren{\|Q_h^t - Q_h^{t-1}\|_\infty + H\|\nu_h^{t}(\cdot|s) -\nu_h^{t-1}(\cdot|s)\|_1}^2\\
    &\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty^2 + 2\eta H^2\sum_{t=1}^k\alpha_k^t\|\nu_h^t(\cdot|s)-\nu_h^{t-1}(\cdot|s)\|_1^2\\
    &\textup{\textcolor{blue}{TODO: check whether the bound can be better if we reweight the $H$-factor of the two terms.}}\\
    &\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2+ 32\eta^3 H^4 \quad \textup{(Lemma \ref{lemma:mu-nu-total-variation-bound})}
\end{align*}
Based on the update of $Q_h^t$, we have
\begin{align*}
    |Q_h^t(s,a,b) - Q_h^{t-1}(s,a,b)| = \left|\alpha_t\paren{[r_h + \P_h[\<Q_{h+1}^t(s',\cdot,\cdot),\mu_{h+1}^t(\cdot|s')\times\nu_{h+1}^t(\cdot|s)\>]](s,a,b)} - \alpha_t Q_h(s,a,b)\right| \le \alpha_t H, 
\end{align*}
thus we get that
\begin{align*}
    \sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2 &\le  \sum_{t=1}^k\alpha_k^t\alpha_t^2 H^2 \le \frac{(H+1)^3}{k}\quad \textup{(Lemma \ref{lemma:bound-A-k})}
\end{align*}
Substituting this bound to the above inequality we get that
\begin{align*}
    \reg_{h,\mu}^k(s)\le \frac{H+1}{k\eta} + 2\eta\sum_{t=1}^k\alpha_k^t \|Q_h^t - Q_h^{t-1}\|_\infty^2+ 32\eta^3 H^4\le \frac{H+1}{k\eta} + \frac{2\eta(H+1)^3}{k} + 32\eta^3 H^4.
\end{align*}
The same bound also holds for $\reg_{h,\nu}^k(s)$, which completes the proof.
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:NE-gap-OFTRL}
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le \frac{12(H+1)^3\ln(k+1)^2}{k\eta} + \frac{24(H+1)^5\ln(k+1)^2}{k}\eta + 384\eta^3H^6\ln(k+1)
\end{align*}
\begin{proof}
From Lemma \ref{lemma:NE-gap} we have
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t \le \frac{12H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
    &=\frac{12H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{H+1}{t\eta} + \frac{2\eta(H+1)^3}{t} + 32\eta^3 H^4}\\
    &\le \frac{12(H+1)^3\ln(k+1)^2}{k\eta} + \frac{24(H+1)^5\ln(k+1)^2}{k}\eta + 384\eta^3H^6\ln(k+1)
    %2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t}
\end{align*}
\end{proof}
\end{lemma}



\subsection{Nash Q-learning (full feedback)}
\begin{algorithm}[h]
\caption{Nash Q-learning}
\label{alg:Nash-Q}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \NE(Q_h^{k-1}(s,\cdot,\cdot)).
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{$\alpha_k = 1$}
In this case, we have that $Q_h^k$ equals to $Q_h^{\mu^k\times\nu^k}$.
\begin{lemma}
When $\alpha_k$'s are all set to $\alpha_k = 1$, then we have that for $k \ge H-h+1$,
\begin{equation*}
    Q_h^k(s,a,b) = Q_h^*(s,a,b),~~\forall ~h, ~\forall~s,a,b
\end{equation*}
\begin{proof}
We prove this by induction. For h = H, we have that
\begin{equation*}
    Q_H^{k}(s,a,b) = r_H(s,a,b),~~\forall k \ge 1.
\end{equation*}
Assume that for $h+1$, the condition holds, then for time horizon $h$ and iteration step $k\ge H-h+1$, we have that
\begin{align*}
    Q_h^k(s,a,b) &= \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)
\end{align*}
Additionally, from the induction assumption,
\begin{align*}
    (\mu_{h+1}^k(\cdot|s), \nu_{h+1}^k(\cdot|s)) =  \NE(Q_{h+1}^{k-1}(s,\cdot,\cdot)) = \NE(Q_{h+1}^*(s,\cdot,\cdot)),
\end{align*}
we have that
\begin{align*}
    \<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\> = V_{h+1}^*(s').
\end{align*}
Thus
\begin{align*}
    Q_h^k(s,a,b)
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[V(s')]}(s,a,b) = Q_h^*(s,a,b),
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}
\begin{lemma}
\textcolor{blue}{TODO: bound $\reg_h^k$}
\end{lemma}
\subsection{$\alpha_k = \frac{H+1}{H+k}$}
\begin{lemma}\label{lemma:reg-Nash-Q}
For Algorithm \ref{alg:Nash-Q} with $\alpha_k = \frac{H+1}{H+k}$, we have that 
\begin{equation*}
    \reg^k = \frac{(H+1)^2}{H+k} ,~~~~\avgreg_h^k =\frac{2H^2\ln(H+k)}{k}
\end{equation*}
\begin{proof}
\begin{align*}
    &\reg_{h,\mu}^k(s)+\reg_{h,\nu}^k(s) = \max_{z\in\Delta_\cA} \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\> \\
    &~~\le \sum_{t=1}^k  \alpha_k^t \left(\max_{z\in\Delta_\cA}\< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> -\min_{z\in\Delta_\cB} \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\> \right)+ 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty\\
    &~~\le 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty.\\
    &\avgreg_{h,\mu^k} + \avgreg_{h,\nu^k} = \frac{1}{k}\max_{z\in\Delta_\cA} \sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\>- \min_{z\in\Delta_\cB}\sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>\\
    &~~\le \frac{1}{k} \sum_{t=1}^k \left(\max_{z\in\Delta_\cA}\< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\>- \min_{z\in\Delta_\cB}\< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>\right) + \frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty\\
    &~~\le\frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty.
\end{align*}
Thus
\begin{equation*}
    \reg_h^k \le 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty,\quad \avgreg_h^k \le \frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty.
\end{equation*}
Since
\begin{align*}
    &Q_h^{t}(s,a,b) = (1-\alpha_t) Q_h^{t-1}(s,a,b) + \alpha_t \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }\\
    \Longrightarrow & |Q_h^{t}(s,a,b) -  Q_h^{t-1}(s,a,b)|\le \alpha_t |Q_h^{t-1}(s,a,b) - \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }|
    \le \alpha_t H\\
    \Longrightarrow&\|Q_h^{t}-Q_h^{t-1}\|_\infty\le \alpha_t H ,
\end{align*}
substituting this into the above equations we have that
\begin{equation*}
    \reg_h^k \le H \sum_{t=1}^k \alpha_k^t \alpha_t,~~~~\avgreg_h^k \le\frac{H}{k} \sum_{t=1}^k\alpha_t \le\frac{2H^2\ln(H+k)}{k}
\end{equation*}
we now further bound $\reg_h^k$. Define $x_k:= \sum_{t=1}^k \alpha_k^t \alpha_t$. From the definition of $x_k$ we have that~\yub{check}
\begin{align*}
    &x_{k+1} =  \sum_{t=1}^{k+1} \alpha_{k+1}^t \alpha_t = \sum_{t=1}^k (1-\alpha_{k+1})\alpha_k^t\alpha_t + \alpha_{k+1}^2 = (1-\alpha_{k+1}^t)x_k + \alpha_{k+1}\\
    \Longrightarrow ~~&x_{k+1} = \frac{k}{H+k+1}x_k + \frac{(H+1)^2}{(H+k+1)^2}\le \frac{k}{H+k+1}x_k  + \frac{(H+1)^2}{(H+k+1)(H+k)}\\
    \Longrightarrow ~~&\paren{x_{k+1} - \frac{(H+1)^2}{H(H+k+1)}}\le\frac{k}{H+k+1} \paren{x_{k+1} - \frac{(H+1)^2}{H(H+k)}}.
\end{align*}
Since $x_1 = \alpha_1^2 = 1\le \frac{(H+1)^2}{H(H+2)}$, we have that $x_k \le \frac{(H+1)^2}{H(H+k)} $, which completes the proof.
\end{proof}
\end{lemma}
\begin{theorem}\label{thm:Nash-Q}
For all $(i,h)\in[2]\times[H]$, 
$$
\|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger} \|_\infty\le 
\frac{32H^4\left(\ln(H+k)^2+1\right)}{k}.
$$
\begin{proof}
From Lemma \ref{lemma:NE-gap} and Lemma \ref{lemma:reg-Nash-Q} we have that
\begin{align*}
     \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
     &\le 2H\paren{\frac{2H^2\ln(H+k)}{k}} + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{(H+1)^2}{H+k}}\\
     &\le \frac{4H^3\ln(H+k)}{k} +\frac{32H^4\ln(H+k)^2}{k}\\
     &\le \frac{32H^4\left(\ln(H+k)^2+1\right)}{k}
\end{align*}
\end{proof}
\end{theorem}


\subsection{A Counterexample - 'Eager value function'}
In this section, we consider the GDA-critic algorithm (Algorithm \ref{alg:gda.critic-ver2}) with 
\begin{equation*}
    \alpha_k = 1.
\end{equation*}
In this case, $V_h^k$ is the true value function of policy $\mu^k\times \nu^k$. However, although the value function estimation is more accurate in this setting, this actually introduces larger weighted regret $\reg_h^k$ and thus this algorithm no-longer works. \textcolor{blue}{TODO: put our numerical simulation suggesting the problem of this algorithm} Notice that in this setting we can no longer guarantee that the weighted regret $\reg_h^k$'s are small, i.e.,
\begin{align*}
    & \reg_{h,\mu}^k(s) = \max_{z\in\Delta_\cA} \< Q_h^{k-1}(s,\cdot,\cdot), z\times \nu_h^{k-1}(\cdot|s)\> - \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> \sim O(1)\\
    & \reg_{h,\nu}^k(s) = \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> - \min_{z\in\Delta_\cB} \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times z\> \sim O(1) \\
    &\Longrightarrow~~ \reg_h^k = \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\} \sim O(1)
\end{align*}


\section{Auxillaries}
\subsection{Auxiliary lemma for gradient descent}
To begin with, we derive a weighted regret bound for gradient descent. 

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Initialize} $x_1\in\cX$
\FOR{$t=1,\ldots,T$}
\STATE $y_{t+1} = x_t - \eta g_t$
\STATE $x_{t+1} = \cP_\cX( y_{t+1}) $
\ENDFOR
\end{algorithmic}
\end{algorithm}

For simplicity of notation, denote the diameter of $\cX$ by $R$ and $G=\max_{t\in[T]}\|g_t\|_2$.

\begin{lemma}\label{lem:gd.regret}
 For any $z\in\cX$ and $\mathbf{w}\in\Delta_T$ satisfying $w_{t+1}\ge w_t$ for $t\in[T-1]$, we have
$$
 \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le \frac{1}{2\eta} w_T R^2  + \frac{\eta G^2}{2}.
$$
\end{lemma}
\begin{proof}
By following the standard GD analysis, we first have
%~\yub{$1/\eta$ should be $1/(2\eta)$?}
\begin{align*}
    \langle x_t -z, g_t\rangle =& \frac{1}{\eta} \langle x_t -z, x_t - y_{t+1}\rangle \\
    = & \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-y_{t+1}\|^2 \right]\\
    \le& \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-x_{t+1}\|^2 \right]\\
    = &\frac{1}{2\eta} \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right],
\end{align*}
where the inequality follows from $z\in\cX$ and $x_{t+1} = \cP_\cX( y_{t+1})$. By multiplying both sides with $w_t$ and taking summation over $t\in[T]$, we have
\begin{align*}
   \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le & \frac{1}{2\eta}\sum_{t=1}^T  w_t  \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right]\\
   \le  &\frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t)\|z-x_{t+1}\|^2
   + w_1 \|x_1 - z\|^2 + \frac{ \eta G^2}{2}\\
   \le & \frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t) R^2 + w_1 R^2 + \frac{ \eta G^2}{2} = \frac{1}{2\eta} w_T R^2  +\frac{ \eta G^2}{2},
\end{align*}
where the second inequality uses $\w\in\Delta_{T}$ and the third one uses $w_{t+1}\ge w_t$.
\end{proof}
\subsection{Auxiliary lemma for FTRL}
In this subsection, we consider the following FTRL algorithm. Here we assume that vectors $x_t$'s lie inside a probability simplex $\Delta_\cA$, i.e., $\sum_{a\in\cA} x_t(a) = 1, x_t(a)\ge 0, \forall a\in \cA$, here the notation $x_t(a)$ represents the $a$-th entry of $x_t$.  
\begin{algorithm}[h]\label{alg:FTRL}
\begin{algorithmic}
\STATE \textbf{Initialize} $x_1\in\Delta_\cA$
\FOR{$t=1,\ldots,T$}
\STATE 
\vspace{-20pt}
\begin{align*}
    x_{t+1}&\setto \argmin_{x\in\Delta_\cA} \sum_{s=1}^t w_s \<x,g_s\> - \frac{w_t}{\eta} H(x)\\
    \Longrightarrow~~ &x_{t+1}(a)\propto \exp\paren{-\frac{\eta}{w_t}\sum_{s=1}^t w_sg_s(a)}
\end{align*}
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{lemma}\label{lemma:FTRL}
For weights $\{w_t\}$'s that satisfies $w_{t+1}\ge w_t, ~\forall 1\le t\le T$, running Algorithm \ref{alg:FTRL} with guarantee that
$$
 \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le \frac{w_{T+1}}{\eta}\log(A) + \frac{\eta G^2}{2} \sum_{t=1}^T w_t,
$$
where $G:= \max_{t}\|g_t\|_\infty.$
\begin{proof}
From standard FTRL results (see, e.g., Excercise 28.12 in \cite{lattimore2020bandit}), we have that
\begin{align*}
    \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle &\le \frac{w_{T+1}\max_x H(x)}{\eta} + \sum_{t=1}^Tw_t\paren{\<x_t - x_{t+1}, g_t\> - \frac{w_t \KL(x_{t+1}||x_t)}{\eta}}\\
    &\le \frac{w_{T+1}\log(A)}{\eta} + \sum_{t=1}^T\paren{w_t\<x_t - x_{t+1}, g_t\> - \frac{w_t \|x_t - x_{t+1}\|_1^2}{2\eta}}~~~~\textup{(Pinsker's inequality)}\\
    &\le \frac{w_{T+1}\log(A)}{\eta} + \sum_{t=1}^T \frac{w_t\eta}{2}\|g_t\|_\infty^2\\
    &\le \frac{w_{T+1}\log(A)}{\eta}+\frac{\eta G^2}{2}\sum_{t=1}^Tw_t,
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}


\subsection{Auxiliary lemma for anytime optimistic FTRL}

Define 
\begin{align}
    q_{t+1} = \arg\min_{x\in\Delta_d} \left\langle x, \sum_{s=1}^t g_s \right\rangle + R_t(x)
\end{align}
and 
\begin{align}
\label{equation:oftrl}
    x_{t} = \arg\min_{x\in\Delta_d} \left\langle x, \sum_{s=1}^{t-1} g_s +M_t \right\rangle + R_t(x)
\end{align}
WLOG, we assume $R_t$ always takes nonnegative value for any $t$.~\yub{be careful with this, neg-entropy does not satisfy this. a more general assumption is bounded range and everything still holds, by shifting.}

\begin{lemma}\label{lem:OFTRL-recursion}
For any $T\in\mathbb{N}^+$ and $x\in\Delta_d$,
$$
\sum_{t=1}^{T-1} \langle q_{t+1}, g_t\rangle + \sum_{t=1}^{T-1} \langle x_t - q_{t+1}, M_t\rangle \le \sum_{t=1}^{T-1}\langle x, g_t\rangle + R_T (x) + S_{T-1},
$$
where 
$$
S_{T-1} = 
\sum_{t=1}^{T-1}
\left(R_{t}(q_{t+1})- R_{t+1}(q_{t+1})\right)-
\sum_{t=1}^{T-1} \left(D_{R_t}(q_{t+1},x_t) +  D_{R_t}(x_t,q_t)\right).
$$
\end{lemma}
\begin{proof}
We prove the lemma by induction.
The above relation holds trivially for $T=1$ since $R_1$ is nonnegative. Assume the relation holds for $\tau= T-1$. For $\tau= T$, we have
\begin{equation}
    \begin{aligned}
    &\sum_{t=1}^{T} \langle q_{t+1}, g_t\rangle + \sum_{t=1}^{T} \langle x_t - q_{t+1}, M_t\rangle\\ 
    \le & \min_{x\in\Delta_d}\sum_{t=1}^{T-1}\langle x, g_t\rangle + R_T (x) + S_{T-1}+  \langle q_{T+1}, g_T\rangle +  \langle x_T - q_{T+1}, M_T\rangle \\
    = & \sum_{t=1}^{T-1}\langle q_T, g_t\rangle + R_T (q_T) + S_{T-1}+  \langle q_{T+1}, g_T\rangle +  \langle x_T - q_{T+1}, M_T\rangle \quad \mbox{(by the definition of $q_T$)}\\
    \le &\sum_{t=1}^{T-1}\langle x_T, g_t\rangle + R_T (x_T) - D_{R_T}(x_T,q_T) + S_{T-1}+  \langle q_{T+1}, g_T\rangle +  \langle x_T - q_{T+1}, M_T\rangle \quad \mbox{(by the optimality of $q_T$)}\\
    = &\min_{x\in\Delta_d} \langle x, \sum_{t=1}^{T-1}g_t + M_T\rangle + R_T (x) - D_{R_T}(x_T,q_T) + S_{T-1}+  \langle q_{T+1}, g_T-M_T\rangle  \quad \mbox{(by the definition of $x_T$)} \\
    \le &  \langle q_{T+1}, \sum_{t=1}^{T-1}g_t + M_T\rangle + R_T (q_{T+1}) - D_{R_T}(q_{T+1},x_T)  \\ &\qquad - D_{R_T}(x_T,q_T) + S_{T-1}+  \langle q_{T+1}, g_T-M_T\rangle  \quad \mbox{(by the optimality of $x_T$)} \\
    = &\min_{x\in\Delta_d} \langle x, \sum_{t=1}^{T}g_t\rangle + R_{T+1} (x) + (R_{T}(q_{T+1})- R_{T+1}(q_{T+1})) \\ &\qquad- D_{R_T}(q_{T+1},x_T) -  D_{R_T}(x_T,q_T) + S_{T-1}\quad \mbox{(by the definition of $q_{T+1}$)}, 
    \end{aligned}
\end{equation}
which completes the induction.
\end{proof}

\begin{lemma}\label{lemma:OFTRL-auxillary}
Assume $R$ is $1$-strongly convex w.r.t. $\|\cdot\|_1$ and $R_t =R/\eta_t$ with $\eta_t\ge \eta_{t+1}$  for any $t\in\mathbb{N}^+$. Then for any $T\in\mathbb{N}^+$ and $x\in\Delta_d$,
$$
\sum_{t=1}^T \langle x_t - x, g_t\rangle\le 
R_{T+1}(x)+
\sum_{t=1}^{T} \eta_t \|g_t-M_t\|_\infty^2  -\sum_{t=1}^{T-1} \frac{1}{8\eta_t}\|x_t-x_{t+1}\|_1^2.
$$
\end{lemma}
\begin{proof}
Consider a fixed $T\in\mathbb{N}^+$. 
We first decompose the regret into the following three terms
$$
\sum_{t=1}^T \langle x_t - x, g_t\rangle =
\sum_{t=1}^{T} \langle q_{t+1}-x, g_t\rangle + \sum_{t=1}^{T} \langle x_t - q_{t+1}, M_t\rangle + \sum_{t=1}^{T}\langle x_t-q_{t+1}, g_t-M_t\rangle.
$$
By Lemma \ref{lem:OFTRL-recursion}, we can upper bound the first two terms by $R_{T+1}(x)+S_{T}$ and obtain
\begin{align*}
&\sum_{t=1}^T \langle x_t - x, g_t\rangle \\
\le& R_{T+1}(x)+\sum_{t=1}^{T}
\left(R_{t}(q_{t+1})- R_{t+1}(q_{t+1})\right)+
\sum_{t=1}^{T} \left(\langle x_t-q_{t+1}, g_t-M_t\rangle - D_{R_t}(q_{t+1},x_t) -  D_{R_t}(x_t,q_t)\right)\\
\le &  R_{T+1}(x)+
\sum_{t=1}^{T} \left(\|x_t-q_{t+1}\|_1 \|g_t-M_t\|_\infty - \frac{1}{2\eta_t}\|q_{t+1}-x_t\|_1^2 -  \frac{1}{2\eta_t}\|x_t-q_t\|_1^2\right),
\end{align*}
where the second inequality uses $R_t \le R_{t+1}$ and $R_t$ is $1/\eta_t$ strongly-convex w.r.t. $\|\cdot\|_1$.
Finally, we conclude the proof by applying Cauchy-Schwarz inequality: 
$$
\|x_t-q_{t+1}\|_1 \|g_t-M_t\|_\infty - \frac{1}{4\eta_t}\|q_{t+1}-x_t\|_1^2  \le  \eta_t \|g_t-M_t\|_\infty^2, 
$$
and triangle inequality
$$
- \frac{1}{4\eta_t}\|q_{t+1}-x_t\|_1^2 - \frac{1}{4\eta_{t+1}}\|q_{t+1}-x_{t+1}\|_1^2
\le \frac{1}{8\eta_t}\|x_{t+1}-x_t\|_1^2.
$$
\end{proof}

\begin{lemma}[Bounding stability by the smoothness of loss]
Suppose $R$ has a bounded range $\max_{x\in\Delta_d} R(x) - \min_{x\in\Delta_d} R(x) \le R_0$ for some $R_0\ge 0$, and the learning rate is non-increasing: $\eta_t\ge \eta_{t+1}$ for all $t\ge 1$. Then the OFTRL algorithm~\eqref{equation:oftrl} satisfies
\begin{align*}
    & \quad \sum_{t=2}^{T} \frac{1}{\eta_t} \lone{x_t - x_{t-1}}^2 \le \frac{R_0}{\eta_T} + \max_{x\in\Delta_d} \sum_{t=1}^{T-1} \<x_t - x, g_t\> + \sum_{t=2}^{T} \linf{M_t - M_{t-1}} \\
    & \le \frac{2R_0}{\eta_T} + \sum_{t=1}^{T-1} \eta_t\linf{g_t - M_t}^2 + \sum_{t=2}^{T} \linf{M_t - M_{t-1}}.
\end{align*}
In particular, choosing $M_t=g_{t-1}$ with $g_0\defeq 0$, and assume that $0\le g_t\le G_t$ (in an entry-wise sense) for some $G_t\in\R_{\ge 0}$ such that $G_t\le G_{t+1}$ (non-decreasing) for all $t\ge 1$. Then we have
\begin{align*}
    & \quad \sum_{t=2}^{T} \frac{1}{\eta_t} \lone{x_t - x_{t-1}}^2 \le \frac{2R_0}{\eta_T} + \sum_{t=1}^{T-1} \eta_t\linf{g_t - g_{t-1}}^2 + \sum_{t=2}^{T} \linf{g_{t-1} - g_{t-2}} \\
    & \le \frac{2R_0}{\eta_T} + \sum_{t=1}^{T-1} (1 + \eta_tG_t) \linf{g_t - g_{t-1}}.
\end{align*}
\end{lemma}
\begin{proof}
\yub{TBA}
\end{proof}



\subsection{Auxiliary lemma for the iterative sequence}
\begin{lemma}\label{lem:delta.monotonic}
Given a sequence $\{\Delta_h^k\}_{h,k}$ defined by
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \beta_k,\\
    \Delta_{H+1}^k= 0 \text{ for all } k,
    \end{cases}
\end{equation}
where $\{\beta_k\}$ is non-increasing w.r.t. $k$. Then $\Delta_h^{k+1}\le \Delta_h^k$ for all $(k,h)\in\mathbb{N}\times[H+1]$.

\begin{proof}
We prove by doing backward induction on $h$. For the base case of induction, notice that the claim is true for $H+1$. Assume the claim is true for $h+1$. At step $h$, we have 
\begin{align*}
    \Delta_h^{k+1} & =  \sum_{t=1}^{k+1} \alpha_{k+1}^t \Delta_{h+1}^{t} + \beta_{k+1}\\
    & = (1-\alpha_{k+1}) \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \alpha_{k+1}\Delta_{h+1}^{k+1} +\beta_{k+1}\\
    & \le (1-\alpha_{k+1}) \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \alpha_{k+1} \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} +\beta_{k} = \Delta_h^k,
\end{align*}
where the inequality follows from the induction hypothesis and $\beta_{k+1}\le \beta_k$.
\end{proof}
\end{lemma}

\appendix
\section{Auxillary lemma for Lemma \ref{lemma:OFTRL-reg}}
\begin{lemma}\label{lemma:mu-nu-total-variation-bound}
Running OFTRL algorithm will guarantee that
\begin{align*}
    \|\mu_h^{t+1}(\cdot|s)-\mu_h^{t}(\cdot|s)\|_1,\|\nu_h^{t+1}(\cdot|s)-\nu_h^{t}(\cdot|s)\|_1 \le 4\eta H, ~~\forall 1\le h\le H, ~t\ge 0,~s\in\cS
\end{align*}
\begin{proof}
Without loss of generality, we will only proof the bound on $\mu$.
\begin{align*}
    \mu_h^t(\cdot|s)& = \argmax_{\mu}\<\mu, \frac{\eta}{w_t}\left(\sum_{i=1}^{t-1}w_i\E_{b\sim\nu_h^i(\cdot|s)}Q_h^i(s,\cdot,b) + w_t\E_{b\sim\nu_h^{t-1}}(\cdot|s)Q_h^{t-1}(s,\cdot,b)\right)\> - H(\mu)
\end{align*}
From Lemma \ref{lemma:Hedge-smoothness} we have that for $t=0$,
\begin{align*}
    \|\mu_h^{1}(\cdot|s)-\mu_h^{0}(\cdot|s)\|_1 \le 2\eta \left\|\E_{b\sim\nu_h^{0}}(\cdot|s)Q_h^{0}(s,\cdot,b)\right\|\le 2\eta H.
\end{align*}
For $t\ge 1$
\begin{align*}
    \|\mu_h^{t+1}(\cdot|s)-\mu_h^{t}(\cdot|s)\|_1 &\le 2\eta \left\|\frac{1}{w_{t+1}}\left(\sum_{i=1}^{t}w_i\E_{b\sim\nu_h^i(\cdot|s)}Q_h^i(s,\cdot,b) + w_{t+1}\E_{b\sim\nu_h^{t}}(\cdot|s)Q_h^{t}(s,\cdot,b)\right)\right.\\
&\quad     \left.-\frac{1}{w_t}\left(\sum_{i=1}^{t-1}w_i\E_{b\sim\nu_h^i(\cdot|s)}Q_h^i(s,\cdot,b) + w_t\E_{b\sim\nu_h^{t-1}}(\cdot|s)Q_h^{t-1}(s,\cdot,b)\right) \right\|_\infty\\
    &\le 2\eta \left\|\paren{\frac{1}{w_t} - \frac{1}{w_{t+1}}}\sum_{i=1}^{t-1}w_i\E_{b\sim\nu_h^i(\cdot|s)}Q_h^i(s,\cdot,b)\right\|_\infty + 2\eta\left\|Q_h^{t}(s,\cdot,b) -Q_h^{t-1}(s,\cdot,b)\right\| \\
    &\le 2\eta\paren{\frac{1}{w_t} - \frac{1}{w_{t+1}}}\sum_{i=1}^{t-1}w_i H + 2\eta H.
\end{align*}
Since
\begin{align*}
        &\paren{\frac{1}{w_t} - \frac{1}{w_{t+1}}}\sum_{i=1}^{t-1}w_i = \paren{\frac{1}{w_t} - \frac{1}{w_{t+1}}} \frac{1}{\alpha_{t-1}^1}\sum_{i=1}^{t-1}\alpha_{t-1}^i = \frac{1}{w_t\alpha_{t-1}^1} - \frac{1}{w_{t+1}\alpha_{t-1}^1}\\
    &= \frac{1-\alpha_t}{\alpha_t} - \frac{(1-\alpha_{t+1})(1-\alpha_t)}{\alpha_{t+1}} = (1-\alpha_t) \left(\frac{1}{\alpha_t} - \frac{1-\alpha_{t+1}}{\alpha_{t+1}}\right) = (1-\alpha_t)\frac{H}{H+1}\le 1,
\end{align*}
we have that
\begin{align*}
    \|\mu_h^{t+1}(\cdot|s)-\mu_h^{t}(\cdot|s)\|_1 \le 2\eta H+2\eta H = 4\eta H
\end{align*}
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:Hedge-smoothness}
Let $g_1, g_2\in \mathbb{R}^n$ and
\begin{align*}
    x_1 &= \argmax_{x\in\Delta_n} \<x, g_1\> - H(x)\\
    x_2 &= \argmax_{x\in\Delta_n}\<x,g_2\> - H(x),
\end{align*}
then $\|x_1 - x_2\|_1 \le 2\|g_1 - g_2\|_\infty$.
\begin{proof}
Since $H$ is $1$-strongly convex in $\|\cdot\|_1$ (Pinsker's inequality), we have that
\begin{align*}
    \frac{\|x_1-x_2\|_1^2}{2} &\le H(x_1) - H(x_2) - \<\nabla H(x_2), x_1-x_2\>\\
    &= H(x_1) + \left(\<x_2,g_1\>-H(x_2)\right) - \<x_2,g_1\> - \<\nabla H(x_2), x_1-x_2\>\\
    &\le  H(x_1) + \left(\<x_1,g_1\>-H(x_1)\right) - \<x_2,g_1\> - \<\nabla H(x_2), x_1-x_2\>\\
    &= \<x_1-x_2,g_1\> - \<\nabla H(x_2), x_1-x_2\>\\
    &= \<x_1-x_2,g_1-g_2\> + \<g_2 -\nabla H(x_2), x_1-x_2 \>\\
    &\le \<x_1-x_2,g_1-g_2\> ~~~\textup{(From the optimality of $x_2$)}\\
    &\le \|x_1-x_2\|_1\|g_1-g_2\|_\infty,
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:bound-A-k}
Define the sequence $\{A_k\}$ as
\begin{equation*}
    A_k:= \sum_{t=1}^k\alpha_k^t(\alpha_t)^2,
\end{equation*}
then we have the followings:
\begin{enumerate}
    \item $A_k\ge (\alpha_k)^2$ 
    \item $A_{k+1}\le A_k$
    \item $A_k \le \frac{(H+1)^3}{H^2 k}$
\end{enumerate}
\begin{proof}
We prove the first claim by induction. Since $A_1 = 1 = \alpha_1$, it naturally holds for $k=1$. Assume that the statement holds for $k$, then for $k+1$
\begin{align*}
    A_{k+1} &= \sum_{t=1}^{k+1}\alpha_{k+1}^t(\alpha_t)^2=(1-\alpha_{k+1})\sum_{t=1}^k\alpha_k^t(\alpha_t)^2 + (\alpha_{k+1})^3\\
    &= (1-\alpha_{k+1})A_k + (\alpha_{k+1})^3 \ge (1-\alpha_{k+1})(\alpha_k)^2 + (\alpha_{k+1})^3\\
    &\ge (1-\alpha_{k+1})(\alpha_{k+1})^2 + (\alpha_{k+1})^3\ge \alpha_{k+1}^2.
\end{align*}
Then the second claim holds naturally because
\begin{align*}
    A_{k+1} - A_k =  (1-\alpha_{k+1})A_k + (\alpha_{k+1})^3 - A_k = (\alpha_{k+1})^3 - \alpha_{k+1}A_k\le (\alpha_{k+1})^3-\alpha_{k+1}(\alpha_k)^2\le 0.
\end{align*}
The third claim is proved via the following bound
\begin{align*}
    A_k&\le \frac{1}{k}\sum_{t=1}^kA_t = \frac{1}{k}\sum_{t=1}^k\sum_{j=1}^t\alpha_t^j(\alpha_j)^2= \frac{1}{k}\sum_{j=1}^k(\alpha_j)^2\sum_{t=j}^t\alpha_t^j\\
    &\le \frac{1}{k}\sum_{j=1}^k(\alpha_j)^2\sum_{t=j}^{+\infty}\alpha_t^j= \frac{1}{k}\paren{1+\frac1H}\sum_{j=1}^k(\alpha_j)^2\\
    &\le \frac{1}{k}\paren{1+\frac1H}\sum_{j=1}^{k}\paren{\frac{H+1}{H+j}}^2\le\frac{1}{k}\paren{1+\frac1H}\frac{(H+1)^2}{H} \\
    &= \frac{(H+1)^3}{H^2k},
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

==> Sections/framework_clean_up_old.tex <==
\section{Algorithm framework for two-player zero-sum Markov Games}
\begin{algorithm}[h]
\caption{Algorithm framework for 2p0s Markov Games}
\label{alg:framework}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$, algorithm \matrixgamealg.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \matrixgamealg\paren{ \set{Q_h^{t}(s, \cdot, \cdot)}_{t\le {\color{red}k-1}}, 
    \set{\mu_h^{t}(\cdot|s)}_{t\le k-1}, 
    \set{\nu_h^{t}(\cdot|s)}_{t\le k-1}
    }.
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align}\label{eq:Q-update}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{{\color{red} k}}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


We define the following auxiliary variables:
\begin{align*}
    \alpha_k^t = (1-\alpha_k)(1-\alpha_{k-1})\cdots(1-\alpha_{t+1})\alpha_t
\end{align*}
It is not hard to verify that
\begin{equation*}
    \sum_{t=1}^k \alpha_k^t = 1,
\end{equation*}
and we have that
\begin{align}\label{eq:Q-relationship}
    Q_h^{k}(s,a,b) = \sum_{t=1}^k\alpha_k^t \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }
\end{align}


Define weighted regret as

\textcolor{blue}{[Runyu: I did some index change to match with the algorithm]}
\begin{align*}
    & \reg_{h,\mu}^k(s) \defeq \max_{z\in\Delta_\cA} \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\>, \\
    & \reg_{h,\nu}^k(s) \defeq \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>  \\
    & \reg_h^k \defeq \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\}.
\end{align*}
Define the unweighted average regret as:
\begin{align*}
    & \avgreg_{h,\mu}^k(s) \defeq \frac{1}{k}\max_{z\in\Delta_\cA} \sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\>, \\
    & \avgreg_{h,\nu}^k(s) \defeq \frac{1}{k}\sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>  \\
    & \avgreg_h^k \defeq \max_{s\in\cS}( \avgreg_{h,\mu}^k(s)+ \avgreg_{h,\nu}^k(s)).
\end{align*}

From now on, we assume that exist sequences $\reg^k, \avgreg^k$'s such that
\begin{align*}
    \reg^k \ge \reg_h^k, ~~\forall~ h,k,\\
    \avgreg^k \ge \avgreg_h^k, ~~\forall~ h,k,
\end{align*}
and that $\reg^k, \avgreg^k$'s are non-increasing with respect to $k$.

Define the state-wise average policy as
\begin{equation*}
    \hat{\mu}_h^k(\cdot|s) := \frac{1}{k}\sum_{t=1}^k\mu_{h}^{t}(\cdot|s),\quad 
    \hat{\nu}_h^k(\cdot|s) := \frac{1}{k}\sum_{t=1}^k \nu_h^{t}(\cdot|s).
\end{equation*}

Consider the value estimation error
\begin{align*}
    \delta_h^k \defeq \linf{ Q_h^k - Q_h^\star } = \max_{s,a,b} \abs{Q_h^k(s,a,b) - Q_h^\star(s,a,b)}.
\end{align*}


\begin{lemma}[Recursion of value estimation]\label{lemma:recursion-of-value-estimation}
We have for all $(k,h)\in[K]\times[H]$ that
\begin{align*}
    \delta_h^{k} \le \sum_{t=1}^k \alpha_k^t \delta_{h+1}^{t} + \reg_{h+1}^k.
\end{align*}
Further, we have that
\begin{equation*}
    \delta_h^k\le \frac{2H}{k}\sum_{t=1}^k\reg^t
\end{equation*}
\end{lemma}
\begin{proof}
From the definition of $Q_h^*$ we have that
\begin{align*}
    Q^*_h(s,a,b) &= r_h(s,a,b) + \max_{\mu_{h+1}}\min_{ \nu_{h+1}} \P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\nu_{h+1}(\cdot|s')\>}(s,a,b)\\
    &\le r_h(s,a,b) + \max_{\mu_{h+1}}\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times\paren{\sum_{t=1}^k \alpha_k^t \nu_{h+1}^{t}}(\cdot|s')\>}(s,a,b)\\
    &= r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b)}\\
    &\le  r_h(s,a,b) + \max_{\mu_{h+1}}\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b) + \delta_{h+1}^{t}}\\
    &\le r_h(s,a,b)+\sum_{t=1}^k \alpha_k^t\paren{\P_h\brac{\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times \nu_{h+1}^{t}(\cdot|s')\>}(s,a,b)} + \reg_{h+1}^k + \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}\\
    &= Q_h^{k}(s,a,b) +\sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k ~~\textup{(From \eqref{eq:Q-relationship})}
\end{align*}
Thus we have that
\begin{equation*}
    Q^*_h(s,a,b) - Q_h^{k}(s,a,b) \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Apply similar analysis to the minimizing player, we get
\begin{equation*}
      Q_h^{k}(s,a,b) -  Q^*_h(s,a,b)  \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,~~\forall~s,a,b.
\end{equation*}
Thus we get
\begin{equation*}
    \delta_h^{k} \le \sum_{t=1}^k\alpha_k^t \delta_{h+1}^{t}+\reg_{h+1}^k,
\end{equation*}
which completes the proof of the first inequality in the Lemma. Now consider an auxiliary sequence 
$\{\Delta_h^k \}_{h,k}$ defined by 
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \reg^k,\\
    \Delta_{H+1}^k= 0 \text{ for all } k.
    \end{cases}
\end{equation}
Observe that $\{\Delta_h^k \}_{h,k}$ satisfies the following properties 
\begin{equation}
    \begin{cases}
    \Delta_h^k \ge \delta_h^k\qquad &\text{ (by definition)},\\
    \Delta_h^k \le \Delta_h^{k-1} \quad &\text{ (by Lemma \ref{lem:delta.monotonic})}.
    \end{cases}
\end{equation}
Therefore, to control $\delta_h^k$, it suffices to bound $\frac{1}{k}\sum_{t=1}^k \Delta_h^t$, which follows from the standard argument in \cite{jin2018q}:
\begin{align*}
     \frac{1}{k}\sum_{t=1}^k \Delta_h^t 
     = & \frac{1}{k}\sum_{t=1}^k  \sum_{j=1}^{t} \alpha_{t}^j \Delta_{h+1}^{j} + \frac{1}{k}\sum_{t=1}^k \reg^t\\
      \le  & \frac{1}{k}  \sum_{j=1}^{k} \left(\sum_{t=j}^k \alpha_{t}^{j}\right) \Delta_{h+1}^{j} + \frac{1}{k}\sum_{t=1}^k \reg^t\\
     \le & \left(1+\frac{1}{H}\right)\frac{1}{k}\sum_{t=1}^k \Delta_{h+1}^t + \frac{1}{k}\sum_{t=1}^k \reg^t\\
     \le & \left(1+\frac{1}{H}\right)^2\frac{1}{k}\sum_{t=1}^k \Delta_{h+2}^t + \left(1+\left(1+\frac{1}{H}\right)\right)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le &\cdots\\
     \le &  \left(\sum_{h=1}^H\left(1+\frac{1}{H}\right)^h\right)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le & H(e-1)\left(\frac{1}{k}\sum_{t=1}^k \reg^t\right)\\
     \le& \frac{2H}{k}\sum_{t=1}^k \reg^t,
\end{align*}
which completes the proof of the second inequality in the Lemma.
\end{proof}




\begin{lemma}\label{lemma:NE-gap}
\begin{align*}
    \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t %2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t}
\end{align*}
\begin{proof}
We first give a bound for $\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB} Q_h^*(s,\hat\mu_h^k\times z)$, then we will  apply Lemma \ref{lem.duality} to complete the proof.
\begin{align*}
    &\max_{z\in\Delta_\cA}Q_h^*(s,z\times \hat \nu_h^k) - \min_{z\in\Delta_\cB}    Q_h^*(s,\hat\mu_h^k\times z) \\
    &= \max_{z\in\Delta_\cA}\frac{1}{k}\sum_{t=1}^kQ_h^*(s,z\times \nu_h^{t}) - \min_{z\in\Delta_\cB} \frac{1}{k}\sum_{t=1}^{k}Q_h^*(s,\mu_h^{t}\times z) \\
    &\le \max_{z\in\Delta_\cA}\frac{1}{k}\sum_{t=1}^kQ_h^t(s,z\times \nu_h^{t}) - \min_{z\in\Delta_\cB} \frac{1}{k}\sum_{t=1}^{k}Q_h^t(s,\mu_h^{t}\times z) + \frac{2}{k}\sum_{t=1}^k\delta_h^{t}\\
    &= \avgreg_h^k + \frac{2}{k}\sum_{t=1}^k\delta_h^{t}\\
    &\le \avgreg^k + \frac{2}{k}\sum_{t=1}^k\frac{2H}{t}\sum_{t=1}^j\reg^j~~~\textup{(Lemma \ref{lemma:bound_delta_h_k})}\\
    &\le \avgreg^k + \frac{2}{k}\sum_{j=1}^k\paren{\sum_{t=1}^k\frac{2H}{t}}\reg^j\\
    &\le \avgreg^k+\frac{4H\ln(k+1)}{k}\sum_{j=1}^k\reg^j
\end{align*}
Then by applying Lemma \ref{lem.duality}, we have
\begin{align*}
    &\|V_h^{\dagger,\hat{\nu}^k} - V_h^{\hat{\mu}^k,\dagger}\|\le \|V_h^{\dagger,\hat{\nu}^k} - V_h^*\| + \|V_h^*- V_h^{\hat{\mu}^k,\dagger}\|\\
    &\le \sum_{h'=h}^{H}\max_s\max_{z\in\Delta_\cA} \paren{Q_{h'}^*(s,z\times\hat\nu_{h'}^k)- V_{h'}^*(s)} + \sum_{h'=h}^H\max_s\min_{z\in\Delta_\cB}\paren{V_{h'}^*(s) - Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H \max_s\paren{\max_{z\in\Delta_\cA} Q_{h'}^*(s,z\times\hat\nu_{h'}^k) - \min_{z\in\Delta_\cB}Q_{h'}^*(s,\hat{\mu}_{h'}^k)}\\
    &\le 2\sum_{h'=h}^H\paren{\avgreg^k+\frac{4H\ln(k+1)}{k}\sum_{j=1}^k\reg^j}\\
    &\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{j=1}^k\reg^j,
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}

\section{Examples}
\subsection{GDA-critic}
\begin{algorithm}[h]
\caption{GDA-critic}
\label{alg:gda.critic-ver2}
\begin{algorithmic}
\STATE \textbf{Initialize:} learning rate $\eta$ and $\{\alpha_k\}_{k=1}^K$, set $V_{i,h}^0(s)=H-h+1$ and $\pi_{i,h}^0(s)$ to be uniform for all $i,h,s$.
\FOR{$k=1,\ldots,K$}
\FOR{$h = H, \ldots, 1$}
\STATE Update policy for all $s\in\cS$:
\begin{equation}\label{eq:mu-nu-update}
\begin{split}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\paren{\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,\cdot,b)}}}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) - \eta\paren{\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k-1}(s') }(s,a, \cdot)}}}
\end{split}
\end{equation}
\STATE Update V value for all $s\in\cS$:
\begin{align}\label{eq:V-update}
    V_h^{k}(s) \setto (1-\alpha_k) V_h^{k-1}(s) + \alpha_k \mathbb{E}_{a\sim \mu_h^{k}(\cdot|s), b\sim \nu_h^{k}(\cdot|s)}\paren{ \brac{r_h + \P_h V_{h+1}^{k}(s') }(s,a,b) }.
\end{align}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{lemma}
Algorithm \ref{alg:gda.critic-ver2} is equivalent to using the unified framework (Algorithm \ref{alg:framework}) with the $\matrixgamealg$ as
\begin{align*}
    \mu_h^k(\cdot|s)& \setto \mathcal{P}_{\Delta_{\cA}}\paren{\mu_h^{k-1}(\cdot|s) + \eta\mathbb{E}_{b\sim \nu_h^{k-1}(\cdot|s)}Q_h^{k-1}(s,\cdot,b)}\\
    \nu_h^k(\cdot|s)&\setto \mathcal{P}_{\Delta_{\cB}}\paren{\nu_h^{k-1}(\cdot|s) - \eta\mathbb{E}_{a\sim \mu_h^{k-1}(\cdot|s)} Q_h^{k-1}(s,a, \cdot)}
\end{align*}
\begin{proof}
It suffices to show that
\begin{equation}\label{eq:relation-Q-V}
    Q_h^{k}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^k(s')}(s,a,b)
\end{equation}
It is not hard to verify that
\begin{equation*}
    Q_h^{1}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^1(s')}(s,a,b),
\end{equation*}
We now prove by induction on both $k$ and $h$. Given that $ Q_h^{0}(s,a,b) = \brac{r_h+ \mathbb{P}_hV_{h+1}^0(s')}(s,a,b)$, it is not hard to verify that $Q_H^{k}(s,a,b) = r_H(s,a,b),~\forall~k\ge 0$. We assume that \eqref{eq:relation-Q-V} holds for $(k-1,h)$ and $(k, h+1)$, then for $(k,h)$, from \eqref{eq:Q-relationship}
\begin{align*}
     Q_h^{k}(s,a,b) &= (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }\\
     &= (1-\alpha_k)\brac{r_h+ \mathbb{P}_hV_{h+1}^{k-1}(s')}(s,a,b)\\
     &+\alpha_k \paren{ \brac{r_h + \P_h[\<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s')}(s,\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) } ~~\textup{(induction assumptions)}\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \<\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>\right) }(s,a,b)\\
     &=\brac{r_h+ \mathbb{P}_h\left((1-\alpha_k)V_{h+1}^{k-1}(s') +\alpha_k \mathbb{E}_{a\sim\mu_{h+1}^{k}(\cdot|s'), b\sim \nu_{h+1}^{k}(\cdot|s')}\brac{r_{h+1}+ \mathbb{P}_{h+1}V_{h+2}^k(s'')}(s',a,b)\right) }(s,a,b)\\
     &= \brac{r_h + \mathbb{P}_h V_{h+1}^k(s')}(s,a,b)~~\textup{(from \eqref{eq:V-update})},
\end{align*}
which completes the proof by induction
\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:reg-h-k-GDA-critic}
Set $\alpha_k$ in Algorithm \ref{alg:gda.critic-ver2} as
\begin{equation*}
    \alpha_k = \frac{H+1}{H+k}.
\end{equation*},
then we have that
\begin{equation*}
    \reg^k = \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta \max\{A,B\}H^2}{2}, \avgreg = \frac{4}{\eta k}+\frac{\eta(A+B)H^2}{2}
\end{equation*}
\begin{proof}
We apply Lemma \ref{lem:gd.regret} to \eqref{eq:mu-nu-update} and we can get an upperbound for both $\reg_{h,\mu}^k, \reg_{h,\nu}^k$:
\begin{align*}
    \reg_{h,\mu^k}&\le \frac{1}{2\eta}\alpha_k^k\max_{z,z'\in\Delta_\cA}\|z-z'\|^2 + \frac{\eta AH^2}{2}\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta AH^2}{2}\\
    \reg_{h,\nu^k}&\le \frac{1}{2\eta}\alpha_k^k\max_{z,z'\in\Delta_\cB}\|z-z'\|^2 + \frac{\eta BH^2}{2}\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta BH^2}{2},\\
    \Longrightarrow\quad \reg_h^k &\le \frac{2}{\eta}\frac{H+1}{H+k} + \frac{\eta \max\{A,B\}H^2}{2}.
\end{align*}
Similarly,
\begin{align*}
    \avgreg_{h,\mu^k}&\le \frac{1}{2\eta k}\max_{z,z'\in\Delta_\cA}\|z-z'\|^2 + \frac{\eta AH^2}{2}\le \frac{2}{\eta k} + \frac{\eta AH^2}{2}\\
    \avgreg_{h,\nu^k}&\le \frac{1}{2\eta k}\max_{z,z'\in\Delta_\cB}\|z-z'\|^2 + \frac{\eta BH^2}{2}\le \frac{2}{\eta k} + \frac{\eta BH^2}{2},\\
    \Longrightarrow\quad \avgreg_h^k &\le \frac{4}{\eta k} + \frac{\eta (A+B)H^2}{2} .
\end{align*}
\end{proof}
\end{lemma}

\begin{theorem}\label{thm:2p0s}
For all $(i,h)\in[2]\times[H]$, 
$$
\|V_{i,h}^{\dagger,\hat\pi_{-i}^k} - V_{i,h}^\star \|_\infty\le 
6\eta\max\{A,B\}H^4 + \frac{32H^3\left(\ln(H+k)^2 + 1\right)}{\eta k}.
$$
\begin{proof}
From Lemma \ref{lemma:NE-gap} and Lemma \ref{lemma:reg-h-k-GDA-critic} we have that
\begin{align*}
     \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
     &\le 2H\paren{ \frac{4}{\eta k} + \frac{\eta (A+B)H^2}{2}} + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{2}{\eta}\frac{H+1}{H+t} + \frac{\eta \max\{A,B\}H^2}{2}}\\
     &\le \frac{8H}{\eta k}+{\eta (A+B)H^3} +\frac{32H^3\ln(H+k)\ln(k+1)}{\eta k} + {4\eta\max\{A,B\}H^4}\\
     &\le 6\eta\max\{A,B\}H^4 + \frac{32H^3\left(\ln(H+k)^2 + 1\right)}{\eta k}
\end{align*}
\end{proof}
\end{theorem}

\subsection{Nash V-learning (full feedback)}
\textcolor{blue}{TODO}

\yub{State-wise averaging guarantee}


\subsection{Nash Q-learning (full feedback)}
\begin{algorithm}[h]
\caption{Nash Q-learning}
\label{alg:Nash-Q}
\begin{algorithmic}
\STATE \textbf{Require:} Learning rate $\set{\alpha_k}_{k\ge 1}$.
\STATE \textbf{Initialize:} $Q_h^0(s,a,b)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$k=1,\dots,K$}
\FOR{$h=H,\dots,1$}
\STATE Update policy for all $s\in\cS$:
\begin{align*}
    (\mu_h^k(\cdot|s), \nu_h^k(\cdot|s)) \setto \NE(Q_h^{k-1}(s,\cdot,\cdot)).
\end{align*}
\STATE Update Q value for all $(s,a,b)\in\cS\times\cA\times\cB$:
\begin{align*}
    Q_h^{k}(s,a,b) \setto (1-\alpha_k) Q_h^{k-1}(s,a,b) + \alpha_k \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b) }.
\end{align*}
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{$\alpha_k = 1$}
In this case, we have that $Q_h^k$ equals to $Q_h^{\mu^k\times\nu^k}$.
\begin{lemma}
When $\alpha_k$'s are all set to $\alpha_k = 1$, then we have that for $k \ge H-h+1$,
\begin{equation*}
    Q_h^k(s,a,b) = Q_h^*(s,a,b),~~\forall ~h, ~\forall~s,a,b
\end{equation*}
\begin{proof}
We prove this by induction. For h = H, we have that
\begin{equation*}
    Q_H^{k}(s,a,b) = r_H(s,a,b),~~\forall k \ge 1.
\end{equation*}
Assume that for $h+1$, the condition holds, then for time horizon $h$ and iteration step $k\ge H-h+1$, we have that
\begin{align*}
    Q_h^k(s,a,b) &= \brac{r_h + \P_h[\<Q_{h+1}^{k}(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)
\end{align*}
Additionally, from the induction assumption,
\begin{align*}
    (\mu_{h+1}^k(\cdot|s), \nu_{h+1}^k(\cdot|s)) =  \NE(Q_{h+1}^{k-1}(s,\cdot,\cdot)) = \NE(Q_{h+1}^*(s,\cdot,\cdot)),
\end{align*}
we have that
\begin{align*}
    \<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\> = V_{h+1}^*(s').
\end{align*}
Thus
\begin{align*}
    Q_h^k(s,a,b)
    & = \brac{r_h + \P_h[\<Q_{h+1}^*(s',\cdot,\cdot), \mu_{h+1}^{k}(\cdot|s')\times\nu_{h+1}^{k}(\cdot|s')\>] }(s,a,b)\\
    & = \brac{r_h + \P_h[V(s')]}(s,a,b) = Q_h^*(s,a,b),
\end{align*}
which completes the proof.
\end{proof}
\end{lemma}
\begin{lemma}
\textcolor{blue}{TODO: bound $\reg_h^k$}
\end{lemma}
\subsection{$\alpha_k = \frac{H+1}{H+k}$}
\begin{lemma}\label{lemma:reg-Nash-Q}
For Algorithm \ref{alg:Nash-Q} with $\alpha_k = \frac{H+1}{H+k}$, we have that 
\begin{equation*}
    \reg^k = \frac{(H+1)^2}{H+k} ,~~~~\avgreg_h^k =\frac{2H^2\ln(H+k)}{k}
\end{equation*}
\begin{proof}
\begin{align*}
    &\reg_{h,\mu}^k(s)+\reg_{h,\nu}^k(s) = \max_{z\in\Delta_\cA} \sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> - \min_{z\in\Delta_\cB}\sum_{t=1}^k \alpha_k^t \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\> \\
    &~~\le \sum_{t=1}^k  \alpha_k^t \left(\max_{z\in\Delta_\cA}\< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\> -\min_{z\in\Delta_\cB} \< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\> \right)+ 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty\\
    &~~\le 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty.\\
    &\avgreg_{h,\mu^k} + \avgreg_{h,\nu^k} = \frac{1}{k}\max_{z\in\Delta_\cA} \sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\>- \min_{z\in\Delta_\cB}\sum_{t=1}^k \< Q_h^{t}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>\\
    &~~\le \frac{1}{k} \sum_{t=1}^k \left(\max_{z\in\Delta_\cA}\< Q_h^{t-1}(s,\cdot,\cdot), z\times \nu_h^{t}(\cdot|s)\>- \min_{z\in\Delta_\cB}\< Q_h^{t-1}(s,\cdot,\cdot), \mu_h^{t}(\cdot|s)\times z\>\right) + \frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty\\
    &~~\le\frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty.
\end{align*}
Thus
\begin{equation*}
    \reg_h^k \le 2 \sum_{t=1}^k \alpha_k^t\|Q_h^t - Q_h^{t-1}\|_\infty,\quad \avgreg_h^k \le \frac{1}{k}\sum_{t=1}^k \|Q_h^t - Q_h^{t-1}\|_\infty.
\end{equation*}
Since
\begin{align*}
    &Q_h^{t}(s,a,b) = (1-\alpha_t) Q_h^{t-1}(s,a,b) + \alpha_t \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }\\
    \Longrightarrow & |Q_h^{t}(s,a,b) -  Q_h^{t-1}(s,a,b)|\le \alpha_t |Q_h^{t-1}(s,a,b) - \paren{ \brac{r_h + \P_h[\<Q_{h+1}^{t}(s',\cdot,\cdot), \mu_{h+1}^{t}(\cdot|s')\times\nu_{h+1}^{t}(\cdot|s')\>] }(s,a,b) }|
    \le \alpha_t H\\
    \Longrightarrow&\|Q_h^{t}-Q_h^{t-1}\|_\infty\le \alpha_t H ,
\end{align*}
substituting this into the above equations we have that
\begin{equation*}
    \reg_h^k \le H \sum_{t=1}^k \alpha_k^t \alpha_t,~~~~\avgreg_h^k \le\frac{H}{k} \sum_{t=1}^k\alpha_t \le\frac{2H^2\ln(H+k)}{k}
\end{equation*}
we now further bound $\reg_h^k$. Define $x_k:= \sum_{t=1}^k \alpha_k^t \alpha_t$. From the definition of $x_k$ we have that~\yub{check}
\begin{align*}
    &x_{k+1} =  \sum_{t=1}^{k+1} \alpha_{k+1}^t \alpha_t = \sum_{t=1}^k (1-\alpha_{k+1})\alpha_k^t\alpha_t + \alpha_{k+1}^2 = (1-\alpha_{k+1}^t)x_k + \alpha_{k+1}\\
    \Longrightarrow ~~&x_{k+1} = \frac{k}{H+k+1}x_k + \frac{(H+1)^2}{(H+k+1)^2}\le \frac{k}{H+k+1}x_k  + \frac{(H+1)^2}{(H+k+1)(H+k)}\\
    \Longrightarrow ~~&\paren{x_{k+1} - \frac{(H+1)^2}{H(H+k+1)}}\le\frac{k}{H+k+1} \paren{x_{k+1} - \frac{(H+1)^2}{H(H+k)}}.
\end{align*}
Since $x_1 = \alpha_1^2 = 1\le \frac{(H+1)^2}{H(H+2)}$, we have that $x_k \le \frac{(H+1)^2}{H(H+k)} $, which completes the proof.
\end{proof}
\end{lemma}
\begin{theorem}\label{thm:Nash-Q}
For all $(i,h)\in[2]\times[H]$, 
$$
\|V_{i,h}^{\dagger,\hat\pi_{-i}^k} - V_{i,h}^\star \|_\infty\le 
\frac{32H^4\left(\ln(H+k)^2+1\right)}{k}.
$$
\begin{proof}
From Lemma \ref{lemma:NE-gap} and Lemma \ref{lemma:reg-Nash-Q} we have that
\begin{align*}
     \|V_h^{\dagger,\hat{\nu}^k} -V_h^{\hat{\mu}^k, \dagger}\|_\infty&\le 2H\avgreg^k + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k \reg^t\\
     &\le 2H\paren{\frac{2H^2\ln(H+k)}{k}} + \frac{8H^2\ln(k+1)}{k}\sum_{t=1}^k\paren{\frac{(H+1)^2}{H+k}}\\
     &\le \frac{4H^3\ln(H+k)}{k} +\frac{32H^4\ln(H+k)^2}{k}\\
     &\le \frac{32H^4\left(\ln(H+k)^2+1\right)}{k}
\end{align*}
\end{proof}
\end{theorem}


\subsection{A Counterexample - 'Eager value function'}
In this section, we consider the GDA-critic algorithm (Algorithm \ref{alg:gda.critic-ver2}) with 
\begin{equation*}
    \alpha_k = 1.
\end{equation*}
In this case, $V_h^k$ is the true value function of policy $\mu^k\times \nu^k$. However, although the value function estimation is more accurate in this setting, this actually introduces larger weighted regret $\reg_h^k$ and thus this algorithm no-longer works. \textcolor{blue}{TODO: put our numerical simulation suggesting the problem of this algorithm} Notice that in this setting we can no longer guarantee that the weighted regret $\reg_h^k$'s are small, i.e.,
\begin{align*}
    & \reg_{h,\mu}^k(s) = \max_{z\in\Delta_\cA} \< Q_h^{k-1}(s,\cdot,\cdot), z\times \nu_h^{k-1}(\cdot|s)\> - \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> \sim O(1)\\
    & \reg_{h,\nu}^k(s) = \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times \nu_h^{k-1}(\cdot|s)\> - \min_{z\in\Delta_\cB} \< Q_h^{k-1}(s,\cdot,\cdot), \mu_h^{k-1}(\cdot|s)\times z\> \sim O(1) \\
    &\Longrightarrow~~ \reg_h^k = \max_{s\in\cS} \max\{\reg_{h,\mu}^k(s), \reg_{h,\nu}^k(s)\} \sim O(1)
\end{align*}


\section{Auxillaries}
\subsection{Auxiliary lemma for gradient descent}
To begin with, we derive a weighted regret bound for gradient descent. 

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Initialize} $x_1\in\cX$
\FOR{$t=1,\ldots,T$}
\STATE $y_{t+1} = x_t - \eta g_t$
\STATE $x_{t+1} = \cP_\cX( y_{t+1}) $
\ENDFOR
\end{algorithmic}
\end{algorithm}

For simplicity of notation, denote the diameter of $\cX$ by $R$ and $G=\max_{t\in[T]}\|g_t\|_2$.

\begin{lemma}\label{lem:gd.regret}
 For any $z\in\cX$ and $\mathbf{w}\in\Delta_T$ satisfying $w_{t+1}\ge w_t$ for $t\in[T-1]$, we have
$$
 \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le \frac{1}{2\eta} w_T R^2  + \frac{\eta G^2}{2}.
$$
\end{lemma}
\begin{proof}
By following the standard GD analysis, we first have
%~\yub{$1/\eta$ should be $1/(2\eta)$?}
\begin{align*}
    \langle x_t -z, g_t\rangle =& \frac{1}{\eta} \langle x_t -z, x_t - y_{t+1}\rangle \\
    = & \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-y_{t+1}\|^2 \right]\\
    \le& \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-x_{t+1}\|^2 \right]\\
    = &\frac{1}{2\eta} \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right],
\end{align*}
where the inequality follows from $z\in\cX$ and $x_{t+1} = \cP_\cX( y_{t+1})$. By multiplying both sides with $w_t$ and taking summation over $t\in[T]$, we have
\begin{align*}
   \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le & \frac{1}{2\eta}\sum_{t=1}^T  w_t  \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right]\\
   \le  &\frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t)\|z-x_{t+1}\|^2
   + w_1 \|x_1 - z\|^2 + \frac{ \eta G^2}{2}\\
   \le & \frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t) R^2 + w_1 R^2 + \frac{ \eta G^2}{2} = \frac{1}{2\eta} w_T R^2  +\frac{ \eta G^2}{2},
\end{align*}
where the second inequality uses $\w\in\Delta_{T}$ and the third one uses $w_{t+1}\ge w_t$.
\end{proof}



\begin{lemma}\label{lem:delta.monotonic}
Given a sequence $\{\Delta_h^k\}_{h,k}$ defined by
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \beta_k,\\
    \Delta_{H+1}^k= 0 \text{ for all } k,
    \end{cases}
\end{equation}
where $\{\beta_k\}$ is non-increasing w.r.t. $k$. Then $\Delta_h^{k+1}\le \Delta_h^k$ for all $(k,h)\in\mathbb{N}\times[H+1]$.

\begin{proof}
We prove by doing backward induction on $h$. For the base case of induction, notice that the claim is true for $H+1$. Assume the claim is true for $h+1$. At step $h$, we have 
\begin{align*}
    \Delta_h^{k+1} & =  \sum_{t=1}^{k+1} \alpha_{k+1}^t \Delta_{h+1}^{t} + \beta_{k+1}\\
    & = (1-\alpha_{k+1}) \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \alpha_{k+1}\Delta_{h+1}^{k+1} +\beta_{k+1}\\
    & \le (1-\alpha_{k+1}) \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} + \alpha_{k+1} \sum_{t=1}^{k} \alpha_{k}^t \Delta_{h+1}^{t} +\beta_{k} = \Delta_h^k,
\end{align*}
where the inequality follows from the induction hypothesis and $\beta_{k+1}\le \beta_k$.
\end{proof}
\end{lemma}


==> Sections/gdacritic.tex <==
\section{GDA-Critic algorithm for Markov Games}


\subsection{Algorithm}
The algorithm below is general, does not assume 2p0s.

\begin{algorithm}[h]
\caption{Learning Markov Games with Gradient Ascent}
\label{alg:gda.critic}
\begin{algorithmic}
\STATE \textbf{Initialize:} learning rate $\eta$ and $\{\alpha_k\}_{k=1}^K$, set $V_{i,h}^0(s)=H$ and $\pi_{i,h}^0(s)$ to be uniform for all $i,h,s$.
\FOR{$k=1,\ldots,K$}
\FOR{$(i,s,h)\in[N]\times\cS\times [H]$}
\STATE $\pi_{i,h}^k(s) = \mathcal{P}_{\Delta_{A_i}}\left(\pi_{i,h}^{k-1}(s)+\eta Q_{i,h}^{k-1}(s, \cdot\times \pi_{i,h}^{k-1}(s))\right)$~\yub{corrected to $Q$, may have some indexing issue}
% \STATE $\pi_{i,h}^k(s) = \mathcal{P}_{\Delta_{A_i}}\left(\pi_{i,h}^{k-1}(s)+\eta V_{i,h}^{k-1}(s)\right)$
\STATE $V_{i,h}^{k}(s) = (1-\alpha_{k})V_{i,h}^{k-1}(s)+\alpha_{k} \E\left[ r_{i,h}(s,\a)+V_{i,h+1}^{k-1}(s') \mid \a\sim \pi^{k-1}_{h}(s),s'\sim\P_h(s,\a)\right]$
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{Auxiliary lemma for gradient descent}
To begin with, we derive a weighted regret bound for gradient descent. 
\QL{Let's do fixed learning rate $\eta$ for now.}

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Initialize} $x_1\in\cX$
\FOR{$t=1,\ldots,T$}
\STATE $y_{t+1} = x_t - \eta g_t$
\STATE $x_{t+1} = \cP_\cX( y_{t+1}) $
\ENDFOR
\end{algorithmic}
\end{algorithm}

For simplicity of notation, denote the diameter of $\cX$ by $R$ and $G=\max_{t\in[T]}\|g_t\|_2$.

\QL{Do we have something similar in OGDA?}
\begin{lemma}\label{lem:gd.regret}
 For any $z\in\cX$ and $\mathbf{w}\in\Delta_T$ satisfying $w_{t+1}\ge w_t$ for $t\in[T-1]$, we have
$$
 \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le \frac{1}{2\eta} w_T R^2  + \frac{\eta G^2}{2}.
$$
\end{lemma}
\begin{proof}
By following the standard GD analysis, we first have
%~\yub{$1/\eta$ should be $1/(2\eta)$?}
\begin{align*}
    \langle x_t -z, g_t\rangle =& \frac{1}{\eta} \langle x_t -z, x_t - y_{t+1}\rangle \\
    = & \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-y_{t+1}\|^2 \right]\\
    \le& \frac{1}{2\eta} \left[ \|x_t-z\|^2+\|x_t-y_{t+1}\|^2 - \|z-x_{t+1}\|^2 \right]\\
    = &\frac{1}{2\eta} \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right],
\end{align*}
where the inequality follows from $z\in\cX$ and $x_{t+1} = \cP_\cX( y_{t+1})$. By multiplying both sides with $w_t$ and taking summation over $t\in[T]$, we have
\begin{align*}
   \sum_{t=1}^T  w_t \langle x_t -z, g_t\rangle \le & \frac{1}{2\eta}\sum_{t=1}^T  w_t  \left[ \|x_t-z\|^2 - \|z-x_{t+1}\|^2 + \eta^2\|g_t\|^2\right]\\
   \le  &\frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t)\|z-x_{t+1}\|^2
   + w_1 \|x_1 - z\|^2 + \frac{ \eta G^2}{2}\\
   \le & \frac{1}{2\eta}\sum_{t=1}^{T-1} (w_{t+1}-w_t) R^2 + w_1 R^2 + \frac{ \eta G^2}{2} = \frac{1}{2\eta} w_T R^2  +\frac{ \eta G^2}{2},
\end{align*}
where the second inequality uses $\w\in\Delta_{T}$ and the third one uses $w_{t+1}\ge w_t$.
\end{proof}

\subsection{Two-player zero-sum Markov Games}

The following lemma will be useful in controlling the duality gap of the state-wise average policy produced by GDA in the two-player zero-sum setting. Specifically, it shows that if a policy is approximately Nash at each state with respect to $Q^\star$, then its minimax duality gap is small.

\QL{I feel there might be a multi-player general-sum version of this lemma.}
\begin{lemma}\label{lem.duality}
In two-player zero-sum Markov games, suppose a Markov policy $\pi$ satisfies 
$$\max_{s} \max_{z\in\Delta_{A_i}} \left(Q_{i,h}^\star(s,z\times\pi_{-i,h}(s))-V_{i,h}^\star(s) \right)\le \epsilon_h$$ for all $(i,h)\in[2]\times[H+1]$, then 
$$
\|V_{i,h}^{\dagger,\pi_{-i}} - V_{i,h}^\star \|_\infty\le \sum_{h'=h}^H \epsilon_{h'}.
$$
\end{lemma}
\begin{proof}
We prove by induction.
The claim is trivial for $h=H+1$.
Suppose the claim holds  for step $h+1$. At step $h$,
\begin{align*}
&\| V_{i,h}^{\dagger,\pi_{-i}} - V_{i,h}^\star\|_\infty \\
\le &  \max_s \left( \max_{z\in\Delta_{A_i}} Q_{i,h}^{\dagger,\pi_{-i}}(s,z\times\pi_{-i,h}(s)) - V_{i,h}^\star(s)\right)\\
\le &  \max_s \left(  \max_{z\in\Delta_{A_i}} Q_{i,h}^{\star}(s,z\times\pi_{-i,h}(s)) - V_{i,h}^\star(s)\right)+ \sum_{h'=h+1}^H \epsilon_{h'}\le \sum_{h'=h}^H \epsilon_{h'},
\end{align*}
where the second inequality follows from the induction hypothesis and the third one uses the precondition of the lemma.
\yub{second inequality used the 2p0s property too}
\end{proof}


\begin{lemma}\label{lem:delta.monotonic}
Given a sequence $\{\Delta_h^k\}_{h,k}$ defined by
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} + \beta_k,\\
    \Delta_{H+1}^k= 0 \text{ for all } k,
    \end{cases}
\end{equation}
where $\{\beta_k\}$ is non-increasing w.r.t. $k$. Then $\Delta_h^{k+1}\le \Delta_h^k$ for all $(k,h)\in\mathbb{N}\times[H+1]$.
\end{lemma}
\begin{proof}
We prove by doing backward induction on $h$. For the base case of induction, notice that the claim is true for $H+1$. Assume the claim is true for $h+1$. At step $h$, we have 
\begin{align*}
    \Delta_h^{k+1} & =  \sum_{j=1}^{k+1} \alpha_{k+1}^j \Delta_{h+1}^{j-1} + \beta_{k+1}\\
    & = (1-\alpha_{k+1}) \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} + \alpha_{k+1}\Delta_{h+1}^{k} +\beta_{k+1}\\
    & \le (1-\alpha_{k+1}) \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} + \alpha_{k+1} \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} +\beta_{k} = \Delta_h^k,
\end{align*}
where the inequality follows from the induction hypothesis and $\beta_{k+1}\le \beta_k$.
\end{proof}


\subsection{Bounding the error between $V^k$ and  $V^\star$}

We first introduce some notations that will be frequently used in this section. 

Denote 
$$
Q^k_{i,h}(s,\a):= \E\left[ r_{i,h}(s,\a)+V_{i,h+1}^{k}(s') \mid s'\sim\P_h(s,\a)\right]
$$
$$
\delta_h^k:=\max_{i}\|V^k_{i,h}-V^\star_{i,h}\|_\infty
$$
$$
A = \max_i A_i
$$

\begin{lemma}\label{lem:Vk-Vstar}
For all $(k,h)$,
$$
 \delta_h^k \le 
 \cO\left(\frac{H^2}{k}+\frac{H^2\log k}{k\eta}+\eta AH^3\right).
$$
\end{lemma}
\begin{proof}
The proof works by computing a  recursive formula for $\delta_{h,k}$.
By the definition of $V^k$, we have
\begin{align*}
    \delta_{h}^k &  = \max_{i,s} | V_{i,h}^k(s)-V^\star_{i,h}(s)|\\
    & = \max_{i,s}\left| \sum_{j=1}^{k} \alpha_{k}^j Q_{i,h}^{j-1}(s,\pi_h^{j-1}(s))-V^\star_{i,h}(s)\right|.
\end{align*}
By Lemma \ref{lem:gd.regret} and noticing that $\|Q^k_{i,h}-Q^\star_{i,h}\|_\infty \le \delta_{h+1}^k$,
\begin{equation}\label{eq:1}
\begin{aligned}
    &\sum_{j=1}^{k} \alpha_{k}^j Q_{i,h}^{j-1}(s,\pi_h^{j-1}(s))\\
    \ge & \max_{z\in\Delta_{A_i} }\sum_{j=1}^{k} \alpha_{k}^j Q_{i,h}^{j-1}(s,z\times \pi_{-i,h}^{j-1}(s)) -  (\frac{1}{2\eta} \alpha_{k}^{k} + \eta A_iH^2) \\
    \ge & \max_{z\in\Delta_{A_i} }\sum_{j=1}^{k} \alpha_{k}^j Q_{i,h}^\star(s,z\times \pi_{-i,h}^{j-1}(s)) -  (\frac{1}{2\eta} \alpha_{k}^{k} + \eta A_iH^2) -\sum_{j=1}^{k} \alpha_{k}^j \delta_{h+1}^{j-1} \\
    \ge & V_{i,h}^\star(s)-  (\frac{1}{2\eta} \alpha_{k}^{k} + \eta A_iH^2) -\sum_{j=1}^{k} \alpha_{k}^j \delta_{h+1}^{j-1}.
\end{aligned}
\end{equation}
\yub{Last ineq uses 2p0s}
Besides, notice that in two-player zero-sum Markov games, we always have 
\begin{equation}\label{eq:2}
    Q_{i,h}^j = -  Q_{3-i,h}^j, \quad V_{i,h}^\star = - V_{3-i,h}^\star.
\end{equation}
By combining equation \eqref{eq:1} and \eqref{eq:2}, we obtain
$$
\delta_h^k \le  \sum_{j=1}^{k} \alpha_{k}^j \delta_{h+1}^{j-1} + \left(\frac{1}{2\eta} \frac{H+1}{H+k} + \frac{\eta A H^2}{2}\right).
$$
Now consider an auxiliary sequence 
$\{\Delta_h^k \}_{h,k}$ defined by 
\begin{equation}
    \begin{cases}
    \Delta_h^k =  \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} + \left(\frac{1}{2\eta} \frac{H+1}{H+k} + \frac{\eta A H^2}{2}\right),\\
    \Delta_{H+1}^k= 0 \text{ for all } k.
    \end{cases}
\end{equation}
Observe that $\{\Delta_h^k \}_{h,k}$ satisfies the following properties 
\begin{equation}
    \begin{cases}
    \Delta_h^k \ge \delta_h^k\qquad &\text{ (by definition)},\\
    \Delta_h^k \le \Delta_h^{k-1} \quad &\text{ (by Lemma \ref{lem:delta.monotonic})}.
    \end{cases}
\end{equation}
Therefore, to control $\delta_h^K$, it suffices to bound $\frac{1}{K}\sum_{k=1}^K \Delta_h^k$, which follows from the standard argument in \cite{jin2018q}:
\begin{align*}
     \frac{1}{K}\sum_{k=1}^K \Delta_h^k 
     = & \frac{1}{K}\sum_{k=1}^K  \sum_{j=1}^{k} \alpha_{k}^j \Delta_{h+1}^{j-1} + \frac{1}{K}\sum_{k=1}^K \left(\frac{1}{2\eta} \frac{H+1}{H+k} + \frac{\eta A H^2}{2}\right)\\
      \le  & \frac{1}{K}  \sum_{j=0}^{K} \left(\sum_{k=j+1}^K \alpha_{k}^{j+1}\right) \Delta_{h+1}^{j} + \frac{1}{K}\sum_{k=1}^K \left(\frac{1}{2\eta} \frac{H+1}{H+k} + \frac{\eta A H^2}{2}\right)\\
     \le & \frac{1}{K}\left(1+\frac{1}{H}\right)\sum_{k=0}^K \Delta_{h+1}^k + \cO\left(\frac{H\log K}{K\eta}+\eta AH^2\right)\\
     \le &\frac{1}{K}\left(1+\frac{1}{H}\right)\sum_{k=1}^K \Delta_{h+1}^k + \cO\left(\frac{H}{K}+\frac{H\log K}{K\eta}+\eta AH^2\right),
\end{align*}
which implies for all $(k,h)$
$$
 \frac{1}{k}\sum_{t=1}^k \Delta_h^t \le 
 \cO\left(\frac{H^2}{k}+\frac{H^2\log k}{k\eta}+\eta AH^3\right).
$$
We conclude the proof by recalling 
$\delta_h^k \le \Delta_h^k \le \frac{1}{k}\sum_{t=1}^k \Delta_h^t$.
\end{proof}

\subsection{Main theorem}
Define the state-wise average policy of player $i$ in the $k^{\rm th}$ iteration as below
$$
\hat\pi_{i,h}^k(s) = \frac{1}{k}\sum_{t=1}^k \pi_{i,h}^{t-1}(s) \quad (s,h)\in\cS\times[H].
$$
\yub{This is a Markov policy (which is good), not certified policy}
\begin{theorem}\label{thm:2p0s}
For all $(i,h)\in[2]\times[H]$, 
$$
\|V_{i,h}^{\dagger,\hat\pi_{-i}^k} - V_{i,h}^\star \|_\infty\le 
\cO\left(\frac{H^2\log k}{k}+\frac{H^2\log^2 k}{k\eta}+\eta AH^3\right).
$$
\end{theorem}
\begin{proof}
By Lemma \ref{lem:gd.regret} and the definition of $\delta_h^k$,
\begin{equation}\label{eq:3}
\begin{aligned}
&\max_{z\in\Delta_{A_i}}  Q_{i,h}^\star (s,z\times \hat\pi^k_{-i,h}(s))\\
= & \frac{1}{k}\max_{z\in\Delta_{A_i} }\sum_{j=1}^{k}  Q_{i,h}^\star(s,z\times \pi_{-i,h}^{j-1}(s)) \\
\le  & \frac{1}{k} \max_{z\in\Delta_{A_i} }\sum_{j=1}^{k}  Q_{i,h}^{j-1}(s,z\times \pi_{-i,h}^{j-1}(s)) +\frac{1}{k}\sum_{j=1}^{k}  \delta_{h+1}^{j-1} \\
  \le &\frac{1}{k}\sum_{j=1}^{k}  Q_{i,h}^{j-1}(s,\pi_h^{j-1}(s))+\frac{1}{k}\sum_{j=1}^{k}  \delta_{h+1}^{j-1}+( \frac{1}{2\eta k} + \frac{\eta AH^2}{2}).
\end{aligned}
\end{equation}
Combining equation \eqref{eq:2} and \eqref{eq:3} gives
\begin{align*}
    \min_{y\in\Delta_{A_{3-i}}}  Q_{i,h}^\star (s, \hat\pi^k_{i,h}(s)\times y)
    \ge   \frac{1}{k}\sum_{j=1}^{k}  Q_{i,h}^{j-1}(s,\pi_h^{j-1}(s))-\frac{1}{k}\sum_{j=1}^{k}  \delta_{h+1}^{j-1}-( \frac{1}{2\eta k} + \frac{\eta AH^2}{2}).
\end{align*}
As a result, we have
$$
\max_{z\in\Delta_{A_i}}  Q_{i,h}^\star (s,z\times \hat\pi^k_{-i,h}(s)) -     \min_{y\in\Delta_{A_{3-i}}} \sum_{j=1}^k Q_{i,h}^\star (s, \hat\pi^k_{i,h}(s)\times y) \le \frac{2}{k}\sum_{j=1}^{k}  \delta_{h+1}^{j-1}+( \frac{1}{\eta k} + \eta AH^2).
$$
By Lemma \ref{lem:Vk-Vstar}
%~\yub{two terms below have same order}, 
\begin{equation}
\frac1k \sum_{j=1}^{k}  \delta_{h+1}^{j-1} \le \cO\left(\frac{H^2\log k}{k}+\frac{H^2\log^2 k}{k\eta}+\eta AH^3\right).
\end{equation}
Therefore, we have 
$$
\max_{z\in\Delta_{A_i}} Q_{i,h}^\star (s,z\times \hat\pi^k_{-i,h}(s)) 
- V_{i,h}^{\star}(s)\le \cO\left(\frac{H^2\log k}{k}+\frac{H^2\log^2 k}{k\eta}+\eta AH^3\right).
$$
Finally, we conclude the proof by revoking Lemma \ref{lem.duality} with the above inequality.
\end{proof}

\subsection{Regret bound}

\yub{Based on Lemma 3, avg policy (non-Markov) should also converge to Nash?}

\begin{theorem}[Regret bound for GDA-Critic]
For two-player zero-sum Markov Games, Algorithm~\ref{alg:gda.critic} achieves
\begin{align*}
    \max_{z} \frac{1}{K} \sum_{k=1}^K V_1^{z, \pi_2^k}(s_1) - \min_y \frac{1}{K}\sum_{k=1}^K V_1^{\pi_1^k, y}(s_1) 
    \le \frac{1}{K}\sum_{k=1}^K\sum_{h=1}^H \delta_{h+1}^k + \frac{H}{2\eta K} + \frac{\eta AH^3}{2}.
\end{align*}
\end{theorem}
\begin{proof}
For any fixed $(h, s)$ and fixed Markov policy $z\in\Pi_1$, we have
\begin{align*}
    & \quad \frac{1}{K}\sum_{k=1}^K Q_{i,h}^\star(s, z_h(s) \times \pi_{2, h}^k(s)) \\
    & \le \frac{1}{K}\sum_{k=1}^K Q_{i,h}^k(s, z_h(s) \times \pi_{2, h}^k(s)) + \frac{1}{K}\sum_{k=1}^K \delta_{h+1}^k \\
    & \le \frac{1}{K}\sum_{k=1}^K Q_{i,h}^k(s, \pi_{h}^k(s)) + \frac{1}{K}\sum_{k=1}^K \delta_{h+1}^k + \left( \frac{1}{2\eta K} + \frac{\eta AH^2}{2} \right),
\end{align*}
where the last step applied the regret bound of GDA in Lemma~\ref{lem:gd.regret}. By symmetry, we also have for any fixed Markov policy $y\in\Pi_2$ that
\begin{align*}
    & \quad \frac{1}{K}\sum_{k=1}^K Q_{i,h}^\star(s, \pi_{1, h}^k(s)\times y_h(s)) \\
    & \ge \frac{1}{K}\sum_{k=1}^K Q_{i,h}^k(s, \pi_{h}^k(s)) - \frac{1}{K}\sum_{k=1}^K \delta_{h+1}^k - \left( \frac{1}{2\eta K} + \frac{\eta AH^2}{2} \right).
\end{align*}
Summing up these two bounds, we get
\begin{align*}
    \frac{1}{K}\sum_{k=1}^K Q_{i,h}^\star(s, z_h(s) \times \pi_{2, h}^k(s)) - \frac{1}{K}\sum_{k=1}^K Q_{i,h}^\star(s, \pi_{1, h}^k(s)\times y_h(s)) \le \frac{2}{K}\sum_{k=1}^K \delta_{h+1}^k + \left( \frac{1}{\eta K} + \eta AH^2 \right).
\end{align*}
% Next, by the performance difference decomposition, we get for any Markov policies $(z, y)\in\Pi_1\times \Pi_2$ that
% \begin{align*}
% & \quad \frac{1}{K}\sum_{k=1}^K \left[ V_1^{z, \pi_2^k}(s_1) - V_1^{\pi_1^k, y}(s_1) \right] \\
% & = \frac{1}{K}\sum_{k=1}^K \left[ V_1^{z, \pi_2^k}(s_1) - V_1^\star(s_1) + V_1^\star(s_1) - V_1^{\pi_1^k, y}(s_1) \right] \\
% & \le \sum_{h=1}^H \max_{s} Q_h^\star(
% \end{align*}
\end{proof}

\yub{This does not seem to imply the regret?}
\yub{Not very important, as OGDA achieves $\sqrt{T}$ regret.}




==> Sections/multiplayer.tex <==
\section{Multi-player General-sum Markov Games}

Let $\hat\pi$ denote the certified policy of the game, which samples $k\sim{\rm Unif}([K])$ and plays $\hat\pi_1^k$. Let $\hat\pi_h^k$ denote the certified policy starting from step $h$ and episode count $k$, which samples $j\in[k]$ from $\alpha_k^j$, plays policy $\pi_h^{j-1}$ at the $h$-th step, and then plays certified policy $\hat\pi_{h+1}^{j-1}$.

\yub{TBA: Add algorithm box for certified policy}


\begin{lemma}[Certified value function]
\label{lem.certified-value}
For Algorithm~\yub{??}, we have for all $i\in[m]$ and all $(h,k,s)\in[H]\times[K]\times \cA$ that
\begin{align*}
    V_{i,h}^k(s) = V_{i,h}^{\hat\pi_h^k}(s).
\end{align*}
\end{lemma}
\begin{proof}
\yub{Follows directly from their definitions.}
\end{proof}

\begin{lemma}[Per-state CCEGap to overall CCEGap]
\label{lem.regret-decompose}
In multi-player general-sum Markov games, suppose we have
\begin{align*}
    \max_{s} \max_{z_i\in\Delta_{A_i}} \sum_{j=1}^k \alpha_k^j \< (r_{i,h} + \P_hV_{i,h+1}^{\hat\pi_{h+1}^{j-1}}(s, \cdot), z_i\times\pi_{-i,h}^{j-1}(s) - \pi_h^{j-1}(s) \> \le \reg_{i,h}^k
\end{align*}
for all $(i,h)\in[2]\times[H+1]$, then 
$$
\|V_{i,h}^{\dagger,\hat\pi_{-i,h}^k} - V_{i,h}^{\hat\pi_{h}^k} \|_\infty
\le \reg_{i,h}^k + \sum_{j=1}^k \alpha_k^j \|V_{i,h+1}^{\dagger,\hat\pi_{-i,h+1}^{j-1}} - V_{i,h+1}^{\hat\pi_{h+1}^{j-1}} \|_\infty.
$$
\end{lemma}
\begin{proof}
\yub{Follows directly by telescoping.}
\yub{The infinity norm above is one-sided (dagger value always $\ge$ value)}
\end{proof}

\yub{Based on Lemma~\ref{lem.certified-value} \&~\ref{lem.regret-decompose}, should be able to prove that certified policy $\hat\pi$ is a CCE for multi-player general-sum. Proof should be direct by bounding $\reg_{i,h}^k$ by GDA guarantee + apply Lemma~\ref{lem.regret-decompose} and standard argument in~\citep{jin2018q} to get overall policy guarantee.}

==> Sections/outline.tex <==
\section*{Outline}

We study policy optimization algorithms for two-player zero-sum Markov games.

\begin{enumerate}
    \item Framework: General algorithm with value computation or incremental value update, and matrix game algorithm. Encompasses seemingly disparate existing algorithms as special cases.
    \begin{enumerate}
        \item Nash PI: $\alpha_t=1$, $\matrixgamealg$ is $\NE$.
        \item Nash Q-Learning: $\alpha_t=(H+1)/(H+t)$, $\matrixgamealg$ is $\NE$.
        \item Nash V-Learning: $\alpha_t=(H+1)/(H+t)$, $\matrixgamealg$ is weighted anytime FTRL.
        \item GDA/Hedge-critic: $\alpha_t=(H+1)/(H+t)$, $\matrixgamealg$ is GDA/Hedge.~\yub{new algorithm}
        \item OGDA/OFTRL-critic: $\alpha_t=(H+1)/(H+t)$, $\matrixgamealg$ is OGDA/OFTRL.
    \end{enumerate}
    \item Main generic result: state-wise policy guarantee.
    \begin{enumerate}
        \item Plug-in for above examples.
        \item Analysis slightly different from existing works (even for the sampled case such as Nash V-Learning).
    \end{enumerate} 
    \item OFTRL / OGDA $\tO(1/T)$ convergence.
    \begin{enumerate}
        \item First $1/T$ acceleration for Markov Games.
        \item Compared with Cen, they are VI style (though they do achieve $1/\eps$ query complexity with the same feedback). Our algorithm is policy optimization algorithm.
        \item \yub{anything else can be delved into this?}
    \end{enumerate}
    \item Extension to general-sum Markov Game, OFTRL achieves $T^{-3/4}$ convergence.
    \item Towards vanilla PO with eager value functions: $\alpha_t=1$, $\matrixgamealg$ is no-regret algorithm on simplex.
    \begin{enumerate}
        %   \item $\exp(H)$ algorithm?~\yub{TODO, check Chen-Yu's result in their first version}
        \item Counter-example with $\matrixgamealg$ to be Hedge or FTRL?~\yub{TODO}~\yub{also mention GDA in appendix due to projection?}
    \end{enumerate}
    \item Some issues
    \begin{enumerate}
        \item How to justify our feedback model? $Q^t\nu^t$?
    \end{enumerate}
\end{enumerate}

% We study the ``GDA-Critic" algorithm, with slowly changing $V$ updates.

% \begin{itemize}
%     \item (Done) Convergence of GDA-Critic in 2p0s.
%     \item Convergence of GDA-Critic in multi-player general-sum, with certified policy converging to CCE.
%     \begin{itemize}
%         \item Swap version for CE.
%         % \item Can certified policy be improved to simple mixture of Markov policy?
%     \end{itemize}
%     \item Abstraction.
%     \item Proof / counterexample for vanilla GDA with ``eager" value function $V^{\pi_{k-1}}$ in 2p0s~\yub{All players use the same $\eta$}~\yub{try ``cyclic" type of counterexample for $H=2$}:
%     \begin{itemize}
%         \item GDA without state distribution: $\pi_{i,h}^k(s) = \mathcal{P}_{\Delta_{A_i}}\left(\pi_{i,h}^{k-1}(s) + \eta \cdot V_{i,h}^{\pi_{k-1}}(s)\right)$. This algorithm is called ``policy mirror descent with dynamically weighted divergences" (with Euclidean distance function) in e.g.~\citep{xiao2022convergence}.
%         \item GDA with vanilla policy gradient: $\pi_{i,h}^k(s) = \mathcal{P}_{\Delta_{A_i}}\left(\pi_{i,h}^{k-1}(s) + \eta \cdot d^{\pi_{k-1}}_h(s) V_{i,h}^{\pi_{k-1}}(s)\right)$.
%     \end{itemize}
% \end{itemize}

==> Sections/proof_general_sum.tex <==
\section{Optimistic policy optimization for general-sum Markov Games}
\label{appendix:general-sum}

\subsection{Preliminaries}
\label{appendix:general-sum-prelim}

Here we formally present the preliminaries for multi-player general-sum Markov games, parallel to the zero-sum setting considered in Section~\ref{section:prelim}.

\paragraph{Multi-player general-sum Markov games} We consider tabular episodic (finite-horizon) $m$-player general-sum Markov games (MGs), which can be denoted as $\cM(H,\cS, \set{\cA_i}_{i=1}^m,\P, \set{r_i}_{i=1}^m)$, where $H$ is the horizon length; $\cS$ is the state space with $|\cS| = S$; $\cA_i$ is the action space of the $i$-th player, with $|\cA_i| = A_i$. We use $\a=(a_1,\dots,a_m)\in\prod_{i\in[m]}\cA_i\eqdef \cA$ to denote a joint action taken by all players; $\P = \{\P_h\}_{h=1}^H$ is the transition probabilities, where each $\P_h(s'|s, \a)$ gives the probability of transition to state $s'$ from state-action $(s,\a)$; $r_i = \{r_{i,h}\}_{h=1}^H$ are the reward functions, where each $r_{i,h}(s,\a)$ is the deterministic reward function of the $i$-th player at time step $h$ and state-action $(s, \a)$.
In each episode, the MG starts with a deterministic initial state $s_1$. Then at each time step $1\le h\le H$, all players observes the state $s_h$, each player takes an action $a_{i,h}\in \cA_i$. Then, each player receive their rewards $r_{i,h}(s_h, \a_h)$, and the game transitions to the next state $s_{t+1}\sim \P_h(\cdot|s_h,\a_h)$. 

% the MG starts with a fixed initial state distribution $s_1\sim \rho(\cdot)$. 
% make decisions based on this observation.  , at time step $h$ and The maximizing player

% This process will proceed iteratively until $s_{H+1}$ is reached.
% \yub{deterministic $s_1$?}

% maps the observation $s_h$ at time step $h$ to a distribution on the actions
% and the player is going to sample from this distribution (denoted as $\mu_h(\cdot|s_h)$) to get $a_h$
% \vspace{-6pt}
\paragraph{Policies \& value functions}
A (Markov) policy $\pi_i$ of the $i$-th player is a collection of policies $\pi_i = \{\pi_{i,h}: \cS \to \Delta_{\cA_i}\}_{h=1}^H$, where each $\pi_{i,h}(\cdot|s_h)\in\Delta_{\cA_i}$ specifies the probability of taking action $a_{i,h}$ at $(h, s_h)$. We use $\pi=\set{\pi_i}_{i\in[m]}$ to denote a product policy of all players. For any joint policy $\pi$ (not necessarily a product policy), we use $V_{i,h}^{\pi}: \cS\to\R$ and $Q_{i,h}^{\pi}:\cS\times\cA\to \R$ to denote the ($i$-th player's) value function and Q-function at time step $h$, respectively, i.e.%,~\yub{compress following eq?}
\begin{talign}
    V_{i,h}^{\pi}(s)&:= \E_{\pi}\brac{\sum_{h=h'}^H r_{i,h'}(s_{h'}, \a_{h'})~|~s_h = s}, \\
    Q_{i,h}^{\pi}(s,\a)&:= \E_{\pi}\brac{\sum_{h=h'}^H r_{i,h'}(s_{h'}, \a_{h'})~|~s_h = s, \a_h = \a}.
\end{talign}
For notational simplicity, we use the following abbreviation: $[\P_h V](s,\a):= \E_{s'\sim\P_h(\cdot|s,\a)}V(s')$ for any value function $V$. By definition of the value functions and Q-functions, we have the following Bellman equations for all Markov product policy $\pi$ and all $(i,h,s,\a)$:
\begin{align*}
    Q_{i,h}^{\pi}(s,\a)&= \paren{r_{i,h} + \P_hV_{i,h+1}^{\pi}} (s,\a), \\
    V_{i,h}^{\pi}(s,\a)&=\E_{\a\sim \pi_h(\cdot|s)}\brac{Q_{i,h}^{\pi}(s,\a)} = \<Q_{i,h}^{\pi}(s,\cdot), \pi_h(\cdot|s)\>.
\end{align*}
The goal for the $i$-th player is to maximize their own value function.

% \vspace{-6pt}
% \paragraph{Best response \& Nash equilibrium}

\paragraph{Correlated policy \& best response}
A (general) correlated policy $\pi$ is any policy for which players may take actions in a history-dependent and correlated fashion. More precisely, a correlated policy $\pi$ is a mapping $\set{\pi_{h}:\Omega\times (\cS\times\cA)^{h-1}\times \cS\to \Delta_{\cA}}$, and executes as follows. At the beginning of an episode, a random seed $w\in \Omega$ is sampled from some distribution (also denoted as $\Omega$ with slight abuse of notation). Then, at each step $h$ and state $s_h$, suppose the history so far is $(s_1,\a_1,\dots,s_{h-1},\a_{h-1})$. Then, $\pi$ samples a joint action $\a_h\sim \pi_h(\cdot|\omega,(s_1,\a_1,\dots,s_{h-1},\a_{h-1}); s_h)$. This formulation allows each $\pi_h(\cdot|\omega, \cdot, \cdot)$ to be a Markov product policy for any \emph{fixed} $\omega$ while still making $\pi$ to be a correlated policy, due to the correlation introduced by $\omega$.

For any correlated policy $\pi$, let $\pi_{-i}$ denote the (marginal) policy of all but the $i$-th player. Then, the ($i$-th) player's best-response value function is
\begin{align*}
    V_{i,1}^{\dagger, \pi_{-i}}(s_1) \defeq \max_{\pi_i^\dagger} V_{i,1}^{\pi_i^\dagger\times \pi_{-i}}(s_1),
\end{align*}
where the max is over all (potentially history-dependent) policy $\pi_i^\dagger$ for the $i$-th player. 
% The best-response value function $V_{i,h}^{\dagger, \pi_{-i}}$ and Q-function $Q_{i,h}^{\dagger, \pi_{-i, h}}$ can be similarly defined for any correlated policy $\pi_{-i,h:H}$ that starts from the $h$-th layer.


\paragraph{Coarse Correlated Equilibrium (CCE)}
For general-sum MGs, we consider learning an approximate Coarse Correlated Equilibrium~\citep{liu2021sharp,song2021can} defined as follows.
\begin{definition}[$\eps$-approximate Coarse Correlated Equilibrium]
\label{definition:cce}
For any $\eps\ge 0$, a correlated policy $\pi$ is an $\epsilon$-approximate Coarse Correlated Equilibrium ($\eps$-CCE) if 
\begin{align*}
    \ccegap(\pi) \defeq \max_{i\in[m]} V_{i,1}^{\dagger, \pi_{-i}}(s_1) - V_{i,1}^\pi(s_1) \le \eps.
\end{align*}
\end{definition}

% \yub{Add preliminary, notation, definition of CCEGap}

\paragraph{Additional notation}
For any Q function $Q_{i,h}(s, \cdot):\cS\times(\prod_{i=1}^m \cA_i)\to\R$ and joint policy $\pi_h(\cdot|s)$, we use $[Q_{i,h}\pi_h](s)\defeq \< Q_{i,h}(s, \cdot), \pi_h(\cdot|s)\>$ for shorthand. Similarly, for any joint policy $\pi_{-i,h}(\cdot|s)$ over all but the $i$-th player, $[Q_{i,h}\pi_{-i,h}](s, a_i)\defeq \< Q_{i,h}(s, a_i, \cdot), \pi_{-i,h}(\cdot|s)\>$.


\subsection{Algorithm and formal statement of result}
\label{appendix:general-sum-formal}

\begin{algorithm}[t]
\caption{OFTRL for multi-player general-sum Markov games}
\label{algorithm:oftrl-general-sum-mg}
\begin{algorithmic}[1]
\STATE \textbf{Initialize:} $Q_h^0(s,\a)\setto H-h+1$ for all $(h,s,a,b)$.
\FOR{$t=1,\dots,T$}
\FOR{$h=H,\dots,1$}
\STATE Update policies for all $s\in\cS$ and $i\in[m]$ by OFTRL
% ~\yub{to be edited}
\begin{align}
\label{equation:oftrl-pii}
    & \textstyle \pi_{i,h}^t(a_i | s) \propto_{a_i} \exp\paren{ (\eta/w_t) \cdot \brac{ \sum_{j=1}^{t-1} w_j(Q_{i,h}^j\pi_{-i,h}^j)(s, a_i) + w_t(Q_{i,h}^{t-1}\pi_{-i,h}^{t-1})(s, a_i) } }. 
\end{align}
\STATE Update Q-value for all $(i,s,\a)\in[m]\times \cS\times\cA$:
\begin{align}
\label{eq:Q-update-general-sum}
    Q_{i,h}^{t}(s,\a) \setto (1-\alpha_t) Q_{i,h}^{t-1}(s,\a) + \alpha_t \paren{r_h + \P_h[ Q_{i,h+1}^t\pi_{h+1}^t ]} (s,\a).
\end{align}
\ENDFOR
\ENDFOR
\STATE Output policy $\hat{\pi}^T=\hat{\pi}_1^T$, where $\hat{\pi}_1^T$ is defined in Algorithm~\ref{algorithm:certified-policy}.
% Output policy $\hat{\pi}^T={\rm Unif}(\set{\hat{\pi}_1^t}_{t=1}^T)$, where $\hat{\pi}_1^t$ is defined in Algorithm~\ref{algorithm:certified-policy}.
% \vspace{-5pt}
% \begin{equation*}
%     \widehat{\mu}_h^T(\cdot|s) \setto \sum_{t=1}^T\alpha_T^t\mu_{h}^{t}(\cdot|s),\quad 
%     \widehat{\nu}_h^T(\cdot|s)\setto\sum_{t=1}^T\alpha_T^t \nu_h^{t}(\cdot|s).
% \end{equation*}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Policy $\hat{\pi}_h^t$}
\label{algorithm:certified-policy}
\begin{algorithmic}[1]
\REQUIRE Product policies $\pi_{h'}^{t'}(\cdot|s')=\prod_{i=1}^m \pi_{i,h'}^{t'}(\cdot|s')$ for all $(h',t',s')\in[H]\times[T]\in\cS$.
\STATE Sample $j\in[t]$ with probability $\P(j=i)=\alpha_t^i$.
\STATE Play policy $\pi_h^j$ at the $h$-th step of the game.
\STATE Play policy $\hat{\pi}_{h+1}^j$ for step $h+1$ onward.
\end{algorithmic}
\end{algorithm}

% \STATE Play policy $\pi_h^t$ at the $h$-th step of the game.
% \STATE Sample $j\in[t]$ with probability $\P(j=i)=\alpha_t^i$.
% \STATE Play policy $\hat{\pi}_{h+1}^j$ for step $h+1$ onward.

% Let $\hat\pi$ denote the certified policy of the game, which samples $k\sim{\rm Unif}([K])$ and plays $\hat\pi_1^k$. Let $\hat\pi_h^k$ denote the certified policy starting from step $h$ and episode count $k$, which samples $j\in[k]$ from $\alpha_k^j$, plays policy $\pi_h^{j-1}$ at the $h$-th step, and then plays certified policy $\hat\pi_{h+1}^{j-1}$.

% \yub{TBA: Add algorithm box for certified policy}


\begin{theorem}[Formal version of Theorem~\ref{theorem:oftrl-general-sum}]
\label{theorem:oftrl-general-sum-formal}
Suppose Algorithm~\ref{algorithm:oftrl-general-sum-mg} is run for $T$ rounds. Then the per-state regret can be bounded as follows for some absolute constant $C>0$:
\begin{align*}
    \reg_h^t \le \barreg_h^t \defeq C \brac{ \frac{H\log\Amax}{\eta t} + \frac{\eta H^3}{t} + (m-1)^2\eta^3H^4 }~~~\textrm{for all}~(h,t)\in[H]\times[T].
\end{align*}
Further, choosing $\eta=(\log\Amax \log T/(H^3T))^{1/4} (m-1)^{-1/2}$, the output policy $\hat{\pi}^T$ achieves
% ~\yub{add $m$}
\begin{align*}
    \ccegap(\hat{\pi}^T) \le & \cO\Big( H^{11/4}(\log\Amax \log T)^{3/4} \sqrt{m-1} \cdot T^{-3/4} \\
    & \qquad + H^{13/4}(\log\Amax)^{1/4}(\log T)^{5/4}(m-1)^{-1/2}\cdot  T^{-5/4}  \Big).
\end{align*}
\end{theorem}


\paragraph{Proof overview and remarks} 
The proof of Theorem~\ref{theorem:oftrl-general-sum-formal} also follows by relating the performance of the output policy by per-state regrets via performance difference (Lemma~\ref{lem.regret-decompose-general-sum}), and bounding per-state regrets as $\reg_h^t\le \barreg_h^t\defeq \tO(1/(\eta t) + \eta^3(m-1)^2)$ which gives the theorem. The latter builds upon the fast convergence analysis of OFTRL in multi-player normal-form games~\citep{syrgkanis2015fast} as well as additional handling of the changing game rewards, similar as in Theorem~\ref{theorem:oftrl-main}. Note that the $\tO(T^{-3/4})$ rate here is worse than $\tO(T^{-5/6})$ for the zero-sum setting in Theorem~\ref{theorem:oftrl-main}. This happens as the fine-grained analysis of OFTRL~\citep{chen2020hedging} used there relies critically on the game having two players (for translating between the iterate stabilities and loss stabilities between each other), and becomes infeasible when there are more than 2 players. % ~\yub{this paragraph may be moved to appendix}

We first present some lemmas in Section~\ref{appendix:general-sum-lemmas}. The proof of Theorem~\ref{theorem:oftrl-general-sum-formal} is then provided in Section~\ref{appendix:proof-oftrl-general-sum-formal}.

\subsection{Useful lemmas}
\label{appendix:general-sum-lemmas}

We additionally define the V-values maintained by Algorithm~\ref{algorithm:oftrl-general-sum-mg} as
%~\yub{to be modified}
\begin{align}
    V_{i,h}^t(s) \defeq \sum_{j=1}^t \alpha_t^j \brac{Q_{i,h}^j \pi_h^j}(s)
    % V_{i,h}^t(s) = \<Q_{i,h}^t(s, \cdot), \pi_h^t(\cdot|s)\>,
\end{align}
for all $(i,h,t,s)\in[m]\times[H]\times[T]\times\cS$, where $Q_{i,h}^t$ and $\pi_h^t$ are the Q-functions and joint policies maintained within Algorithm~\ref{algorithm:oftrl-general-sum-mg}. Note that by~\eqref{eq:Q-update-general-sum}, we immediately have
\begin{align}
    \label{equation:q-v-general-sum}
    \begin{aligned}
    & \quad Q_{i,h}^t(s,\a) = \sum_{j=1}^t \alpha_t^j \brac{ r_h + \P_h[Q_{i,h+1}^j\pi_{h+1}^j]}(s, \a) \\
    & = \paren{r_h + \P_h\brac{ \sum_{j=1}^t \alpha_t^j Q_{i,h+1}^j\pi_{h+1}^j } }(s, \a) = \paren{r_h + \P_h V_{i,h+1}^t}(s, \a).
\end{aligned}
\end{align}

\begin{lemma}[Equivalence of value functions]
\label{lem.certified-value}
For Algorithm~\ref{algorithm:oftrl-general-sum-mg}, we have for all $i\in[m]$ and all $(h,s,t)\in[H+1]\times\cS\times[T]$ that
\begin{align*}
    V_{i,h}^t(s) = V_{i,h}^{\hat\pi_h^t}(s).
\end{align*}
\end{lemma}
\begin{proof}
We prove this by backward induction over $h\in[H+1]$. The claim trivially holds for $h=H+1$. Suppose the claim holds for steps $h+1$ onward and all $(s,t)\in\cS\times[T]$. For step $h$ and any fixed $(s,t)\in\cS\times[T]$, note that
\begin{align*}
    & \quad V_{i,h}^t(s) = \sum_{j=1}^t \alpha_t^j \brac{Q_{i,h}^j\pi_h^j}(s) \stackrel{(i)}{=} \sum_{j=1}^t \alpha_t^j \brac{(r_h + \P_h V_{i,h+1}^j)\pi_h^j}(s) \\
    & \stackrel{(ii)}{=} \sum_{j=1}^t \alpha_t^j \brac{(r_h + \P_h V_{i,h+1}^{\hat{\pi}_{h+1}^j})\pi_h^j}(s) \stackrel{(iii)}{=} V_{i,h}^{\hat{\pi}_h^t}(s).
    % & \<\paren{r_h + \P_h[Q_{i,h+1}^j\pi_{h+1}^j]}(s,\cdot), \pi_h^t(\cdot|s)\> \\
    % & = \sum_{j=1}^t \alpha_t^j 
    % \<\paren{r_h + \P_hV_{i,h+1}^j}(s,\cdot), \pi_h^t(\cdot|s)\> \\
    % & \stackrel{(ii)}{=}  \sum_{j=1}^t \alpha_t^j 
    % \<\paren{r_h + \P_hV_{i,h+1}^{\hat{\pi}_{h+1}^j}}(s,\cdot), \pi_h^t(\cdot|s)\> \stackrel{(iii)}{=} V_{i,h}^{\hat{\pi}_h^t}(s).
\end{align*}
Above, (i) follows by~\eqref{equation:q-v-general-sum}; (ii) uses the inductive hypothesis; (iii) uses the definition of the output policy $\hat{\pi}_h^t$ (cf. Algorithm~\ref{algorithm:certified-policy}), which samples $j\in[t]$ with probability $\alpha_t^j$, plays $\pi_h^j(\cdot|s)$, and plays $\hat{\pi}_{h+1}^j$ for the rest of the game. This proves the case for step $h$ and thus the lemma.
% \yub{Follows directly from their definitions.}
\end{proof}

% \yub{Add def of dagger values starting from step $h$}


Define the weighted per-state regrets as
\begin{align}
    & \reg_{h,i}^t(s) \defeq \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{j=1}^t \alpha_t^j \< Q_h^j(s, \cdot), (\pi_i^\dagger\times\pi_{-i,h}^j)(\cdot|s) - \pi_h^j(\cdot|s)\> , \label{equation:reghits} \\
    & \reg_h^t \defeq \max_{s\in\cS} \max_{i\in[m]} \reg_{h,i}^t(s). \label{equation:reght-general-sum}
\end{align}
The following lemma bounds the difference between the values of the certified policy $\pi_h^t$ (Algorithm~\ref{algorithm:certified-policy}) and its best-response. We define the value functions of $\hat{\pi}_h^t$ and of its best response for any $(i,h,t,s)$ as (see e.g.~\citep[Definition C.4 \& Eq.(8)]{song2021can}):
\begin{align*}
    & V_{i,h}^{\hat\pi_{h}^t}(s) \defeq \E_{\hat{\pi}_h^t}\brac{ \sum_{h'=h}^H r_{i,h'} | s_h = s }, \\
    & V_{i,h}^{\dagger, \hat\pi_{-i,h}^t}(s) \defeq \max_{\pi_{i,h:H}} \E_{\pi_{i,h:H}\times \hat{\pi}_{-i,h}^t} \brac{ \sum_{h'=h}^H r_{i,h'} | s_h = s }.
\end{align*}


\begin{lemma}[Recursion of best-response values]
\label{lem.regret-decompose-general-sum}
% In multi-player general-sum Markov games, suppose we have
% \begin{align*}
%     \max_{s} \max_{z_i\in\Delta_{A_i}} \sum_{j=1}^k \alpha_k^j \< (r_{i,h} + \P_hV_{i,h+1}^{\hat\pi_{h+1}^{j-1}}(s, \cdot), z_i\times\pi_{-i,h}^{j-1}(s) - \pi_h^{j-1}(s) \> \le \reg_{i,h}^k
% \end{align*}
For the policy $\hat{\pi}_h^t$ defined in Algorithm~\ref{algorithm:certified-policy}, we have for all $(i, h,t)\in[m]\times[H]\times[T]$ that
$$
\linf{V_{i,h}^{\dagger,\hat\pi_{-i,h}^t} - V_{i,h}^{\hat\pi_{h}^t} }
\le \reg_{h}^t + \sum_{j=1}^t \alpha_t^j \linf{ V_{i,h+1}^{\dagger,\hat\pi_{-i,h+1}^{j}} - V_{i,h+1}^{\hat\pi_{h+1}^{j}} }.
$$
\end{lemma}
\begin{proof}
Fix $(i,h,t)\in[m]\times[H]\times[T]$. Note that by definition the left-hand side above within the $\linf{\cdot}$ is non-negative~\yub{fix}. Further, we have for any $s\in\cS$ that
\begin{align*}
    & \quad V_{i,h}^{\dagger,\hat\pi_{-i,h}^t}(s) - V_{i,h}^{\hat\pi_{h}^t}(s) \\
    & = \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \<\pi_i^\dagger, \sum_{j=1}^t \alpha_t^j \brac{(r_h + \P_h V_{i,h+1}^{\dagger, \hat{\pi}_{-i,h+1}^j}) \pi_{-i,h}^j}(s, \cdot) \> - \sum_{j=1}^t \alpha_t^j \<\pi_{i,h}^j, \brac{(r_h + \P_h V_{i,h+1}^{\hat{\pi}_{h+1}^j}) \pi_{-i,h}^j}(s, \cdot) \> \\
    & \stackrel{(i)}{\le} \sum_{j=1}^t \alpha_t^j \linf{V_{i,h+1}^{\dagger,\hat\pi_{-i,h+1}^{j}} - V_{i,h+1}^{\hat\pi_{h+1}^{j}}} + \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{j=1}^t \alpha_t^j \<\pi_i^\dagger - \pi_{i,h}^j, \brac{(r_h + \P_h V_{i,h+1}^{\hat{\pi}_{h+1}^j}) \pi_{-i,h}^j}(s, \cdot)\> \\
    & \stackrel{(ii)}{=} \sum_{j=1}^t \alpha_t^j \linf{V_{i,h+1}^{\dagger,\hat\pi_{-i,h+1}^{j}} - V_{i,h+1}^{\hat\pi_{h+1}^{j}}} + \underbrace{\max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{j=1}^t \alpha_t^j \<\pi_i^\dagger - \pi_{i,h}^j, \brac{(r_h + \P_h V_{i,h+1}^{j}) \pi_{-i,h}^j}(s, \cdot)\>}_{\reg_{i,h}^t(s)} \\
    & \le \sum_{j=1}^t \alpha_t^j \linf{V_{i,h+1}^{\dagger,\hat\pi_{-i,h+1}^{j}} - V_{i,h+1}^{\hat\pi_{h+1}^{j}}} + \reg_h^t.
\end{align*}
Above, (i) follows by substituting $V_{i,h+1}^{\dagger, \hat{\pi}_{-i,h+1}^j}$ with $V_{i,h+1}^{\hat{\pi}_{h+1}^j}$ and paying the additive error; (ii) follows from Lemma~\ref{lem.certified-value}. This proves the desired result.
% \yub{Follows directly by telescoping.}
% \yub{The infinity norm above is one-sided (dagger value always $\ge$ value)}
\end{proof}


\begin{lemma}[Guarantee of Algorithm~\ref{algorithm:oftrl-general-sum-mg} via per-state regrets]
\label{lemma:master-general-sum}
Suppose that the per-state regrets~\eqref{equation:reght-general-sum} can be upper-bounded as $\reg_h^t\le \barreg_h^t$ for all $(h,t)\in[H]\times[T]$, where $\barreg_h^t$ is non-increasing in $t$: $\barreg_h^t\ge \barreg_h^{t+1}$ for all $t\ge 1$. Then running Algorithm \ref{algorithm:oftrl-general-sum-mg} will guarantee that
\begin{equation}\label{eq:NE-gap-general-sum}
    \ccegap(\hat{\pi}^T)\le CH \cdot \frac{1}{T} \sum_{t=1}^T \max_{h\in[H]}\barreg_h^t.
    % \paren{\sum_{h=0}^{H-1} \cbeta^h}
    %2\sum_{h'=h}^H\avgreg_{h'}^k + \frac{4}{k}\sum_{h'=h}^H\sum_{t=1}^k\delta_{h'}^{t}
\end{equation}
for all $T\ge 2$, where $C>0$ is an absolute constant.
% where $\cbeta$ is a constant that satisfies:
% \begin{equation}\label{eq:def-c}
%     \textstyle
%     \cbeta \ge \max\set{1, \sup_{j\ge 1} \sum_{t=j}^{\infty}\beta_t^j}.
%     % , ~~\forall j\ge1
% \end{equation}
\end{lemma}
\begin{proof}
For any $(h,t)\in[H+1]\times[T]$, define
\begin{align*}
    \delta_h^t \defeq \max_{i\in[m]} \linf{ V_{i,h}^{\dagger,\hat\pi_{-i,h}^t} - V_{i,h}^{\hat\pi_{h}^t} }.
\end{align*}
Then Lemma~\ref{lem.regret-decompose-general-sum} implies the recursive relationship
\begin{align*}
    \delta_h^t \le \reg_h^t + \sum_{j=1}^t \alpha_t^j \delta_{h+1}^j.
\end{align*}
Therefore we can imitate the proof of Lemma~\ref{lemma:recursion-of-value-estimation} and obtain that, for any $\barreg_h^t$ such that $\reg_h^t\le \barreg_h^t$ and $\barreg_h^t\ge \barreg_h^{t+1}$,
\begin{align*}
    \delta_h^t \le H\cbeta^{H-1}\cdot \frac{1}{t}\sum_{j=1}^t \max_{h'\in[H]}\barreg_{h'}^j,
\end{align*}
where $\cbeta=1+1/H= \sup_{j\ge 1} \sum_{t=j}^\infty \alpha_t^j$ by Lemma~\ref{lemma:alpha-ti}(a).

Further, by definition of the output policy $\hat{\pi}^T=\hat{\pi}_1^T$ (cf. Algorithm~\ref{algorithm:certified-policy}), we have
\begin{align*}
    & \quad \ccegap(\hat{\pi}^T) = V_{i,1}^{\dagger, \hat{\pi}_{-i,1}^T}(s_1) - V_{i,1}^{\hat{\pi}_1^T}(s_1) \le \delta_1^T \le H\cbeta^{H-1}\cdot \frac{1}{T}\sum_{t=1}^T \max_{h\in[H]}\barreg_{h}^t \\
    & \le CH \cdot \frac{1}{T}\sum_{t=1}^T \max_{h\in[H]}\barreg_{h}^t,
\end{align*}
where $C\le 3$ as $\cbeta^{H-1}\le (1+1/H)^H\le e\le 3$. This is the desired result.
% \yub{Then do recursion using F.2, similar as before, should have one less term in the final bound.}
% \yub{Have not checked constants.}~\yub{priority to check before deadline}
\end{proof}

\subsection{Proof of Theorem~\ref{theorem:oftrl-general-sum-formal}}
\label{appendix:proof-oftrl-general-sum-formal}

\paragraph{Bounding per-state regret}
We first bound $\reg_{i, h}^t(s)$ (cf. definition in~\eqref{equation:reghits}), i.e. the per-state regret for the $i$-th player, for any fixed $(i,h,s,t)\in[m]\times[H]\times[S]\times[T]$. This is the main part of this proof. 

Throughout this part, we will fix $(i,h,s,t)$, and omit the subscript $(h,s)$ within the policies and Q functions, so that $\pi_{i,h}^t(\cdot|s)$ will be abbreviated as $\pi_i^t$, and $Q_{i,h}^t(s, \cdot)$ will be abbreviated as $Q_i^t$. We will also reload $T\ge 1$ to be any positive integer (instead of the fixed total number of iterations).

We first observe that the update~\eqref{equation:oftrl-pii} for $\pi_{i,h}^t(\cdot|s)$ is exactly equivalent to the OFTRL algorithm (Algorithm~\ref{alg:OFTRL}) with loss vectors $g_t=w_t(Q_i^t)^\top \pi_{-i}^t$ (understanding $g_0=0$ and $Q_i^0=0$), prediction vector $M_t=w_{t}(Q_i^{t-1})^\top\pi_{-i}^{t-1}$, and learning rate $\eta_t=\eta/w_t$. Therefore we can apply the regret bound for OFTRL in Lemma~\ref{lemma:OFTRL-auxillary} and obtain for any $T\ge 1$ that
\begin{equation}
\label{equation:oftrl-regret-initial-general-sum}
\begin{aligned}
    & \quad \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{t=1}^T w_t \<\pi_i^t - \pi_i^\dagger, Q_i^t\pi_{-i}^t\> = \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{t=1}^T \<\pi_i^t - \pi_i^\dagger, g_t\>\\
    & \le \frac{\log A_i}{\eta_T} + 
    \sum_{t=1}^{T} \eta_t \|g_t-M_t\|_\infty^2  -\sum_{t=1}^{T-1} \frac{1}{8\eta_t}\|\pi_i^t-\pi_i^{t+1}\|_1^2 \\
    & \le \frac{\log A_i\cdot w_T}{\eta} + 
    \sum_{t=1}^{T} \eta w_t\|Q_i^t\pi_{-i}^t-Q_i^{t-1}\pi_{-i}^{t-1}\|_\infty^2 \\
    & \le \frac{\log \Amax \cdot w_T}{\eta} + 
    \underbrace{\sum_{t=1}^{T} 2\eta w_t \linf{Q_i^t-Q_i^{t-1}}^2}_{\rm I} + \underbrace{\sum_{t=2}^T 2\eta w_t H^2\lone{\pi_{-i}^t - \pi_{-i}^{t-1}}^2}_{\rm II}.
\end{aligned}
\end{equation}
Above, the last inequality uses the fact that $\linf{(Q_i^t-Q_i^{t-1})\pi_{-i}^t}\le \linf{Q_i^t-Q_i^{t-1}}$ for $t\ge 1$, and $\linf{Q_i^{t-1}(\pi_{-i}^t - \pi_{-i}^{t-1})}\le H\lone{\pi_{-i}^t - \pi_{-i}^{t-1}}$ for $t\ge 2$.

For term ${\rm I}$, noticing that $\linf{Q_i^t - Q_i^{t-1}}\le \alpha_t H$ by~\eqref{eq:Q-update-general-sum}, we have
\begin{align*}
    {\rm I} \le \sum_{t=1}^T 2\eta w_t \alpha_t^2 H^2 = 2\eta H^2 \sum_{t=1}^T w_t \alpha_t^2.
\end{align*}

Bounding term ${\rm II}$ requires the following lemma on the stability of the iterates. The proof can be found in Section~\ref{appendix:proof-general-sum-stability}.
\begin{lemma}[Stability of iterates]
\label{lemma:general-sum-stability}
We have for any $i\in[m]$ and any $t\ge 2$ that (recall the subscripts $(h,s)$ are omitted below):
% for all $(i,h,s)\in[m]\times[H]\times\cS$ and $t\ge 2$ that
\begin{align}
\label{equation:stability-general-sum}
    \lone{\pi_i^t - \pi_{i}^{t-1}} \le 4\eta H.
\end{align}
Consequently,
\begin{align}
\label{equation:stability-total-general-sum}
    \lone{\pi_{-i}^t - \pi_{-i}^{t-1}} \le 4(m-1)\eta H.
\end{align}
% \yub{check constant}
\end{lemma}

Using Lemma~\ref{lemma:general-sum-stability}, we have
\begin{align*}
    {\rm II} \le \sum_{t=2}^T 2\eta w_t H^2 \cdot 16(m-1)^2 \eta^2 H^2 = 32\eta^3 H^4 (m-1)^2 \sum_{t=2}^T w_t.
\end{align*}

Plugging the preceding bounds into~\eqref{equation:oftrl-regret-initial-general-sum} and using $\alpha_T^1\cdot w_t=\alpha_T^t$ yields that
\begin{align*}
    & \quad \reg_{i,h}^T(s) = \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{t=1}^T \underbrace{\alpha_T^t}_{\alpha_T^1\cdot w_t} \<\pi_i^t - \pi_i^\dagger, Q_i^t\pi_{-i}^t\> = \alpha_T^1 \max_{\pi_i^\dagger\in\Delta_{\cA_i}} \sum_{t=1}^T w_t \<\pi_i^t - \pi_i^\dagger, Q_i^t\pi_{-i}^t\> \\
    & \le \frac{\log\Amax \cdot \alpha_T^T}{\eta} + 2\eta H^2 \sum_{t=1}^T \alpha_T^t \alpha_t^2 + 32\eta^3 H^4 (m-1)^2 \underbrace{\sum_{t=2}^T \alpha_T^t}_{\le 1} \\
    & \stackrel{(i)}{\le} \frac{2H\log\Amax}{\eta T} + \frac{8\eta H^3}{T} + 32\eta^3 H^4 (m-1)^2 \\
    & \le C\brac{ \frac{H\log\Amax}{\eta T} + \frac{\eta H^3}{T} + \eta^3 H^4 (m-1)^2 } \eqdef \barreg_h^T.
\end{align*}
Above, (i) used the fact that $\alpha_T^T=\alpha_T=(H+1)/(H+T)\le 2H/T$, and $\sum_{t=1}^T\alpha_T^t\alpha_t^2 \le 4H/T$ by Lemma~\ref{lemma:alpha-convolution}(c), and $C\le 32$ is an absolute constant. This proves the per-state regret bounds claimed in Theorem~\ref{theorem:oftrl-general-sum-formal}.


\paragraph{Overall policy guarantee}
Plugging the above per-state regret bounds into Lemma~\ref{lemma:master-general-sum} yields that, the output policy $\hat{\pi}^T$ of Algorithm~\ref{algorithm:oftrl-general-sum-mg} achieves
\begin{align*}
    & \quad \ccegap(\hat{\pi}^T) \le CH \cdot \frac{1}{T} \sum_{t=1}^T \max_{h\in[H]} \barreg_h^T \\
    & \le \cO\paren{ \frac{H^2\log\Amax \log T}{\eta T} + \frac{\eta H^4\log T}{T} + \eta^3 H^5 (m-1)^2 }.
\end{align*}
Choosing $\eta=(\log\Amax \log T/(H^3T))^{1/4} (m-1)^{-1/2}$, the above can be upper bounded as
\begin{align*}
    \cO\paren{ H^{11/4}(\log\Amax \log T)^{3/4} \sqrt{m-1} \cdot T^{-3/4} + H^{13/4}(\log\Amax)^{1/4}(\log T)^{5/4}(m-1)^{-1/2}\cdot  T^{-5/4}  },
\end{align*}
which is the desired result.
\qed


% \yub{Based on Lemma~\ref{lem.certified-value} \&~\ref{lem.regret-decompose}, should be able to prove that certified policy $\hat\pi$ is a CCE for multi-player general-sum. Proof should be direct by bounding $\reg_{i,h}^k$ by GDA guarantee + apply Lemma~\ref{lem.regret-decompose} and standard argument in~\citep{jin2018q} to get overall policy guarantee.}



\subsection{Proof of Lemma~\ref{lemma:general-sum-stability}}
\label{appendix:proof-general-sum-stability}

We first prove~\eqref{equation:stability-general-sum}. By the OFTRL update~\eqref{equation:oftrl-pii} and the smoothness of exponential weights (Lemma~\ref{lemma:Hedge-smoothness}), we have for any $t\ge 2$ that
\begin{align*}
    \lone{\pi_i^t - \pi_i^{t-1}} \le 2\linf{G^t - G^{t-1}},
\end{align*}
where $G^t, G^{t-1}$ are the (weighted) total losses in~\eqref{equation:oftrl-pii}:
\begin{align*}
    & G^t \defeq \frac{\eta}{w_t} \brac{\sum_{j=1}^{t-1} w_j Q_i^j \pi_{-i}^j + w_t Q_i^{t-1} \pi_{-i}^{t-1}}, \\
    & G^{t-1} \defeq \frac{\eta}{w_{t-1}} \brac{\sum_{j=1}^{t-2} w_j Q_i^j \pi_{-i}^j + w_{t-1} Q_i^{t-2} \pi_{-i}^{t-2}}. \\
\end{align*}
Therefore we have
\begin{align*}
    & \quad \lone{\pi_i^t - \pi_i^{t-1}} \le 2\linf{G^t - G^{t-1}} \\
    & \le 2\eta \linf{ \paren{\frac{1}{w_t} - \frac{1}{w_{t-1}}} \sum_{j=1}^{t-1} w_j Q_i^j \pi_{-i}^j } + 2\eta \linf{2Q_i^{t-1}\pi_{-i}^{t-1} - Q_i^{t-2}\pi_{-i}^{t-2}} \\
    & \stackrel{(i)}{\le} 2\eta H \cdot \underbrace{\paren{\frac{1}{w_{t-1}} - \frac{1}{w_{t}}} \sum_{j=1}^{t-1} w_j}_{\stackrel{(ii)}{=} H/(H+1)\le 1} + 2\eta H \le 4\eta H.
\end{align*}
Above, (i) uses the fact that $Q_i^j\pi_{-i}^j\in[0, H]$ entry-wise for all $j\ge 1$, and (ii) uses Lemma~\ref{lemma:wt}(b). This proves~\eqref{equation:stability-general-sum}.

The above directly implies~\eqref{equation:stability-total-general-sum} by the following bound on the TV distance (or $L_1$ norm) of product distributions~\citep{syrgkanis2015fast}:
\begin{align*}
    \lone{\pi_{-i}^t - \pi_{-i}^{t-1}} \le \sum_{j\neq i} \lone{\pi_j^t - \pi_j^{t-1}}.
\end{align*}
This completes the proof.
% \yub{cite vasilis for TV distance.}
\qed

==> Sections/regret.tex <==
\section{Separable Rock-Paper-Scissor}

We show that GDA without critic does not achieve sublinear regret.

We consider a special case of  two-player zero-sum Markov where there is only a single state per step. 
In this case, the transitions are totally independent of players' actions. Therefore, we can also view it as a composition of $H$ independent matrix games. 
In each matrix game, we choose the payoff matrix  for player $1$ to be the same $2\times2$ identity matrix. That is, player $1$ will receive reward $1$ if she picks the same action as player $2$, and otherwise receive zero reward.

Assume we run GDA on each matrix game starting from the same initial  point $(x_0,y_0)=(\mathbf{e}_1,\mathbf{e}_1)$ with learning rate $\eta$. Denote the Nash equilibrium by $(x^\star,y^\star)$.
\begin{lemma}\label{lem:rps-0}
Given $x\in \mathbb{R}^{2}$, if $\|x-(1/2,1/2)\trans\|_2 \le 0.1$, then $\cP_{\Delta_2}(x)= x + (1-\|x_1\|_1)\times (1/2,1/2)\trans$.
\end{lemma}
The proof of this lemma follows from standard algebra, which we omit here.


\begin{lemma}\label{lem:rps-1}
There exists an absolute constant $c\in(0,1)$ such that for any $x,y\in\Delta_2$ satisfying 
 $$
 \left\|
 \begin{pmatrix}
 x\\
 y
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 \right\|_2\in (\frac{c}{2},c),
 $$
\yub{$[0, c)$ also works?}~and $\eta \le c$, we have 
  $$
 \left\|
 \begin{pmatrix}
 \cP_{\Delta_2} (x+\eta y)\\
 \cP_{\Delta_2} (y-\eta x)
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 \right\|_2
 \ge \left\|
 \begin{pmatrix}
 x\\
 y
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 \right\|_2.
 $$
\end{lemma}
\begin{proof}
By Lemma \ref{lem:rps-0}, if $x+\eta y$ is sufficiently close to $(1/2,1/2)\trans$, then we have  $\cP_{\Delta_2} (x+\eta y)= x+\eta y - \eta (1/2,1/2)\trans$. 
Similarly, we also have 
$\cP_{\Delta_2} (y-\eta x)= y-\eta x + \eta (1/2,1/2)\trans$.
Therefore, we have 
$$
\begin{pmatrix}
 \cP_{\Delta_2} (x+\eta y)\\
 \cP_{\Delta_2} (y-\eta x)
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 = 
 \begin{pmatrix}
x -x^\star+\eta y-\eta (1/2,1/2)\trans\\
 y-y^\star -\eta x+\eta (1/2,1/2)\trans
 \end{pmatrix}
$$
Observe that 
$$
\left\langle 
 \begin{pmatrix}
x -x^\star\\
 y-y^\star 
 \end{pmatrix}, \begin{pmatrix}
\eta y-\eta (1/2,1/2)\trans\\
 -\eta x+\eta (1/2,1/2)\trans
 \end{pmatrix}
\right\rangle
=
\left\langle 
 \begin{pmatrix}
x -x^\star\\
 y-y^\star 
 \end{pmatrix}, \begin{pmatrix}
\eta y\\
 -\eta x
 \end{pmatrix}
\right\rangle
=\left\langle 
 \begin{pmatrix}
x -\eta (1/2,1/2)\trans\\
 y-\eta (1/2,1/2)\trans 
 \end{pmatrix}, \begin{pmatrix}
\eta y\\
 -\eta x
 \end{pmatrix}
\right\rangle
= 0.
$$
So we conclude that 
 $$
 \left\|
 \begin{pmatrix}
 \cP_{\Delta_2} (x+\eta y)\\
 \cP_{\Delta_2} (y-\eta x)
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 \right\|_2
 \ge \left\|
 \begin{pmatrix}
 x\\
 y
 \end{pmatrix}-
 \begin{pmatrix}
 x^\star\\
 y^\star
 \end{pmatrix}
 \right\|_2.
 $$
\end{proof}

\begin{theorem}\label{thm:rps}
There exist two absolute constants $c,C>0$ such that if $H>C$ and we run GDA on each matrix game starting from the same initial  point $(x_0,y_0)=(\mathbf{e}_1,\mathbf{e}_1)$ with learning rate $\eta<c$, then 
\begin{align*}
    \max_{z} \frac{1}{K} \sum_{k=1}^K V_1^{z, \pi_2^k}(s_1) - \min_y \frac{1}{K}\sum_{k=1}^K V_1^{\pi_1^k, y}(s_1) 
    \ge \Theta(1) .
\end{align*}
\end{theorem}
\yub{Intuition: Pick non-Markov $z$}
\begin{proof}
 We first claim that the policies induced by running GDA have the same distribution at different steps, so we can denote $x_k = \pi_{1,h}^k$ and $y_k = \pi_{2,h}^k$ for all $h\in[H]$.~\yub{By the property that GDA is not affected by any $c\ones$ component within the gradient.}
 
 
By Lemma \ref{lem:rps-1}, there exists constant $c_1$ so that $\sum_{k=1}^K \sqrt{ \|x_k-x^\star\|_2^2 + \|y_k-y^\star\|_2^2 } \ge c_1 K$. Therefore, $\max\{\sum_{k=1}^K \|x_k-x^\star\|_2,\sum_{k=1}^K \|y_k-y^\star\|_2\} \ge c_1 K$.


WLOG, assume $\sum_{k=1}^K \|x_k-x^\star\|_2\ge c_1 K$.
Now we want to utilize this condition to show  the mixture of $x_1,\ldots,x_K$ is $\Theta(1)$-exploitable by  constructing the following policy to play against the mixture of $x_1,\ldots,x_K$:
\begin{itemize}
    \item From step $1$ to step $m$, we always play $y^\star$. Since  we are playing the Nash policy, we have expected reward equal to $1/2$ per step. However, during these $m$ steps, we can observe the actions picked by the opponent and estimate its policy up to  accuracy $\cO(\sqrt{\frac{\log(\delta)}{m}})$  with probability at least $1-\delta$.
    \item In the remaining $H-m$ steps, we play the best response to the estimated policy.
\end{itemize}
It is direct to see the expected cumulative rewards of our strategy  is lower bounded by 
$$
\frac{m}{2}+\frac{1}{K}\sum_{k=1}^K (1-\delta)\left(\max_{y}x_k\trans y -\cO\left(\sqrt{\frac{\log(\delta)}{m}}\right)\right)(H-m).
$$
Recall that $\sum_{k=1}^K \|x_k-x^\star\|_2\ge c_1 K$. Therefore, if we choose $m\ge \Theta(\log(1/c_1)/c_1^2)$ and $\delta \le \cO(c_1)$, then we can obtain
$$
\frac{1}{K}\sum_{k=1}^K (1-\delta)\left(\max_{y}x_k\trans y -\cO\left(\sqrt{\frac{\log(\delta)}{m}}\right)\right) \ge \frac12 + \Theta(c_1),
$$
which implies the mixture of $x_1,\ldots,x_K$ is $\Theta(c_1)$-exploitable.
\end{proof}




\yub{Check separable Rock-Paper-Scissor example}

==> Sections/time_varying.tex <==
\def\tvalg{{\sc TVAlg}}

\section{Time-varying matrix games}

Here we summarize some guarantees of~\citep{zhang2022no}'s algorithm for a sequence of time-varying matrix games $A_t\in[0,1]^{m\times n}$, henceforth \tvalg, on the following special scenario:
\begin{align*}
    A_t = A_\star + E_t,~~~\linf{E_t}\le \eps\le 1,
\end{align*}
and no further assumption on $E_t$, in particular it may be adversarial instead of random noise. We assume both players run the \tvalg~algorithm.

We further assume $\eps T\ge 1$, i.e. $\eps\ge 1/T$.

For this set of matrices, the stationarity measures defined in~\citep[Section 3]{zhang2022no} satisfy
\begin{align*}
    V_T \le \eps^2T,~~~W_T \le \eps T,~~~P_T~\textrm{can be}~\Theta(T)~\textrm{in general}.
\end{align*}

\begin{cor}[Theorem 4 of~\citep{zhang2022no}]
We have the individual regret bound for both players (summed):
\begin{align*}
\max_{x} \sum_{t=1}^T x^\top A_t y_t - \min_y \sum_{t=1}^T x_t^\top A_t y \le \tO(\sqrt{\eps T}).
\end{align*}
Consequently, we have the regret bound on $A_\star$:
\begin{align*}
\max_{x} \sum_{t=1}^T x^\top A_\star y_t - \min_y \sum_{t=1}^T x_t^\top A_\star y \le \tO(\eps T).
\end{align*}
\end{cor}


\begin{cor}[Theorem 6 of~\citep{zhang2022no}]
We have the dynamic NE regret bound:
\begin{align*}
\abs{ \sum_{t=1}^T x_t^\top A_t y_t - \sum_{t=1}^T \max_x \min_y x^\top A_t y } \le \tO(\eps T),
\end{align*}
Consequently, we have the dynamic NE regret bound on $A_\star$:
\begin{align*}
\abs{ \sum_{t=1}^T x_t^\top A_\star y_t - \sum_{t=1}^T \max_x \min_y x^\top A_\star y } \le \tO(\eps T).
\end{align*}
\end{cor}


\begin{cor}[Theorem 8 of~\citep{zhang2022no}]
We have the duality gap bound:
\begin{align*}
\sum_{t=1}^T \max_x x^\top A_t y_t - \min_y x_t^\top A_t y \le \tO(\eps^{1/4} T),
\end{align*}
Consequently, we have the duality gap bound on $A_\star$:
\begin{align*}
\sum_{t=1}^T \max_x x^\top A_\star y_t - \min_y x_t^\top A_\star y \le \tO(\eps^{1/4} T).
\end{align*}
\end{cor}

As comparison we also present Chen-Yu's result for handling $\eps$:
\begin{cor}[Theorem 1 of~\citep{wei2021last}]
OGDA algorithm with game matrix $A_t$ achieves duality gap bound
\begin{align*}
    \sum_{t=1}^T \max_x x^\top A_\star y_t - \min_y x_t^\top A_\star y \le \tO(\sqrt{T} + \sqrt{\eps}T).
\end{align*}
\end{cor}






